Symmetry Breaking for k-Robust Multi-Agent Path Finding

During Multi-Agent Path Finding (MAPF) problems, agents can be delayed by unexpected events. To address such situations recent work describes k-Robust Conflict-BasedSearch (k-CBS): an algorithm that produces coordinated and collision-free plan that is robust for up to k delays. In this work we introducing a variety of pairwise symmetry breaking constraints, specific to k-robust planning, that can efficiently find compatible and optimal paths for pairs of conflicting agents. We give a thorough description of the new constraints and report large improvements to success rate ina range of domains including: (i) classic MAPF benchmarks;(ii) automated warehouse domains and; (iii) on maps from the 2019 Flatland Challenge, a recently introduced railway domain where k-robust planning can be fruitfully applied to schedule trains.

==> K-Robust Symmetry Breaking (4)/Makefile <==
FICHIER = main

TEXFILES = $(wildcard *.tex) $(wildcard images/*.tex) $(wildcard algo/*.tex) $(wildcard tikz/*.tex) 
BIBFILE  = $(wildcard *.bib)
FIGFILES = $(wildcard images/*.fig)
EPSFILES = $(patsubst %.fig,%.eps,$(FIGFILES))

TMPFILES  = $(wildcard *.aux) $(wildcard *.bbl) $(wildcard *.ps) $(wildcard *.dvi) $(wildcard *.blg) $(wildcard *.toc) $(wildcard *.lof) $(wildcard *.log) $(wildcard *.lot) 
BACKFILES = $(wildcard *.bak) $(wildcard */*.bak) $(wildcard *~) $(wildcard */*~) $(wildcard *.tar.gz)
TRUCFILES = $(wildcard _*)

DOTFILES = $(wildcard *.dot)
PSDOTFILES = $(patsubst %.dot,%.tps,$(DOTFILES))

all: $(FICHIER).pdf

%.pdf: $(TEXFILES)
	pdflatex $(FICHIER)
	if grep -q 'citation' $(FICHIER).aux; then if grep -q 'bibdata' $(FICHIER).aux; then bibtex $(FICHIER); fi else rm -f $(FICHIER).bbl; fi
	pdflatex $(FICHIER) 
	pdflatex $(FICHIER)

#%.pdf: %.ps
#	ps2pdf $<

#%.tps: %.dot
#	dot -Tps -o $@ $<

%.ps:  %.dvi
	dvips -o $@ $< > /dev/null
#	dvips -Pcmz -Pamz -o $@ $< > /dev/null

%.eps: %.fig
	fig2dev -L eps $< $@

%.dvi: _tpsfiles _epsfiles $(TEXFILES)
	pdflatex $(FICHIER)
	if grep -q 'citation' $(FICHIER).aux; then if grep -q 'bibdata' $(FICHIER).aux; then bibtex $(FICHIER); fi else rm -f $(FICHIER).bbl; fi
	pdflatex $(FICHIER) > /dev/null
	pdflatex $(FICHIER) > /dev/null

_tpsfiles: $(PSDOTFILES)
	touch _tpsfiles

%.tps: %.dot
	dot -Tps -o $@ $<

_epsfiles: $(EPSFILES)
	@echo $(EPSFILES) > _epsfiles

clean:
	-rm -f $(EPSFILES) $(BACKFILES) $(PSDOTFILES)
	-rm -f $(TMPFILES)
	-rm -f $(TRUCFILES)
	-rm -f $(FICHIER).pdf

tar: clean
	perl -e '$$line=`date +"\%y-\%m-\%d"`;chomp($$line);`tar cvf $(FICHIER)-$$line.tar *`;`gzip $(FICHIER)-$$line.tar`;';

tardir: clean
	perl -e '$$pwd = `pwd`; my($$path,$$dir) = $$pwd =~ m/(.*\/)(.*)$$/; $$line=`date +"\%y-\%m-\%d"`;chomp($$line);`cd .. ; tar cvf $$dir-$$line.tar $$dir ; gzip $$dir-$$line.tar ; mv $$dir-$$line.tar.gz $$dir`;';

pwd:
	perl -e '$$pwd = `pwd`; print $$pwd;'

touch:
	@touch $(FICHIER).tex
	@echo You touch my ``$(FICHIER)''.

open:
#	@kile $(FICHIER).tex &
#	@texmaker $(FICHIER).tex &
	@emacs $(FICHIER).tex &





==> K-Robust Symmetry Breaking (4)/abstract.tex <==
\begin{abstract}
During Multi-Agent Path Finding (MAPF) problems, agents can be delayed
by unexpected events. To address such situations recent work describes
$k$-Robust Conflict-Based Search ($k$-CBS): an algorithm that
produces a coordinated and collision-free plan that is robust for up to $k$ delays for any agent. 
%
In this work we introduce a variety of pairwise 
symmetry breaking constraints, specific to $k$-robust planning, that can efficiently find
compatible and optimal paths for pairs of colliding agents. 
We give a thorough description of the new constraints and report
large improvements to success rate in a range of domains including:
(i) classic MAPF benchmarks, (ii) automated warehouse domains, and 
(iii) on maps from the 2019 Flatland Challenge, a recently introduced railway
domain where $k$-robust planning can be fruitfully applied to schedule trains.
%In recent years, several symmetric conflict reasoning algorithms
%were proposed to improve the efficiency of CBS-based algorithms, including
%rectangle reasoning, corridor reasoning and target reasoning.  In this
%work we show how to incorporate symmetric conflict reasoning approaches
%into $k$-Robust CBS and evaluate their performance on a variety of
%benchmark maps. The $k$-robust approach can also be used to solve problems
%with agents of fixed length, which occurs in train scheduling problems.
%We give experiments that show that symmetric conflict reasoning algorithms
%significantly improve the performance of $k$-robust CBS in the planning
%of $k$-robust solution, and in tackling train scheduling problems.
\end{abstract}


==> K-Robust Symmetry Breaking (4)/back.tex <==
Proof. Now let’s assume that there is a K-Delay conflict $<a_i, a_j,v, t, \Delta>$ with agent $a_i$ at timestep $t$ and $a_j$ at timestep $t+\Delta, \Delta \in [0, k]$. If $a_i$ and $a_j$ satisfy requirements, which means they all follow their Manhattan optimal paths, then:
\[t_j-t_i=\Delta\]
\[(|v.x-S_j.x|+|v.y-S_j.y|)-(|v.x-S_i.x|+|v.y-S_i.y|)=\Delta\]
\[|v.x-S_j.x|-|v.x-S_i.x|+|v.y-S_j.y|-|v.y-S_i.y|=\Delta\]
If $a_i$ and $a_j$ satisfy requirement b, which means they are moving towards the same direction, then:
\[(v.x-S_i.x)(v.x-S_j.x) \geq 0\]
\[(v.y-S_i.y)(v.y-S_j.y) \geq 0\]
Then, assume $a_i$ and $a_j$ are moving towards the direction that for any vertex $v_a$ in the optimal path of $a_i$ or $a_j$:
\[v_a.x-S_i.x\geq0,v_a.x-S_i.y\geq0\] or \[v_a.x-S_j.x\geq0,v_a.x-S_j.y \geq 0\]
As the problem is invariant with the rotations of direction, this assumption does not lose generality (Li et al., 2019b). 
Then:
\[(v.x-S_j.x)-(v.x-S_i.x)+(v.y-S_j.y)-(v.y-S_i.y) = \Delta\]
\[S_i.x-S_j.x+S_i.y-S_j.y = \Delta\]
for any intersection vertex $v’$ of optimal paths of $a_i$ and $a_j4$:
\[t_j' =|v'.x-S_j.x|+|v'.y-S_j.y|\]
\[t_i' =|v'.x-S_i.x|+|v'.y-S_i.y|\]
\[t_j'-t_i' =|v'.x-S_j.x|+|v'.y-S_j.y|-|v'.x-S_i.x|-|v'.y-S_i.y|\]
\[t_j'-t_i' =|v'.x-S_j.x|-|v'.y-S_i.x|+|v'.y-S_j.y|-|v'.x-S_i.y|\]
As $a_i$ and $a_j$ satisfy requirement $b$, then:
\[(v'.x-S_i.x)(v'.x-S_j.x) \geq 0\]
\[(v'.y-S_i.y)(v'.y-S_j.y) \geq 0\]
As $a_i$ and $a_j$ are moving towards the direction assumed above, Then
\[t_j' -t_i'=(v'.x-S_j.x)-(v'.y-S_i.x)+(v'.y-S_j.y)-(v'.x-S_i.y)\]
\[t_j' -t_i'=S_i.x-S_j.x+S_i.y-S_j.y \]
\[t_j' -t_i'=\Delta\]
As $\Delta \in [0, k]$, then $a_i$ and $a_j$ have a K-Delay conflict at $v’$.
If $a_i$ and $a_j$ also satisfy requirement c, then all optimal path of $a_j$ and $a_j$ always intersect within the rectangle area, and for any intersection vertex $v’$, $a_i$ and $a_j$ have a K-Delay conflict at $v’$. 
Thus, if $a_i$ and $a_j$ have a K-Delay conflict and satisfy all three requirements, $a_i$ and $a_j$ have K-Delay cardinal rectangle conflicts

==> K-Robust Symmetry Breaking (4)/background.tex <==
%\section{Background}
%\subsection{Problem Definition}
\section{Problem Definition}

We consider a multi-agent coordination problem where the operating
environment is an undirected (e.g. gridmap) or directed (e.g. rail network) 
graph $G=(V, E)$. We restrict graph $G$ to be a 4-neighbour grid and we
place upon it $m$ agents $\{a_{1}...a_{m}\}$. 
Every agent $a_i$ is assigned an initial vertex
$s_i$ and a goal vertex $g_i$.  
Time is discretised into unit-size steps. In each timestep, agents can move 
to an adjacent vertex or wait at the current location. Each move or wait
action has an associated unit cost.

We say that a path is $k$-robust if for each location $v$ visited at time $t$ by agent $a$ no other agent
visits the location in the time interval $[t, t+k]$.
We call a $k$-delay \emph{vertex conflict} the situation where agent
$a_i$ at timestep $t$ and $a_j$ at timestep $t'=t+\Delta, \Delta \in [0, k]$, 
visit the same location $v$. We denote such a conflicts 
by $\langle a_i, a_j, v, t, \Delta\rangle$.
%Notice that when $k >0$ we don't need a notion of \emph{edge conflict}, where two agents cross the same edge in opposite directions at the same time, since any edge conflict will result in a vertex conflict.
When $k=0$ it is further possible for two agents to cross the same edge in opposite directions at the same time, 
resulting in a so-called {\em edge conflict}. Notice however that with $k >0$ such a crossing will always 
result in a vertex conflict. Thus for $k>0$ we do not need to model edge conflicts.


A solution to the problem 
(equiv. a \emph{$k$-robust plan}) is a set of  
paths, one for each agent $a_i$, which moves each agent $a_i$ from its start location $s_i$ to its goal location 
$g_i$ such that there are no $k$-delay conflicts with the plans of any other agent.
Our objective is to find a $k$-robust plan which minimises the 
sum of all individual path costs (SIC).  

%If $a_i$ and $a_j$ traverse the same edge $(u,v)$ at same timestep $t$ in opposite
%directions, this is an \emph{edge conflict} $<a_i,a_j,u,v,t>$. 
%Notice that for $k > 0$ there are no \emph{edge coflicts},
%which otherwise appear in classic MAPF (i.e. cases where two agents attempt to 
%cross an edge from opposite directions at the same time).
%
%\subsection{Robustness of MAPF problem}
%
%In real-world applications,  unexpected events can cause delays when executing a plan. These delays prevent agents from following their plans, introducing extra conflicts and force agents to adjust their plans.  Currently, there are three approaches to overcome this problem.
%
%The first approach is to re-plan paths for all agents. However, all the agents need to wait until paths are re-planned, which makes this approach very expensive, sometimes even impossible~\cite{atzmon}.
%
%Some researchers have devised variations of robust plan-execution policies to solve this problem~\cite{ma2017,honig2019}.  Both~\cite{ma2017}  and~\citet{honig2019} introduce a synchronized robust plan-execution policy, which only allows an agent to move to its next vertex when all other agents finish the previous step’s actions. However, this approach causes agents to wait unnecessarily which results in a large overall plan cost. ~\citet{ma2017} propose a Minimal Communication Policy which enforces that any two agents always visit the same location in a specific order, based on the order in the original plan. Every agent needs to check whether another agent traverses its next vertex before itself. The agent then waits if the other agent should visit the next vertex first. This approach can reduce unnecessary waits and reduces the work amount of communications. However, many agents actions will be influenced by one agent's delay and it cannot guarantee the final cost if delays happened.
%~\citet{honig2019} proposed another method that uses a \emph{Action Dependency Graph} to keep track of all agents action state and one agent only can execute an action if depended actions of other agents are all complete. This approach also cannot guarantee the final cost if delays happened.
%\pjs{What about Honig 2017?}
%\mike{Honig 2017 is a typo. More info of honig 2019 added}
%
%
%A different, offline, approach is to develop a $k$-robust plan~\cite{atzmon}.
%The plan is developed so that if any agent is delayed for at most $k$ timesteps and the delayed agent can still follow its original plan without conflict with others. This approach handles delays in the planning stage and can guarantee the cost if agents are delayed by no more than $k$ timesteps. This paper
%Focuses on the planning of $k$-Robust approach to finding robust solutions to MAPF problems.
%


==> K-Robust Symmetry Breaking (4)/conclusion.tex <==
\section{Conclusions and Future Work}
This research introduces symmetry resolution methods for generating $k$-robust plans, which are vital for 
robust (e.g. warehouse robotics) and safe (e.g. railway scheduling) multi-agent plans. 
%
%We evaluate our algorithms on different types of game maps and %apply these algorithms to solve railway scheduling problems from %the Flatland challenge and MAPF problems on a warehouse map. 
Symmetry reasoning methods improve dramatically on K-CBS, with $k$-robust rectangle reasoning being the most important, 
while $k$-robust 
corridor 
%reasoning and $k$-robust
and target reasoning can further improve the performance. 
%
\ignore{
Future work crucially involves resolving the symmetric conflicts that can occur for $k\geq 2$  when two agents moving in the same direction in one dimension and the opposite direction in another dimension conflict. These conflicts 
occur fairly frequently and cause problems for $k$-CBS.
}

\section{Acknowledgments}

Research at Monash University was partially supported by the Australian Research Council under grants DP190100013, DP200100025 and also by a gift from Amazon.


==> K-Robust Symmetry Breaking (4)/experiments.tex <==
\section{Experiments}

The implementation is based on CBS with rectangle, corridor and target reasoning of \citet{corridor} and support for $k$-robust planning is added on top of it. It is programmed in C++ and experiments were performed on a server with AMD Opteron 63xx class CPU and 32 GB RAM. For each map, we keep increasing the number of agents, and for each number of agent we solve 25 different instances. The time limit is set to 90s for each instance. In result plots, K-CBS is the current state of art algorithm to plan $k$-robust plan proposed by \citet{atzmon},which is selected as the baseline, K-CBSH 
is our extension of K-CBS with heuristics (Section~\ref{sec:kCBS}),
RM adds $k$-robust Rectangle reasoning, 
C adds $k$-robust Corridor Reasoning, 
and T adds $k$-robust Target Reasoning. 


\subsubsection{Experiment 1: Game Maps}
The MAPF research community have developed a series of benchmark maps from games \cite{Stern2019}. They are available from movingai.com. We use 25 even scenarios from movingai.com to evaluate our algorithms.
%
We run experiments on following representative maps: \emph{Brc202d}, \emph{Den520d}, \emph{Random-32-32-10}, and \emph{Maze-128-128-1}. 

Figure \ref{fig7} shows the experiment results on grid game maps. K-CBSH-RM based algorithms shows significant higher success rate compared with K-CBS on \emph{Brc202d}, \emph{Den520d}, and \emph{Random-32-32-10}. Although $k$-robust corridor reasoning does not help on these three maps and $k$-robust target reasoning slightly helps, they effectively improves the success rate on \emph{maze-128-128-1}.
%
As $k$ increases, the problem becomes harder, and the success rate drops, but the symmetry-breaking algorithms still show significant advantages over K-CBS. 

\subsubsection{Experiment 2: Warehouse Map}
We use a \emph{31$\times$79 Warehouse map} \cite{corridor} with randomly generated problems to evaluate the performance of robots in warehouse system.
%
Figure \ref{fig7:sub5} shows that k-CBSH significantly improves success rate, $k$-robust target reasoning and corridor reasoning helps  to further improve the success rate of K-CBSH-RM.
%
Here target reasoning is clearly very important.

\subsubsection{Experiment 3: Simplified Railway System }

The Flatland challenge is a railway scheduling challenge \footnote{Swiss Federal Railways, 2019, Flatland Challenge. https://www.aicrowd.com/challenges/flatland-challenge} provides a simplified railway simulator using a directed grid map, where trains cannot move backwards. Railway systems have headway control, one train cannot start to enter a railway block if another train currently occupies
the block. Hence the railway domain requires $k=1$ robust plans.
Our experiments use flatland-rl v2.0.0 to generate experiment problems. 
Note, no target conflicts 
can occur in the Flatland challenge
scenarios since trains ``disappear'' when reaching their destination.

We have two settings for evaluation: (1) a \emph{100$\times$100 fixed dense map} contains fixed 140 start and goal locations, and each pair of start and goal are connected by 5 railways; and (2) a \emph{100$\times$100 incremental sparse map} has one start and goal location per agent, and each pair of start and goal are only connected by 1 railway.

The experiment on railway maps, Figure \ref{fig7:sub6} shows that K-CBSH and K-CBSH-RM performs substantially better than K-CBS. $k$-robust corridor reasoning helps further improve performance on sparse railways map.
Clearly the rectangle methods are more important on the denser map, where more symmetric conflicts are possible, and $k$-robust corridor reasoning is more important on sparse maps.

\subsubsection{Ratio of Rectangle Conflicts}

The Figure \ref{fig-rec-ratio} shows the percentage of $k$-delay rectangle conflicts among all resolved conflicts using K-CBSH-RM-C-T as $k$ increases. The statistics on conflicts are derived from Experiment 1 and Experiment 2. 
Clearly, as $k$ increases, the percentage of $k$-delay rectangle conflicts rises on the maps 
where rectangle conflicts can occur, hence the 
importance of $k$-robust rectangle reasoning is demonstrated. 

\begin{figure}
\centering
\includegraphics[width=0.8\columnwidth]{rectangle_ratio.png}
\caption{Percentage of $k$-delay rectangle conflicts among all conflicts as $k$ increases when using K-CBSH-RM-C-T.}
\label{fig-rec-ratio}
\end{figure}




==> K-Robust Symmetry Breaking (4)/figures.tex <==

\begin{figure*}[t]
\centering
\begin{subfigure}{1\textwidth}
  \centering
  \includegraphics[width=0.8\columnwidth]{legend.png}
\end{subfigure}
\begin{subfigure}{0.16\textwidth}
  \centering
  \includegraphics[width=\columnwidth]{plot32x32.jpg}
  \caption{Random 32x32}
  \label{fig7:sub1}
\end{subfigure}
\begin{subfigure}{0.16\textwidth}
  \centering
  \includegraphics[width=\columnwidth]{plotDen520d.jpg}
  \caption{Den520d}
  \label{fig7:sub2}
\end{subfigure}
\begin{subfigure}{0.16\textwidth}
  \centering
  \includegraphics[width=\columnwidth]{plotBrc202e.jpg}
  \caption{Brc202d}
  \label{fig7:sub3}
\end{subfigure}
\begin{subfigure}{0.16\textwidth}
  \centering
  \includegraphics[width=\columnwidth]{plotMaze.jpg}
  \caption{Maze 128x128}
  \label{fig7:sub4}
\end{subfigure}
\begin{subfigure}{0.16\textwidth}
  \centering
  \includegraphics[width=\columnwidth]{plotWarehouse.jpg}
  \caption{Warehouse map}
  \label{fig7:sub5}
\end{subfigure}
\begin{subfigure}{0.16\textwidth}
  \centering
  \includegraphics[width=\columnwidth]{plotFlatland.jpg}
  \caption{Flatland Railways}
  \label{fig7:sub6}
\end{subfigure}
\caption{Success rate versus number of agents on different problems.}
\label{fig7}
\end{figure*}

==> K-Robust Symmetry Breaking (4)/introduction.tex <==
\section{Introduction}
Multi-Agent Path Finding (MAPF) is a coordination problem
where we need to find collision-free paths for a team of
cooperating agents and is known to be NP-hard on graphs and grids \cite{yu2013structure,banfi2017intractability}.
When MAPF problems are solved in practice, agents can 
sometimes be unexpectedly delayed during plan execution; e.g. due 
to exogenous events or mechanical problems.
Currently, there exist two principal approaches to handle such delays.  
The first approach involves {\em robust execution policies}~\cite{ma2017multi,honig2019}.
Here dependencies are introduced to guarantee that agents execute their 
plans in a specific and compatible order.
Another approach is to reason about potential delays at the planning stage
which involves computing {\em robust plans}.

Following~\cite{atzmon} we say that a plan is $k$-robust if the individual 
path of each agent remains valid for up to $k$ unexpected delays of that 
agent. In other words, provided each agent waits for no more than $k$ timesteps
on the way to its target, its plan is guaranteed to be collision-free. 
In addition to their execution benefits, $k$-robust plans are valuable in
application areas where agents must maintain minimum safety distances.
Such constraints appear in rail scheduling, quay crane scheduling, planning for
warehouse robots and others. 
In these settings a $k$-robust plan naturally provides $k$ timesteps of 
distance between agents that are are moving, while also allowing agents to stay 
close if they are not moving. Furthermore, $k$-robust plans can be used in conjunction with \emph{robust execution policies} to benefit from both methods \cite{atzmon2020robust}.

To compute $k$-robust plans, \citet{atzmon} propose $k$-robust Conflict-Based
Search ($k$-CBS), a robust variant of the popular and well known branch-and-replan
strategy used for MAPF (where $k$ = 0)~\cite{sharon}, and a SAT-based solution, which cannot solve problems on large grids like brc202d DAO map\cite{Stern2019}.
A main problem with CBS is that the algorithm is extremely inefficient
when reasoning \emph{equivalent permutations} of conflicts that
can occur between pairs of agents, such as rectangle symmetry~\cite{li2019}, 
corridor symmetry, and target symmetry~\cite{corridor}.
%Furthermore, computing $k$-robust plans makes the resolving of rectangle conflicts extremely difficult. 
Further complicating the situation is that the reasoning techniques proposed
to handle these situations, do not always extend straightforwardly to the $k$-robust case.
\ignore{
especially those for {\em rectangle symmetries}, cannot
be easily extended to computing $k$-robust plans. 
}
\ignore{
In Section \ref{section:sym}, the paper illustrates $k$-robust rectangle
conflicts and why existing rectangle reasoning methods no longer work.
}

To address this gap in the literature we introduce a variety of specialised 
$k$-robust symmetry breaking constraints that dramatically improve performance
for the $k$-CBS algorithm.  Experimental results show very large gains
in success rate for $k$-CBS; not only on classic MAPF benchmarks but
also in two application specific domains: in \emph{warehouse logistics},
where $k$-robust plans are desirable and in \emph{railway scheduling}
where $k$-robust plans are mandatory.

\ignore{
\MikeNote{Talk about the situation that k-robust make rectangle more difficult. \textbf{Briefly here, more in section 4}\\
Agents get out and back. \textbf{In section 5}\\
Talk about,  safety distance. \textbf{Tick} \\
Example of k=4 which makes the problem much complicated and much more flex. \textbf{In Section 5}}
}


==> K-Robust Symmetry Breaking (4)/k_cbs.tex <==
\section{$k$-Robust Conflict-Based Search}\label{sec:kCBS}
\begin{figure}
\centering
\begin{subfigure}{0.4\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth]{rectangle_small.png}
  \caption{Rectangle}
  \label{fig2:sub0}
\end{subfigure}
\begin{subfigure}{0.43\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth]{corridor.jpg}
  \caption{Corridor}
  \label{fig2:sub1}
\end{subfigure}
\begin{subfigure}{0.5\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth]{target.jpg}
  \caption{Target}
  \label{fig2:sub2}
\end{subfigure}
\caption{Examples of rectangle, corridor and target conflicts when $k$=0, reproduced from~\cite{corridor}. }
\label{fig2}
\end{figure}

$k$-Robust Conflict-Based Search ($k$-CBS)~\cite{atzmon} is a two-level search 
algorithm specialised from classical MAPF ($k$=0)~\cite{sharon}. 
At the high-level, $k$-CBS searches (in a best-first way) a binary
constraint tree ($CT$) where each  node is a complete assignment of paths to agents (i.e. a plan).  
The process of finding such single agent paths constitutes the low level 
of $k$-CBS. Here individual agents find paths (via A*) from 
start to target while subject to a set of collision-avoiding 
\emph{constraints}. 
%The process finishes when a feasible $k$-robust plan is discovered.


%If the proposed plan is invalid, i.e. there exists a
%collision between two agents, CBS \emph{branches} the plan and generates two
%new candidate plans: each the result of re-planning one of the colliding
%agents. 
%Each constraint is a tuple $\langle a_i,
%v, t \rangle$ which says that $a_i$ is forbidden from occupying location
%$v$ at timestep $t$.  Constraints are added branching and they serve to
%force each agent to find a new path: one which avoids the conflict area.
%Each branching plan inherits the constraints of its predecessor and the
%high-level search continues until it expands a node which is conflict
%free. Such a node is a goal node and the search terminates.

%CBS’s high-level generates a binary constraint tree
%($CT$). Each node ($N$) of the $CT$ has a set of constraints that are
%applied to agents. 
%%A vertex constraint is denoted by a tuple $<a_i, v, t>$,
%%which means agent $a_i$ cannot occupy vertex $v$ at timestep $t$.  An edge
%%constraint is denoted by a tuple $<a_i, u, v, t>$ meaning that agent $a_i$
%%cannot use the edge from $u$ to $v$ at timestep $t$.  
%A node $N$ in the $CT$
%also includes a solution which satisfies all constraints, and the cost of
%a solution is the sum of individual path costs of all agents. The root
%node of the $CT$ contains the empty set of constraints. The high-level
%search performs a best-first search on the constraint tree. The low-level
%search uses A* algorithm to search for shortest paths for an agent that
%can satisfy all the constraints of the current node on that agent.

The search process of $k$-CBS proceeds as follows:
At each iteration $k$-CBS expands the CT node with lowest $f$-cost. 
If the current node is conflict-free then that node is a goal and 
the search terminates having found a least-cost feasible plan.  
Otherwise, the current node must contain at least one pair of agents 
that are in collision.
%To resolve the impasse $k$-CBS {\em splits} the node, thereby generating 
%two new CT nodes. In each successor we replan one of the agents,
%subject to collision-avoiding constraints. 
Suppose for example that the conflict is $\langle a_i, a_j, v, t, \Delta\rangle$.
%Then, $k$-CBS adds the constraint 
%$<a_i,
%v, t>$ to one child node and constraint $<a_j, v, t>$ to another node.
%Each constraint says that agent $a_i$ (resp. $a_j$) cannot occupy 
%vertex $v$ at timestep $t$.  
%
%
%In \citet{atzmon} a related algorithm, \textbf{$k$-CBS}, is developed to compute
%$k$-robust plans.  Similar to CBS, this algorithm proceeds by resolving
%so-called $k$-delay conflicts of the type $<a_i, a_j, v, t, \Delta>$ .
This situation occurs when agent $a_i$ at timestep $t$ and $a_j$ at
timestep $t' = t+\Delta, \Delta \in [0, k]$, visit the same location $v$.
To resolve the conflict $k$-CBS re-plans each of the two affected agents and 
thus generates two new candidate plans. To each child node is added a 
\emph{time range constraint} which resolves the situation now and in 
all future descendant nodes derived from each respective child.
The constraint \mbox{$\langle a_i, v, [t,t+k]\rangle$} says that
agent $a_i$ is not allowed to occupy vertex $v$ at any timestep in the 
range $[t,t+k]$.  The second child node, where $a_j$ is replanned, 
receives a similar constraint: $\langle a_j, v, [t,t+k]\rangle$.

$k$-CBS continues in this way, splitting and searching, 
while the current CT node contains any conflict.
This approach is solution complete and optimal. It guarantees to 
find a $k$-robust plans~\cite{atzmon}, if any such plan exists,
since the union of valid plans permitted by the two child 
nodes is the same as at the parent node
(i.e. adding constraints does not eliminate valid solutions).

\textbf{Conflict selection strategies: }
%\pjs{Add definition of cardinal, semi-cardinal, and non-cardinal conflicts here for CBS}
%\mike{Defination added}
Deciding which conflict to resolve next is critical to the success 
of ($k$-)CBS. 
In this work we follow \citet{boyarski2015} where authors classify conflicts as 
\emph{cardinal}, \emph{semi-cardinal} and \emph{non-cardinal}:
%In \citet{li2019} a more general definition is given:
\begin{itemize}
    \item A conflict C is \emph{cardinal} if replanning for any agent involved in the conflict increases the SIC.
    \item A conflict C is \emph{semi-cardinal} if replanning for one agent involved in the conflict always increases the SIC while replanning for the other agent does not.
    \item A conflict C is \emph{non-cardinal} otherwise.
    %, if it is not \emph{cardinal} or \emph{semi-cardinal}.
\end{itemize}
In \citet{boyarski2015} it is shown that resolving cardinal conflicts first can dramatically reduce the size of the resulting CBS tree.
After all cardinal conflicts are resolved we choose semi-cardinal conflicts and finally non-cardinal.
Similar to that work we use a Multi-valued Decision Diagram (MDD) to classify conflicts. 
Each MDD records all nodes (i.e., vertex-time pairs) that can appear on an optimal path 
for each agent. (Semi-)cardinal conflicts require the conflict node to be a \emph{singleton} 
for (resp. one) both agents, i.e. all optimal paths must pass through the node. 

\textbf{CBS Heuristics (CBSH): }
Different from~\cite{atzmon} but following~\cite{CBSH}, we also exploit known cardinal conflicts 
to derive a \emph{minimal cost increase} heuristic for our high-level A* search. This strategy is known to 
improve the performance of CBS and has become a common approach in leading MAPF ($k$ = 0) solvers.
%\citet{CBSH} showed that it was important to resolve cardinal conflicts first, this could dramatically reduce the size of the resulting CBS tree.
%We can also use cardinal conflicts to add define a \emph{minimal cost increase}
%heuristic for the high-level A* search.  This can avoid exploring many high-level nodes and is now universally used in CBS search.
%
%\citet{atzmon} developed $k$-CBS to create $k$-robust plans.  
%$k$-CBS creates these plans resolving $k$-delay conflicts.
%A $k$-delay vertex conflict $<a_i, a_j, v, t, \Delta>$ 
%occurs when agent $a_i$ at timestep $t$ and $a_j$ at timestep $t'$ 
%where $t+\Delta, \Delta \in [0, k]$, visit the same location. 
%Edge conflicts are not necessary for $k$-CBS when $k > 0$ since any edge conflict will also result in a $k$-delay vertex conflict. 
%
%
%In order to resolve this conflict~\citet{atzmon}
%introduce the time range vertex constraint
%$<a_i, v, [t,t+k]>$ which disallows agent
%$a_i$ from visiting vertex $v$ at any timestep in the range $[t,t+k]$.
%\ignore{
%Similarly we have the time range edge constraint 
%$<a_i, u, v, [t,t+k]>$ which disallows agent
%$a_i$ from using edge $(u,v)$ at any timestep in the range $[t,t+k]$.
%$k$-CBS uses a pair of symmetric range constraints to resolve
%a $k$-delay conflict. For example to resolve a $k$ delay vertex conflict
%$<a_i, a_j, v, t, \Delta>$ it will add constraint
%$<a_i, v, [t,t+k]>$ to one child and
%$<a_j, v, [t,t+k]>$ to the other child.  \pjs{CHECK!}
%}
%>>>>>>> bce2f2816fe03fbc7161d3dc972301a9f1f9836e


==> K-Robust Symmetry Breaking (4)/k_symmetries.tex <==
\section{$k$-Robust Rectangle Reasoning}

%$k$-Robust rectangle conflicts occur when 
%two agents arrive in a rectangle area such as Figure~\ref{fig1} (left);
%not just at the same time but also within $k$ timesteps of one another.
The simplest type of rectangle conflict, called CR in~\cite{li2019},
can be understood as follows:
\begin{itemize}
\item[(a)] Both agents follow their Manhattan optimal paths from start to goal. 
\item[(b)] Both agents move in the same direction in all dimensions.
\item[(c)] The start and goal nodes of two agents have relative opposite locations. This requirement ensures that all optimal paths of both agents intersect within the rectangle area.
\end{itemize}

The situation is shown in Figure~\ref{fig1} (left). The only difference between $k$-delay rectangle conflicts and 
$k=0$ is that the agents can arrive at the same vertex in the rectangle area at different timestep. 
To resolve such conflicts we introduce \textbf{Temporal Barrier Constraints}, which unify
the (temporal) range constraints of~\cite{atzmon} and the (spatial) Barrier Constraints of~\cite{li2019}.

%Thus if two agents have a $k$-delay conflict satisfy requirements (a), (b), and (c), they have $k$-delay cardinal rectangle conflicts.

%\subsection{Temporal Barrier Constraints}

%We combine the concept of symmetry range constraint \citet{atzmon} and barrier constraint\citet{li2019} to resolve $k$-delay rectangle conflicts. This new constraint is called the \emph{temporal barrier constraint}.

\begin{defn}
Given a vertex time pair p = (S,t) the \emph{optimal time} 
$ot(p,v)$ to reach 
vertex $v = (v_x,v_y)$ starting from $S = (S_x,S_y)$ at time $t$ is
calculated by adding the Manhattan distance 
$ot(p,v) = t + |v_x - S_x| + |v_y - S_y|$.

A \emph{temporal barrier constraint} is denoted by
$B(a_x, V, p, \Delta)$. 
This constraint forbids the 
agent $a_x$ from visiting any vertex $v \in V$ 
at the optimal time from vertex time pair $p$, or any time step up to $\Delta$ later. 
That is the barrier constraint $B(a_x, V, p, \Delta)$ 
is the set of time-range vertex constraints
$\langle a_x, v, [ot(p,v), ot(p,v) + \Delta] \rangle, v \in V$.
\label{defi:barrier}
\end{defn}

%Figure~\ref{mike-fixme} shows an example. 
Figure~\ref{fig3}(b) shows the example that $a_i$ is blocked by temporal barrier constraint and does not have a $k$-delay conflict anymore.
\ddh{Mike, please fix this example. The diagram should be one picture showing a k-delay conflict and a temporal barrier}\mike{got it}
%Here $a_i$ and $a_j$ have a conflict $(a_i, a_j, v, t, \Delta)$, meaning $a_i$ arrives at $v$ at timestep $t$ and $a_j$ arrives at $v$ at timestep $t+\Delta$. We resolve this conflict with temporal barrier constraints 
%$B(a_i, R_i, R_g, k,0)$ and $B(a_j, R_i, R_g, k,\Delta)$.  

\subsection{Extended Rectangle Area}

\begin{figure}
\centering
\begin{subfigure}{0.48\columnwidth}
  \centering
  \includegraphics[width=0.9\columnwidth]{rectangle.jpg}
  \caption{Rectangle Conflict}
  \label{fig4:sub1}
\end{subfigure}
\begin{subfigure}{0.48\columnwidth}
  \centering
  \includegraphics[width=0.9\columnwidth]{extendedb.jpg}
  \caption{Temporal barrier constraint use start-goal rectangle border eliminate all conflicts and orange area}
  \label{fig4:sub2}
\end{subfigure}
\caption{Extended rectangle area and temporal barrier constraint when k=2. Red numbers are timesteps that $a_j$ reach each vertex. Green numbers for $a_i$. Grey cells are constrained vertexes with constrained timesteps. Orange and yellow area means all paths will conflict in these area. For unconstrained agents these numbers are optimal time they can arrive each location. For constrained agents, numbers are latest time they can reach each vertex.   }
\label{fig4}
\end{figure}

The aim of introducing a temporal barrier constraint is to force the optimal cost of constrained agent to increase by $1+k-delay$. 
However, when $k \geq 2$, the temporal barrier constraint with $B(a_x, R_x, R_g, k, delay)$ failed. As shown in Figure \ref{fig4:sub1}, when $k=2$, temporal barrier constraint $B(a_i,(4,4),(4,5),2,0)$ is used to force $a_i$’s optimal path to increase by 3, to a length of 9, to avoid the conflict with $a_j$. 
However, the cost of optimal paths of agent $a_i$ is still 8, 
because $a_i$ can bypass the temporal barrier constraint. In this case, all paths of $a_i$ with cost 8 conflict with all the optimal paths of $a_j$ in the light yellow area, which is larger than the rectangle. 

The light yellow area is an extended rectangle area. Each time $k$ increased by 2, constrained agent need to find a path with 2 more cost. This makes CBS can choose a wider path with 2 more cost that bypass rectangle area, which means the size of the extended rectangle area increased.

Once $k$ is big enough to force the agent to bypass the unconstrained agent’s start-goal rectangle, the optimal path of constrained agents will no longer intersect with unconstrained agent’s optimal path. Thus the extended rectangle area is at most the unconstrained agent’s start-goal rectangle. 

\subsection{$k$-Robust Cardinal Rectangle Reasoning}

One approach to overcome the above problem is to use the border of the extended rectangle area to define a temporal barrier constraint. 
We use a simpler method which extends the border of unconstrained agent’s start and goal rectangle as the barrier in order to to overcome this problem. Figure \ref{fig4:sub2} shows the latest timestep that $a_i$ can arrive at each vertex in the rectangle area when trying to reach the goal at timestep 9. 
In this case, the low-level search of $a_i$ has many options for reaching 
the goal at timestep 9 without conflicting with the optimal paths of agent $a_j$.  Figure \ref{fig4:sub3} shows the CT tree when solving rectangle conflicts with temporal range constraints. We denote the temporal barrier constraint using the border of unconstrained agent’s start and goal rectangle as $B(a_x, Rs_x, Rg_x, k, delay), x \in [ i, j ]$. 
$Rs_x$ and $Rg_x$ are the two corner nodes of the border of the start-goal rectangle that are opposite to $a_x$’s start location $s_x$. 
We call the algorithm using the extended
temporal border constraint $B(a_x, Rs_x, Rg_x, k, delay), x \in [ i, j ]$ to resolve $k$-delay cardinal rectangle conflict as \textbf{K-CBSH-CR}.

Using the border of unconstrained agent’s start and goal rectangle will introduce some redundant constraints. But they do not over constrain the target agent. Using the example in Figure \ref{fig4:sub2}, if the $k=2$ and 
vertex (4,2) is constrained at timesteps 1, 2, and 3, since the earliest timestep that the constrained agent can arrive at (4,2) is 5 this does remove any possible paths for the agent.
Similarly while vertex (6,7) is constrained at timesteps 6, 7, and 8; paths for $a_i$ to reach the goal through (6,7) have a cost of at least 10, and hence no possible paths are removed. 

\textbf{Property 1.} For any path combination of two agents $a_i$ and $a_j$ that have $k$-delay cardinal rectangle conflict (assuming $a_i$ arrives rectangle area $\Delta$ timestpes early than $a_j$). If one path violates $B(a_i, Rs_i, Rg_i, k,0)$ and the other path violates $B(a_j, Rs_j, Rg_j, k,\Delta)$, then the two agents have $k$-delay conflict within the rectangle area.

\textit{Proof.} 
If the optimal time that agent $a_i$ can arrive vertex $N_i$ on border $Rs_i$ to $Rg_i$ is $c_i$.  Now $a_i$ arrives at $N_i$ at $t_i$, $c_i \leq t_i \leq c_i+k$ and $d_i=t_i-c_i$ ($d_i$ is the timestep difference between the timestep that $a_i$ arrive $N_i$ and the optimal timestep that $a_i$ can arrive $N_i$), hence $a_i$ violates constraint $B(a_i, Rs_i, Rg_i, k,0)$.

If the optimal time that agent $a_j$ can arrive vertex $N_j$ on border $Rs_j$ to $Rg_j$ is $c_j$ and the optimal time that agent $a_i$ can arrive vertex $N_j$ is $c_{i\_nj}$. Hence the timestep difference that two agents optimally arrive a vertex in rectangle area is $\Delta$, $c_{i\_nj} + \Delta = c_j$ and $c_{i\_nj}\leq c_j$. 
Now the $a_j$ arrive $N_j$ at $t_j$, and $c_{i\_nj}\leq c_j\leq t_j\leq c_j-\Delta + k = c_{i\_nj}+k$, hence $a_j$ violate $B(a_j, Rs_j, Rg_j, k,\Delta)$. $d_j=t_j-c_j$, which is the timestep difference between $t_j$ and $c_j$.

The requirement (c) in section 5.1 guarantees that the path of $a_i$ and the path of $a_j$ must have an intersect vertex, which means they both traverse a vertex at same or different timestep. The intersection vertex in denoted as $v$. 

The optimal time that $a_i$ arrive $v$ is $c_{i\_v}$, which is also the earliest time that $a_i$ can arrive $v$. 

The optimal time that $a_j$ can arrive $v$ is $c_{j\_v}$ and the latest time that $a_j$ can arrive $v$ is $c_{j\_v}+d_j$. 

As agent $a_i$ and $a_j$ have $k$-delay rectangle conflicts and the optimal path of $a_i$ arrive rectangle area early than $a_j$, thus $c_{j\_v}-c_{i\_v}=\Delta$ and $\Delta \leq k$. 

Because $t_j\leq c_{i\_nj}+k$:
\[t_j-c_j\leq c_{i\_nj}+k-c_j\]
\[d_j\leq c_{i\_nj}+k-c_j\]
As $a_i$ and $a_j$ have $k$-delay rectangle conflicts, the time difference that two agents' optimal path arrive any vertex in rectangle conflicts is $\Delta$ and also because of $c_{i\_nj}\leq c_j$:
\[d_j\leq -\Delta+k\]
\[d_j+\Delta\leq k\]
Thus 
\[d_j+c_{j\_v}- c_{i\_v} \leq k\]
Hence $d_j+c_{j\_v}$ is the latest time that $a_j$ can arrive vertex $v$ and $c_{i\_v}$ is the earliest time that $a_i$ can arrive $v$, the time difference between the latest time that $a_j$ can arrive $v$ and the earliest time that $a_i$ can arrive $v$ is always smaller than k, which means have a $k$-delay conflict between $a_i$ and $a_j$ at $v$.

Therefore if $a_i$ and $a_j$ have $k$-delay rectangle conflicts, one path violates $B(a_i, Rs_i, Rg_i, k,0)$ and the other path violates $B(a_j, Rs_j, Rg_j, k,\Delta)$, then the two agents have $k$-delay conflict within the rectangle area.
\qed

\mike{Sketch of proof}
\textit{Proof Sketch.} 
The requirement (c) in section 5.1 guarantees that the path of $a_i$ and the path of $a_j$ must have an intersect vertex $v$ if both agents traverse each other's start and goal rectangle. 

Assuming the optimal time that agent $a_i$ can arrive vertex $N_i$ on border $Rs_i$ to $Rg_i$ is $c_i$ and the real time $a_i$ arrives at $N_i$ is $t_i$, $c_i \leq t_i \leq c_i+k$ and $d_i=t_i-c_i$.

Assuming the optimal time that agent $a_j$ can arrive vertex $N_j$ on border $Rs_j$ to $Rg_j$ is $c_j$ and the optimal time that agent $a_i$ can arrive vertex $N_j$ is $c_{i\_nj}$. Hence the timestep difference that two agents optimally arrive a vertex in rectangle area is $\Delta$, $c_{i\_nj} + \Delta = c_j$ and $c_{i\_nj}\leq c_j$. Assuming the real time the $a_j$ arrive $N_j$ is $t_j$, $c_{i\_nj}\leq c_j\leq t_j\leq c_j-\Delta + k = c_{i\_nj}+k$, and $d_j=t_j-c_j$.

Assuming the optimal time (earliest time) that $a_i$ can arrive $v$ is $c_{i\_v}$. 

Assuming optimal time that $a_j$ can arrive $v$ is $c_{j\_v}$, the latest time that $a_j$ can arrive $v$ is $c_{j\_v}+d_j$. 

As $a_i$'s optimal path have $k$-delay conflict with $a_j$'s optimal path, we know $c_{j\_v}-c_{i\_v}=\Delta$.

With these information, we can prove that $c_{j\_v}+d_j - c_{i\_v}$ always smaller than k, which means we have a $k$-delay conflict at $v$.
\qed


\subsubsection{Theorem 1.} K-CBSH-CR is complete and optimal.

\textit{Proof.}  The proof is similar to the proofs in \citet{atzmon} and \citet{li2019}.  
If $a_i$ and $a_j$ have a conflict $(a_i, a_j, v, t, \Delta$. For a CT node $N$, $N1$ and $N2$ are the child nodes for $N$. $N1$ hold the constraint $B(a_i, Rs_i, Rs_i, k,0)$ and $N2$ hold the constraint $B(a_j, Rs_j, 
Rs_j, k,\Delta)$. $\pi(N1)$ denotes all the $k$-Robust plans that satisfy $N1.constraints$ and $\pi(N2)$ denotes all the $k$-Robust plans that satisfy $N2.constraints$. Based on property 1, the temporal barrier constraint does not eliminate any conflict-free solutions. Thus $\pi (N) =  \pi (N1) \cup \pi (N2)$. Thus K-CBSH-CR does not eliminate any possible solution and is complete. Furthermore, the low-level search of any kind of CBS always returns an optimal path, the high-level search always chooses a CT node with minimum $f$-value to expand and K-CBSH-CR does not eliminate any possible solution when splitting. Therefore, the first chosen CT node whose paths are conflict-free has a set of conflict-free paths with minimum cost. Thus K-CBSH-CR is optimal.
\qed

\subsection{Extending $k$-Robust Rectangle Reasoning}

\citet{li2019} shows that rectangle reasoning can also be used to resolve semi-cardinal rectangle conflict and non-cardinal rectangle conflicts, not only cardinal rectangle conflicts. This algorithm is called CBSH-R. As the 
barrier constraints only block paths that traverse the rectangle area and do not block all optimal paths for semi-cardinal or non-cardinal rectangle conflicts, it may fail to resolve some conflicts. CBSH-R needs to esnure 
the barrier constraint resolves the current conflict so that it cannot
arise in the current node’s ancestors.  By replacing the barrier constraint with a temporal barrier constraint using the border of the unconstrained agent’s start-goal rectangle, CBSH-R is modified to plan $k$-Robust solutions and we denote this algorithm \textbf{K-CBSH-R}. 

\textbf{Theorem 2.} K-CBSH-R is complete and optimal.

\textbf{Proof.} As temporal barrier constraint for $a_i$ will not block any path that does not traverse $a_j$’s start goal rectangle, thus temporal barrier constraint for $a_i$ will not block any path that does not intersect with $a_j$’s path. Therefore Property 1 still holds for K-CBSH-R. Thus the proof in Theorem 1 still works for K-CBSH-R, which means K-CBSH-R also is complete and optimal. \qed

\subsubsection{Rectangle Conflict in Path Segments}
\citet{li2019} further extends the usage of barrier constraints and use it to solve rectangle conflicts caused by obstacles and other constraints. It uses a Multi-Valued Decision Diagram (MDD) (Sharon et al. 2013), which is a directed acyclic graph, to find singletons in the paths of each agent. An MDD stores all possible locations at each timestep for an agent to reach its goal optimally, which is the same as storing all optimal paths of an agent. If a timestep only has one possible location, which means all optimal paths must traverse this location at this timestep, this location at this time step is called a singleton. This algorithm uses all the singletons from conflict agents’ paths as candidate start and goal locations and then CBSH-RM try to find and classify rectangle conflicts in all possible start and goal combinations. When multiple conflicts exist, CBSH-RM first prefers rectangle conflicts with higher priority type, then it prefers a larger rectangle area. 

For $k$-delay rectangle conflicts, current conflict detection tie braking policy cannot efficiently resolve all problems, as the rectangle conflicts does not consider extended rectangle area. Thus, for $k$-Robust plan, the rectangle conflicts with larger extended rectangle area are preferred when two rectangle conflicts have the same priority type and rectangle area.\

\subsubsection{Adding Temporal Barrier Constraint}
\citet{li2019} also find that if blocking all vertexes on the border of the rectangle opposite the constrained agent, CBSH-RM may lose optimality. Because when barrier constraint force the agent to reach the goal with a higher cost, it is possible that alternative paths, which do not traverse selected start singleton but traverse constrained barrier vertexes. Blocking all vertexes on the border of the rectangle area loses these path choices. By using MDD for each agent in conflict, CBSH-RM avoid losing optimality by checking does any optimal path of constrained agent traverse the vertexes included in barrier constraint and if no any optimal path traverse a vertex, this vertex will not be constrained.

$k$-Robust rectangle reasoning requires to block the extended rectangle area as well. Although the MDD provides the information of all optimal paths of an agent, these optimal paths do not traverse extended rectangle area. Therefore, if the optimal cost from selected start singleton to selected goal singleton is $c$, an MDD of constrained agent stores all paths from selected start singleton to selected goal singleton with a cost of $c+k$ is used to support the adding of temporal barrier constraint. An MDD with the cost of $c+k$ contains all paths with cost $i,  c\leq i \leq c+k$, as a path with cost i can become a path with cost c+k by waiting at goal location.

For any vertex $v$ in the border of extended rectangle area opposite to constrained agent, if the optimal time that the agent arrives at the vertex is $t$ , the time that the agent arrive selected start singleton is $t_s$, and the level $(t-t_s) +i,i\in (0,k)$, of the MDD include vertex $v$, $v$ is constrained from time $t+i$ to $t +k$. By constraint the vertexes only exist in MDD Property 1 still holds here. This algorithm is denoted as K-CBSH-RM.

\mike{A shorten version:} \citet{li2019} shows that rectangle reasoning can also be used to resolve semi-cardinal rectangle conflict and non-cardinal rectangle conflicts, not only cardinal rectangle conflicts. By replacing the barrier constraint with a temporal barrier constraint, it is modified to plan $k$-Robust solutions and we denote this as \textbf{K-CBSH-R}. \citet{li2019} further extends the usage of barrier constraints and use it to solve rectangle conflicts caused by obstacles and other constraints. It uses a Multi-Valued Decision Diagram (MDD) (Sharon et al. 2013), which is a directed acyclic graph, to find singletons in the paths of each agent. An MDD stores all possible paths of an agent at a certain cost. If a timestep only has one location, which means all paths traverse this location at this timestep, it is called a singleton. This algorithm uses all the singletons from conflict agents’ paths as candidate start and goal locations and then CBSH-RM try to find rectangle conflicts in all possible start and goal combinations. By replacing barrier constraint with temporal constraint, it works for planning $k$-robust solution and is denoted as \textbf{K-CBSH-RM}.



\section{$k$-Robust Corridor Reasoning}
The difference between corridor conflict with $k$-Robust CBS and normal corridor conflict is that agents need to occupy vertexes for extra timesteps to avoid $k$-delay conflicts. Assume there is a corridor conflict with a length of $l$ between vertex $b$ and vertex $e$. Agent $a_1$ moving from $b$ to $e$ and agent $a_2$ moving from $e$ to $b$. If the agent $a_1$ reach vertex $e$ at timestep $t_1$ and agent $a_2$ reach vertex $b$ at timestep $t_2$.For planning $k$-Robust solution, any path of $a_1$ that reach vertex $e$ at or before timestep $t_2+l+k$ must conflict with any paths of $a_2$ that reach vertex $b$ at or before timestep $t_1+l+k$.

When considering bypasses, assuming agent $a_1$ can reach vertex $e$ at timestep $t'_1$ and agent $a_2$ reach vertex $b$ at timestep $t'_2$ without traverse the corridor. Therefore for planning $k$-Robust solution, any path of $a_1$ that reach vertex $e$ at or before timestep $min(t'_1  - 1+k,t_2  + l+k)$ must conflict with any paths of $a_2$ that reach vertex $b$ at or before timestep $min(t'_2  - 1+k,t_1  + l+k)$.

Therefore, a pair of range constraint is used to perform $k$-Robust corridor reasoning. When splitting CT node, child node 1 hold the constraint $<a_1,e,[0,min(t'_1  - 1+k,t_2  + l+k)]>$ and child node 2 hold the constraint $<a_2,b,[0,min(t'_2  - 1+k,t_1  + l+k)]>$.

\textbf{Theorem 2.} $k$-Robust Corridor Reasoning is complete and optimal.

\textit{Proof} We have shown that if $a_1$ and $a_2$ both violate constraint $<a_1,e,[0,min(t'_1  - 1+k,t_2  + l+k)]>$ and constraint $<a_2,b,[0,min(t'_2  - 1+k,t_1  + l+k)]>$, they must have a conflict in the corridor. Thus the adding of these constraints will not eliminate any conflict free $k$-Robust solution. Thus $k$-Robust Corridor Reasoning is complete. $k$-Robust Corridor Reasoning is based on CBS, as proved in Theorem 1, CBS guarantees that the solution is optimal as long as no conflict free solution is eliminated.

\section{$k$-Robust Target Reasoning}
Assuming that agent $a_i$ reaches its goal $g_i$ on timestep $l$, and agent $a_j$ has a target conflict with the agent $a_i$ at $g_i$ on timestep $t,t \geq l$. All solutions that both $a_i$ and $a_j$ visit $g_i$ at $t$ must have conflict. ~\citet{corridor} resolve target conflict by force $a_i$ to reach its goal after $t$ or force any other agent visit $g_i$ at or after $t$. Planning $k$-Robust solution requires the avoiding of $k$-delay conflict. Therefore, when splitting, one child node forces $a_i$ to reach its goal after $t+k$ to give $a_2$ priority and do not cause $k$-delay conflict. Another child node forbids any other agent visit $g_i$ at or after $t$ to force all other agents find bypasses to their goal locations. If any agent failed to find a bypass route, we do not generate this child node. 

\textbf{Theorem 3.} $k$-Robust Target Reasoning is complete and optimal.

\textit{Proof} We have shown that target reasoning only eliminate the solutions that have target conflict and do not eliminate any conflict free solution. Thus $K$-robust Target Reasoning is complete. $k$-Robust Target Reasoning is based on CBS. As proved in Theorem 1, CBS guarantees that the solution is optimal as long as no conflict free solution is eliminated.

%%%%%%%%% OLD OLD OLD OLD  %%%%%%%%%%%%%%%%%%%%%
%\subsection{Identifying $k$-delay Cardinal Rectangle Conflicts}
%
%\citet{li2019} introduced an algorithm to identify cardinal rectangle conflicts for CBSH-CR. If agent $a_i$ and $a_j$ have a conflict $<a_i, a_j, v, t>$, $S_i$, $G_i$ are start and goal nodes for $a_i$ and $S_j$, $G_j$ are start and goal nodes for $a_j$, 
%if they satisfy following requirements, they have cardinal rectangle conflict. Requirements are:
%\begin{itemize}
%\item[(a)] Both agents follow their Manhattan optimal paths from start to goal. 
%\item[(b)] Both agents move in the same direction in all dimensions.
%\item[(c)] Start and goal nodes of two agents have relative opposite locations. This requirement ensures that all optimal paths of both agents intersect within the rectangle area.
%\end{itemize}
%The only difference for $k$-delay rectangle conflicts is that the 
%agents can arrive at the same vertex in the rectangle area at different timestep. Thus if two agents have a $k$-delay conflict satisfy requirements (a), (b), and (c), they have $k$-delay cardinal rectangle conflicts.
%
%\subsection{Temporal Barrier Constraints}
%\begin{figure}
%\centering
%\begin{subfigure}{0.48\columnwidth}
%  \centering
%  \includegraphics[width=1\columnwidth]{rectangle.jpg}
%  \caption{Rectangle Conflict. }
%  \label{fig3:sub1}
%\end{subfigure}
%\begin{subfigure}{0.48\columnwidth}
%  \centering
%  \includegraphics[width=0.98\columnwidth]{temporalBarrier.jpg}
%  \caption{Temporal barrier constraints for $a_i$. }
%  \label{fig3:sub2}
%\end{subfigure}
%\caption{Examples of rectangle conflicts and barrier constraints when k=1. The green numbers are timesteps that agent $a_i$ reach each vertex. The red numbers are timesteps that $a_j$ reach each vertex. Grey cells are constrained vertexes and black numbers are constrained timesteps for constrained vertexes. Orange area means all paths will conflict in this area. For unconstrained agents these numbers are optimal time they can arrive each location. For constrained agents, numbers are latest time they can reach each vertex.}
%\label{fig3}
%\end{figure}
%
%We combine the concept of symmetry range constraint \citet{atzmon} and barrier constraint\citet{li2019} to resolve $k$-delay rectangle conflicts. This new constraint is called the \emph{temporal barrier constraint}.
%
%\textbf{Definition 1}  A  \emph{temporal barrier constraint} is denoted by $B(a_x, R_x, R_g, k, delay), x \in [ i, j ]$. It forbids the agent $a_x$ from visiting any vertex $v_n$ within $R_x$ to $R_g$ area (the rectangle area border that is opposite to $a_x$) from timestep $t - delay$, where $t$ is the earliest time that agent $a_x$ can arrive vertex $v_n$, to timestep $t-delay + k$. The variable $delay$ is used to note the timestep difference between agents in the $k$-delay conflict. For the agent (say $a_i$) that arrives rectangle first, $delay = 0$. For the agent (say $a_j$) arrives rectangle second, $delay$ is the timestep difference that agents arrive at conflict vertex $v$.
%
%Assume $a_i$ and $a_j$ have a conflict $(a_i, a_j, v, t, \Delta)$, meaning $a_i$ arrives at $v$ at timestep $t$ and $a_j$ arrives at $v$ at timestep $t+\Delta$. We resolve this conflict with temporal barrier constraints 
%$B(a_i, R_i, R_g, k,0)$ and $B(a_j, R_i, R_g, k,\Delta)$.  
%Figure~\ref{fig3}(b) shows the example that $a_i$ is blocked by temporal barrier constraint and does not have a $k$-delay conflict anymore.
%
%\subsection{Extended Rectangle Area}
%
%\begin{figure}
%\centering
%\begin{subfigure}{0.48\columnwidth}
%  \centering
%  \includegraphics[width=0.9\columnwidth]{extendeda.jpg}
%  \caption{Normal barrier constraint failed, the orange area still exists.}
%  \label{fig4:sub1}
%\end{subfigure}
%\begin{subfigure}{0.48\columnwidth}
%  \centering
%  \includegraphics[width=0.9\columnwidth]{extendedb.jpg}
%  \caption{Temporal barrier constraint use start-goal rectangle border eliminate all conflicts and orange area}
%  \label{fig4:sub2}
%\end{subfigure}
%\begin{subfigure}{0.8\columnwidth}
%  \centering
%  \includegraphics[width=1\columnwidth]{extendedc.jpg}
%  \caption{The CT tree for resolving $k$-delay rectangle conflicts with temporal barrier constraints using start-goal rectangle border.}
%  \label{fig4:sub3}
%\end{subfigure}
%\caption{Extended rectangle area and using the start-goal border for temporal barrier constraint when k=2.   }
%\label{fig4}
%\end{figure}
%
%The aim of introducing a temporal barrier constraint is to force the optimal cost of constrained agent to increase by $1+k-delay$. 
%However, when $k \geq 2$, the temporal barrier constraint with $B(a_x, R_x, R_g, k, delay)$ failed. As shown in Figure \ref{fig4:sub1}, when $k=2$, temporal barrier constraint $B(a_i,(4,4),(4,5),2,0)$ is used to force $a_i$’s optimal path to increase by 3, to a length of 9, to avoid the conflict with $a_j$. 
%However, the cost of optimal paths of agent $a_i$ is still 8, 
%because $a_i$ can bypass the temporal barrier constraint. In this case, all paths of $a_i$ with cost 8 conflict with all the optimal paths of $a_j$ in the light yellow area, which is larger than the rectangle. 
%
%The light yellow area is an extended rectangle area. Each time $k$ increased by 2, constrained agent need to find a path with 2 more cost. This makes CBS can choose a wider path with 2 more cost that bypass rectangle area, which means the size of the extended rectangle area increased.
%
%Once $k$ is big enough to force the agent to bypass the unconstrained agent’s start-goal rectangle, the optimal path of constrained agents will no longer intersect with unconstrained agent’s optimal path. Thus the extended rectangle area is at most the unconstrained agent’s start-goal rectangle. 
%
%\subsection{$k$-Robust Cardinal Rectangle Reasoning}
%
%On approach to overcome the above problem is to use the border of the extended rectangle area to define a temporal barrier constraint. 
%We use a simpler method which extends the border of unconstrained agent’s start and goal rectangle as the barrier in order to to overcome this problem. Figure \ref{fig4:sub2} shows the latest timestep that $a_i$ can arrive at each vertex in the rectangle area when trying to reach the goal at timestep 9. 
%In this case, the low-level search of $a_i$ has many options for reaching 
%the goal at timestep 9 without conflict with optimal paths of agent $a_i$.  Figure \ref{fig4:sub3} shows the CT tree when solving rectangle conflicts with temporal range constraints. We denote the temporal barrier constraint using the border of unconstrained agent’s start and goal rectangle as $B(a_x, Rs_x, Rg_x, k, delay), x \in [ i, j ]$. 
%$Rs_x$ and $Rg_x$ are the two corner nodes of the border of the start-goal rectangle that are opposite to $a_x$’s start location $s_x$. 
%We call the algorithm using the extended
%temporal border constraint $B(a_x, Rs_x, Rg_x, k, delay), x \in [ i, j ]$ to resolve $k$-delay cardinal rectangle conflict as \textbf{K-CBSH-CR}.
%
%Using the border of unconstrained agent’s start and goal rectangle will introduce some redundant constraints. But they do not over constrain the target agent. Using the example in Figure \ref{fig4:sub2}, if the $k=2$ and 
%vertex (4,2) is constrained at timesteps 1, 2, and 3, since the earliest timestep that the constrained agent can arrive at (4,2) is 5 this does remove any possible paths for the agent.
%Similarly while vertex (6,7) is constrained at timesteps 6, 7, and 8; paths for $a_i$ to reach the goal through (6,7) have a cost of at least 10, and hence no possible paths are removed. 
%
%\textbf{Property 1.} For any path combination of two agents $a_i$ and $a_j$ that have $k$-delay cardinal rectangle conflict (assuming $a_i$ arrives rectangle area $\Delta$ timestpes early than $a_j$). If one path violates $B(a_i, Rs_i, Rg_i, k,0)$ and the other path violates $B(a_j, Rs_j, Rg_j, k,\Delta)$, then the two agents have $k$-delay conflict within the rectangle area.
%
%\textit{Proof.} 
%If the optimal time that agent $a_i$ can arrive vertex $N_i$ on border $Rs_i$ to $Rg_i$ is $c_i$.  Now $a_i$ arrives at $N_i$ at $t_i$, $c_i \leq t_i \leq c_i+k$ and $d_i=t_i-c_i$ ($d_i$ is the timestep difference between the timestep that $a_i$ arrive $N_i$ and the optimal timestep that $a_i$ can arrive $N_i$), hence $a_i$ violates constraint $B(a_i, Rs_i, Rg_i, k,0)$.
%
%If the optimal time that agent $a_j$ can arrive vertex $N_j$ on border $Rs_j$ to $Rg_j$ is $c_j$ and the optimal time that agent $a_i$ can arrive vertex $N_j$ is $c_{i\_nj}$. Hence the timestep difference that two agents optimally arrive a vertex in rectangle area is $\Delta$, $c_{i\_nj} + \Delta = c_j$ and $c_{i\_nj}\leq c_j$. 
%Now the $a_j$ arrive $N_j$ at $t_j$, and $c_{i\_nj}\leq c_j\leq t_j\leq c_j-\Delta + k = c_{i\_nj}+k$, hence $a_j$ violate $B(a_j, Rs_j, Rg_j, k,\Delta)$. $d_j=t_j-c_j$, which is the timestep difference between $t_j$ and $c_j$.
%
%The requirement (c) in section 5.1 guarantees that the path of $a_i$ and the path of $a_j$ must have an intersect vertex, which means they both traverse a vertex at same or different timestep. The intersection vertex in denoted as $v$. 
%
%The optimal time that $a_i$ arrive $v$ is $c_{i\_v}$, which is also the earliest time that $a_i$ can arrive $v$. 
%
%The optimal time that $a_j$ can arrive $v$ is $c_{j\_v}$ and the latest time that $a_j$ can arrive $v$ is $c_{j\_v}+d_j$. 
%
%As agent $a_i$ and $a_j$ have $k$-delay rectangle conflicts and the optimal path of $a_i$ arrive rectangle area early than $a_j$, thus $c_{j\_v}-c_{i\_v}=\Delta$ and $\Delta \leq k$. 
%
%Because $t_j\leq c_{i\_nj}+k$:
%\[t_j-c_j\leq c_{i\_nj}+k-c_j\]
%\[d_j\leq c_{i\_nj}+k-c_j\]
%As $a_i$ and $a_j$ have $k$-delay rectangle conflicts, the time difference that two agents' optimal path arrive any vertex in rectangle conflicts is $\Delta$ and also because of $c_{i\_nj}\leq c_j$:
%\[d_j\leq -\Delta+k\]
%\[d_j+\Delta\leq k\]
%Thus 
%\[d_j+c_{j\_v}- c_{i\_v} \leq k\]
%Hence $d_j+c_{j\_v}$ is the latest time that $a_j$ can arrive vertex $v$ and $c_{i\_v}$ is the earliest time that $a_i$ can arrive $v$, the time difference between the latest time that $a_j$ can arrive $v$ and the earliest time that $a_i$ can arrive $v$ is always smaller than k, which means have a $k$-delay conflict between $a_i$ and $a_j$ at $v$.
%
%Therefore if $a_i$ and $a_j$ have $k$-delay rectangle conflicts, one path violates $B(a_i, Rs_i, Rg_i, k,0)$ and the other path violates $B(a_j, Rs_j, Rg_j, k,\Delta)$, then the two agents have $k$-delay conflict within the rectangle area.
%\qed
%
%\mike{Sketch of proof}
%\textit{Proof Sketch.} 
%The requirement (c) in section 5.1 guarantees that the path of $a_i$ and the path of $a_j$ must have an intersect vertex $v$ if both agents traverse each other's start and goal rectangle. 
%
%Assuming the optimal time that agent $a_i$ can arrive vertex $N_i$ on border $Rs_i$ to $Rg_i$ is $c_i$ and the real time $a_i$ arrives at $N_i$ is $t_i$, $c_i \leq t_i \leq c_i+k$ and $d_i=t_i-c_i$.
%
%Assuming the optimal time that agent $a_j$ can arrive vertex $N_j$ on border $Rs_j$ to $Rg_j$ is $c_j$ and the optimal time that agent $a_i$ can arrive vertex $N_j$ is $c_{i\_nj}$. Hence the timestep difference that two agents optimally arrive a vertex in rectangle area is $\Delta$, $c_{i\_nj} + \Delta = c_j$ and $c_{i\_nj}\leq c_j$. Assuming the real time the $a_j$ arrive $N_j$ is $t_j$, $c_{i\_nj}\leq c_j\leq t_j\leq c_j-\Delta + k = c_{i\_nj}+k$, and $d_j=t_j-c_j$.
%
%Assuming the optimal time (earliest time) that $a_i$ can arrive $v$ is $c_{i\_v}$. 
%
%Assuming optimal time that $a_j$ can arrive $v$ is $c_{j\_v}$, the latest time that $a_j$ can arrive $v$ is $c_{j\_v}+d_j$. 
%
%As $a_i$'s optimal path have $k$-delay conflict with $a_j$'s optimal path, we know $c_{j\_v}-c_{i\_v}=\Delta$.
%
%With these information, we can prove that $c_{j\_v}+d_j - c_{i\_v}$ always smaller than k, which means we have a $k$-delay conflict at $v$.
%\qed
%
%
%\subsubsection{Theorem 1.} K-CBSH-CR is complete and optimal.
%
%\textit{Proof.}  The proof is similar to the proofs in \citet{atzmon} and \citet{li2019}.  
%If $a_i$ and $a_j$ have a conflict $(a_i, a_j, v, t, \Delta$. For a CT node $N$, $N1$ and $N2$ are the child nodes for $N$. $N1$ hold the constraint $B(a_i, Rs_i, Rs_i, k,0)$ and $N2$ hold the constraint $B(a_j, Rs_j, 
%Rs_j, k,\Delta)$. $\pi(N1)$ denotes all the $k$-Robust plans that satisfy $N1.constraints$ and $\pi(N2)$ denotes all the $k$-Robust plans that satisfy $N2.constraints$. Based on property 1, the temporal barrier constraint does not eliminate any conflict-free solutions. Thus $\pi (N) =  \pi (N1) \cup \pi (N2)$. Thus K-CBSH-CR does not eliminate any possible solution and is complete. Furthermore, the low-level search of any kind of CBS always returns an optimal path, the high-level search always chooses a CT node with minimum $f$-value to expand and K-CBSH-CR does not eliminate any possible solution when splitting. Therefore, the first chosen CT node whose paths are conflict-free has a set of conflict-free paths with minimum cost. Thus K-CBSH-CR is optimal.
%\qed
%
%\subsection{Extending $k$-Robust Rectangle Reasoning}
%
%\citet{li2019} shows that rectangle reasoning can also be used to resolve semi-cardinal rectangle conflict and non-cardinal rectangle conflicts, not only cardinal rectangle conflicts. This algorithm is called CBSH-R. As the 
%barrier constraints only block paths that traverse the rectangle area and do not block all optimal paths for semi-cardinal or non-cardinal rectangle conflicts, it may fail to resolve some conflicts. CBSH-R needs to esnure 
%the barrier constraint resolves the current conflict so that it cannot
%arise in the current node’s ancestors.  By replacing the barrier constraint with a temporal barrier constraint using the border of the unconstrained agent’s start-goal rectangle, CBSH-R is modified to plan $k$-Robust solutions and we denote this algorithm \textbf{K-CBSH-R}. 
%
%\textbf{Theorem 2.} K-CBSH-R is complete and optimal.
%
%\textbf{Proof.} As temporal barrier constraint for $a_i$ will not block any path that does not traverse $a_j$’s start goal rectangle, thus temporal barrier constraint for $a_i$ will not block any path that does not intersect with $a_j$’s path. Therefore Property 1 still holds for K-CBSH-R. Thus the proof in Theorem 1 still works for K-CBSH-R, which means K-CBSH-R also is complete and optimal. \qed
%
%\subsubsection{Rectangle Conflict in Path Segments}
%\citet{li2019} further extends the usage of barrier constraints and use it to solve rectangle conflicts caused by obstacles and other constraints. It uses a Multi-Valued Decision Diagram (MDD) (Sharon et al. 2013), which is a directed acyclic graph, to find singletons in the paths of each agent. An MDD stores all possible locations at each timestep for an agent to reach its goal optimally, which is the same as storing all optimal paths of an agent. If a timestep only has one possible location, which means all optimal paths must traverse this location at this timestep, this location at this time step is called a singleton. This algorithm uses all the singletons from conflict agents’ paths as candidate start and goal locations and then CBSH-RM try to find and classify rectangle conflicts in all possible start and goal combinations. When multiple conflicts exist, CBSH-RM first prefers rectangle conflicts with higher priority type, then it prefers a larger rectangle area. 
%
%For $k$-delay rectangle conflicts, current conflict detection tie braking policy cannot efficiently resolve all problems, as the rectangle conflicts does not consider extended rectangle area. Thus, for $k$-Robust plan, the rectangle conflicts with larger extended rectangle area are preferred when two rectangle conflicts have the same priority type and rectangle area.\
%
%\subsubsection{Adding Temporal Barrier Constraint}
%\citet{li2019} also find that if blocking all vertexes on the border of the rectangle opposite the constrained agent, CBSH-RM may lose optimality. Because when barrier constraint force the agent to reach the goal with a higher cost, it is possible that alternative paths, which do not traverse selected start singleton but traverse constrained barrier vertexes. Blocking all vertexes on the border of the rectangle area loses these path choices. By using MDD for each agent in conflict, CBSH-RM avoid losing optimality by checking does any optimal path of constrained agent traverse the vertexes included in barrier constraint and if no any optimal path traverse a vertex, this vertex will not be constrained.
%
%$k$-Robust rectangle reasoning requires to block the extended rectangle area as well. Although the MDD provides the information of all optimal paths of an agent, these optimal paths do not traverse extended rectangle area. Therefore, if the optimal cost from selected start singleton to selected goal singleton is $c$, an MDD of constrained agent stores all paths from selected start singleton to selected goal singleton with a cost of $c+k$ is used to support the adding of temporal barrier constraint. An MDD with the cost of $c+k$ contains all paths with cost $i,  c\leq i \leq c+k$, as a path with cost i can become a path with cost c+k by waiting at goal location.
%
%For any vertex $v$ in the border of extended rectangle area opposite to constrained agent, if the optimal time that the agent arrives at the vertex is $t$ , the time that the agent arrive selected start singleton is $t_s$, and the level $(t-t_s) +i,i\in (0,k)$, of the MDD include vertex $v$, $v$ is constrained from time $t+i$ to $t +k$. By constraint the vertexes only exist in MDD Property 1 still holds here. This algorithm is denoted as K-CBSH-RM.
%
%\mike{A shorten version:} \citet{li2019} shows that rectangle reasoning can also be used to resolve semi-cardinal rectangle conflict and non-cardinal rectangle conflicts, not only cardinal rectangle conflicts. By replacing the barrier constraint with a temporal barrier constraint, it is modified to plan $k$-Robust solutions and we denote this as \textbf{K-CBSH-R}. \citet{li2019} further extends the usage of barrier constraints and use it to solve rectangle conflicts caused by obstacles and other constraints. It uses a Multi-Valued Decision Diagram (MDD) (Sharon et al. 2013), which is a directed acyclic graph, to find singletons in the paths of each agent. An MDD stores all possible paths of an agent at a certain cost. If a timestep only has one location, which means all paths traverse this location at this timestep, it is called a singleton. This algorithm uses all the singletons from conflict agents’ paths as candidate start and goal locations and then CBSH-RM try to find rectangle conflicts in all possible start and goal combinations. By replacing barrier constraint with temporal constraint, it works for planning $k$-robust solution and is denoted as \textbf{K-CBSH-RM}.
%
%
%
%\section{$k$-Robust Corridor Reasoning}
%The difference between corridor conflict with $k$-Robust CBS and normal corridor conflict is that agents need to occupy vertexes for extra timesteps to avoid $k$-delay conflicts. Assume there is a corridor conflict with a length of $l$ between vertex $b$ and vertex $e$. Agent $a_1$ moving from $b$ to $e$ and agent $a_2$ moving from $e$ to $b$. If the agent $a_1$ reach vertex $e$ at timestep $t_1$ and agent $a_2$ reach vertex $b$ at timestep $t_2$.For planning $k$-Robust solution, any path of $a_1$ that reach vertex $e$ at or before timestep $t_2+l+k$ must conflict with any paths of $a_2$ that reach vertex $b$ at or before timestep $t_1+l+k$.
%
%When considering bypasses, assuming agent $a_1$ can reach vertex $e$ at timestep $t'_1$ and agent $a_2$ reach vertex $b$ at timestep $t'_2$ without traverse the corridor. Therefore for planning $k$-Robust solution, any path of $a_1$ that reach vertex $e$ at or before timestep $min(t'_1  - 1+k,t_2  + l+k)$ must conflict with any paths of $a_2$ that reach vertex $b$ at or before timestep $min(t'_2  - 1+k,t_1  + l+k)$.
%
%Therefore, a pair of range constraint is used to perform $k$-Robust corridor reasoning. When splitting CT node, child node 1 hold the constraint $<a_1,e,[0,min(t'_1  - 1+k,t_2  + l+k)]>$ and child node 2 hold the constraint $<a_2,b,[0,min(t'_2  - 1+k,t_1  + l+k)]>$.
%
%\textbf{Theorem 2.} $k$-Robust Corridor Reasoning is complete and optimal.
%
%\textit{Proof} We have shown that if $a_1$ and $a_2$ both violate constraint $<a_1,e,[0,min(t'_1  - 1+k,t_2  + l+k)]>$ and constraint $<a_2,b,[0,min(t'_2  - 1+k,t_1  + l+k)]>$, they must have a conflict in the corridor. Thus the adding of these constraints will not eliminate any conflict free $k$-Robust solution. Thus $k$-Robust Corridor Reasoning is complete. $k$-Robust Corridor Reasoning is based on CBS, as proved in Theorem 1, CBS guarantees that the solution is optimal as long as no conflict free solution is eliminated.
%
%\section{$k$-Robust Target Reasoning}
%Assuming that agent $a_i$ reaches its goal $g_i$ on timestep $l$, and agent $a_j$ has a target conflict with the agent $a_i$ at $g_i$ on timestep $t,t \geq l$. All solutions that both $a_i$ and $a_j$ visit $g_i$ at $t$ must have conflict. ~\citet{corridor} resolve target conflict by force $a_i$ to reach its goal after $t$ or force any other agent visit $g_i$ at or after $t$. Planning $k$-Robust solution requires the avoiding of $k$-delay conflict. Therefore, when splitting, one child node forces $a_i$ to reach its goal after $t+k$ to give $a_2$ priority and do not cause $k$-delay conflict. Another child node forbids any other agent visit $g_i$ at or after $t$ to force all other agents find bypasses to their goal locations. If any agent failed to find a bypass route, we do not generate this child node. 
%
%\textbf{Theorem 3.} $k$-Robust Target Reasoning is complete and optimal.
%
%\textit{Proof} We have shown that target reasoning only eliminate the solutions that have target conflict and do not eliminate any conflict free solution. Thus $K$-robust Target Reasoning is complete. $k$-Robust Target Reasoning is based on CBS. As proved in Theorem 1, CBS guarantees that the solution is optimal as long as no conflict free solution is eliminated.


==> K-Robust Symmetry Breaking (4)/reasoning-old.tex <==
\section{$k$-Robust Rectangle Reasoning}

%$k$-Robust rectangle conflicts occur when 
%two agents arrive in a rectangle area such as Figure~\ref{fig1} (left);
%not just at the same time but also within $k$ timesteps of one another.


A rectangle conflict arises when two agents paths need to cross
but there are many ways that they can cross. This causes difficulty 


Figure~\ref{fig1} (a) illustrates a ($k = 0$) rectangle conflict,
any optimal paths for the two agents from their start to target will conflict somewhere in the rectangle. In a $k$-delay rectangle conflict the agents may not arrive at a vertex at the same time, but within $k$ timesteps. For example is we move $S_2$ to (2,2) the same illustrated rectangle is a $1$-delay rectangle conflict. 

To resolve such conflicts we introduce \textbf{Temporal Barrier Constraints}, which unify
the (temporal) range constraints of~\cite{atzmon} and the (spatial) Barrier Constraints of~\cite{li2019}.

\begin{defn}
Given a vertex time pair $p = (u,t)$ the \emph{optimal time} 
$ot(p,v)$ to reach 
vertex $v = (v_x,v_y)$ starting from $u = (u_x,u_y)$ at time $t$ is
calculated by adding the Manhattan distance 
$ot(p,v) = t + |v_x - u_x| + |v_y - u_y|$.

A \emph{$w$ temporal barrier constraint} is denoted by
$B(a_x, V, p, w)$. 
This constraint forbids the 
agent $a_x$ from visiting any vertex $v \in V$ 
at the optimal time from vertex time pair $p$, or any time step up to $w$ later. 
That is the barrier constraint $B(a_x, V, p, w)$ 
is the set of time-range vertex constraints$\langle a_x, v, [ot(p,v), ot(p,v) + w] \rangle, v \in V$.
\label{defi:barrier}
\end{defn}


Given a rectangular grid map we can define a \emph{rooted rectangle} $R$ as the set of vertices
occurring in the rectangle defined by the 
two corner points $(D_x,D_y)$ the root corner, and 
$(E_x,E_y)$ the opposite corner. 
In Figure~\ref{fig1} the illustrated rectangle is  defined by (2,2) and (3,3).

A rectangle $R$ defined by $((D_x,D_y),(E_x,E_y))$ defines 4 sides: 
$S1(R) = \{ (D_x,D_y) .. (D_x,E_y) \}$,
$S2(R) = \{ (D_x,D_y) .. (E_x,D_y) \}$,
$S3(R) = \{ (D_x,E_y) .. (E_x,E_y) \}$, and
$S4(R) = \{ (E_x,D_y) .. (E_x,E_y) \}$.
For the illustrated rectangle of Figure~\ref{fig1}, 
$S1(R)$ is the left side \{ (2,2),(2,3)\},
$S2(R)$ is the top, $S3(R)$ is the bottom, and $S4(R)$ the right side.

We can now explain a rectangle conflict for the case $k = 0$
differently from the explanation in ~\cite{li2019}.

\begin{theorem}\label{thm:rect:0}
Given an arbitrary rectangle $R$ defined by $((D_x,D_y),(E_x,E_y))$
and root time $rt$
and two paths for agents $a_1$ and $a_2$ such that
constraints $B(a_1,S1(R),(D,rt),0)$,
$B(a_1,S4(R),(D,rt),0)$,
$B(a_2,S2(R),(D,rt),0)$, and
$B(a_2,S3(R),(D,rt),0)$ are all violated, then
the paths of the two agents have a $0$-delay vertex conflict.
\end{theorem}
\begin{proof}
Assume that $S1(R)$ is the left of the rectangle, 
$S4(R)$ the right, $S2(R)$ the top, and $S3(R)$ the bottom, 
the other cases follow similarly. 

Since agent $a_1$ enters the rectangle at the left at the optimal time, and leaves from the right at the optimal time it cannot wait, and must remain within the rectangle, and every vertex it visits within the rectangle it visits at the optimal time.
Similarly for agent $a_2$. 
Now since agent $a_1$ crosses from left to right, and agent $a_2$ from top to bottom, there paths must cross.  Since they share a vertex $v \in R$ and they only visit vertices at the optimal time, their paths have the vertex conflict $\langle a_1,a_2,v,ot((D,rt),v),0 \rangle$.
\end{proof}

This leads to a generic way of handling a rectangle conflict. 
Since no two compatible agents paths can violate all four barriers we can impose the constraint 
$B(a_1,S1(R),(D,rt),0)$ $\vee$
$B(a_1,S4(R),(D,rt),0)$ $\vee$
$B(a_2,S2(R),(D,rt),0)$ $\vee$
$B(a_2,S3(R),(D,rt),0)$ 
without removing solutions.  This is imposed by a four way branch where we impose of the constraints in each branch. 

We can usually do better than this. If all possible paths for $a_1$ 
(given the current set of constraints upon it) that violate
$B(a_1,S4(R),(D,rt),0)$ must also violate $B(a_1,S1(R),(D,rt),0)$ 
we can remove the second disjunct. 
This is common, note for the example that any path for agent $a_1$ in Figure~\ref{fig1}
which reaches the right side at the optimal time, also crossed the left side at the optimal time.
The same reasoning applies for $B(a_2,S2(R),(D,rt),0)$ $\vee$
$B(a_2,S3(R),(D,rt),0)$. Hence usually we end up with a two way branch
$B(a_1,S4(R),(D,rt),0)$ $\vee$
$B(a_2,S3(R),(D,rt),0)$.

We can extend the above 
reasoning for $k > 0$ conflicts.

\begin{theorem}\label{thm:rect:1}
Given an arbitrary rectangle $R$ defined by $((D_x,D_y),(E_x,E_y))$
and two root times $rt_1$ and $rt_2$
and two paths for agents $a_1$ and $a_2$ such that
constraints 
$B(a_1,S1(R),(D,rt_1),1)$,
$B(a_1,S4(R),(D,rt_1),1)$,
$B(a_2,S2(R),(D,rt_2)),1)$, and
$B(a_2,S3(R),(D,rt_2)),1)$ are all violated, then
the paths of the two agents have a $k$-delay vertex conflict,
assuming $max(rt_1,rt_2)+1 - min(rt_1,rt_2) \leq k$
\end{theorem}
\begin{proof}
Assume that $S1(R)$ is the left of the rectangle, 
$S4(R)$ the right, $S2(R)$ the top and $S3(R)$ the bottom, 
the other cases follow similarly. 

Since agent $a_1$ enters the rectangle at the left at the optimal time wrt $rt_1$ or one later, and leaves from the right at the optimal time or one later
its path can wait at most one step in the rectangle, and cannot leave the rectangle, since this would require at least 2 time steps.
Every vertex it visits in the rectangle is visited at the optimal time wrt $rt_1$, or the optimal time + 1 (or both).
Similarly agent $a_2$ enters the top of rectangle at optimal time wrt $rt_2$ or one later, and leaves the bottom of the rectangle at the optimal time wrt $rt_2$ or one later. Again it cannot leave the rectangle, and can take at most one wait in the rectangle. Every vertex it visits at the optimal time wrt $r_t$ or one later (or both).

Now since agent $a_1$ crosses from left to right, and agent $a_2$ from top to bottom, there paths must cross.  Since they share a vertex $v \in R$ since they agent $a_1$ this vertex at $t_1 \in ot((D,rt_1),v) .. ot((D,rt_1),v)+1$, agent $a_2$ visits this vertex at $t_2 \in ot((D,rt_1),v).. ot((D,rt_2),v) + 1$
there is a $k$-delay conflict
$\langle a_1, a_2, v, t, k \rangle$, 
since by the conditions on
$rt_1$ and $rt_2$, $| t_1 - t_2| \leq k$.
\end{proof}

We can resolve the rectangle conflict by branching on 
$B(a_1,S1(R),(D,rt_1),1)$ $\vee$
$B(a_1,S4(R),(D,rt_1),1)$ $\vee$
$B(a_2,S2(R),(D,rt_2),1)$ $\vee$
$B(a_2,S3(R),(D,rt_2),1)$,
and often, if we can prove the required implications, the simpler 
$B(a_1,S4(R),(D,rt_1),1)$ $\vee$
$B(a_2,S3(R),(D,rt_2),1)$.
Currently none of our methods detect the simpler 2 way splitting case.
\pjs{Is this true mike! mike: for the plots currently showing in this paper, no 2-way split CR/RM.}
Note that the barriers we create are $1$-barriers (for two consecutive time steps). 
Unfortunately we cannot easily extend to $w$-barriers where $w \geq 2$.
As shown in Figure~\ref{fig3}, consider the 3x3 rectangle $R = ((2,2),(4,4))$ 
with root times $rt_1 = rt_2 = 1$, 
and the paths for agent $a_1$ 
[((1,2),0), ((1,3),1), ((1,4),2), ((2,4),3), 
 ((2,5),4), ((3,5),5), ((4,5),6), ((4,4),7), ((5,4),8))]
 and for agent $a_2$
[((2,1),0), ((3,1),1), ((3,2),2), ((3,3),3), ((3,4),4), 
 ((3,4),5), ((3,4),6), ((3,4),7), ((3,5),8), ((4,5),9)].
Note that agent $a_1$ violates $2$-barrier $B(a_1,S1(R),((2,2),1),2)$ 
at $((2,4),3)$
and $2$-barrier $B(a_1,S4(R),((2,2),1),2)$ at $((4,4),7)$; while
agent $a_2$ violates $2$-barrier $B(a_2,S2(R),((2,2),1),2)$ 
at $((3,2),2)$
and $2$-barrier $B(a_2,S3(R),((2,2),1),2)$ at $((3,4),4)$ but 
the paths of the agents do not intersect within the rectangle $R$,
indeed there are no conflicts, since agent $a_2$ waits before leaving the rectangle. 



\begin{figure}
  \centering
  \includegraphics[width=0.50\columnwidth]{2barrierExample.jpg}
  \caption{Example of how $w$-barriers where $w \geq 2$ can eliminate a conflict free solution.}
  \label{fig3}
\end{figure}

\subsection{Detecting Rectangle Conflicts}

When we detect a vertex conflict during CBS we need to recognise that it's actually a 
rectangle conflict, in order to perform the rectangle symmetry breaking.
The simplest way of recognizing a rectangle conflict, called CR in~\cite{li2019}, can be understood as follows:
\begin{itemize}
\item[(a)] Both agents follow their Manhattan optimal paths from start to goal. 
\item[(b)] Both agents move in only the same horizontal and vertical directions along their paths.
\item[(c)] The start and goal nodes of two agents have relative opposite locations. This requirement ensures that all optimal paths of both agents intersect within the rectangle area.
\end{itemize}
Figure~\ref{fig1} gives an example. 

In this case \citet{li2019} defines the rectangle from the start and goal locations.
Suppose the agents currents paths have $k$-delay conflict 
at vertex $v$ with agent $a_1$ arriving at time $t$ and agent $a_2$ arriving at time $t + \Delta, 
\Delta \leq k$. 
$D = (D_x,D_y)$ is given by $D_x$ is the closest of the start locations in the $x$ dimension to $v$, and similarly $D_y$ in the $y$ dimension.
$E = (E_x,E_y)$ is defined similarly from the goal locations. 

Using Theorem~\ref{thm:rect:1} we can extend this to handle $k$-delay conflicts.
Clearly the current paths must conflict with barriers of the rectangle $R$ defined by $D$ and $E$.
Hence we can apply the rectangle conflict splitting to remove the current paths.
We call the detection of CR rectangle and the associated branching K-CBSH-CR

\begin{theorem}
K-CBSH-CR is correct.
\end{theorem}
\begin{proof}
By definition all barrier constraints of the rectangle $R$ are violated by the current paths of the agents. 
From Theorem~\ref{thm:rect:1} applying the barrier disjunction cannot remove solutions, and certainly removes the current paths.
\end{proof}


We can extend the detection of rectangle conflicts to more complicated cases as follows.

Assume agent $a_1$ and $a_2$ have a $k$-delay vertex conflict $\langle a_1, a_2, v, t, \Delta \rangle$.
Assume that $a_1$ enters $v$ moving in direction $d_1$ and $a_2$ enters moving in direction $d_2$.  They must be different or there is an earlier vertex conflict (where they both came from). 
If they are opposite directions then there is no rectangle conflict.

So assume $d_1$ and $d_2$ are orthogonal directions.
Let $(B1_x,B1_y)$ be the earliest singleton in the path of agent $a_1$ where all moves from here to $v$ are in direction $d_1$ or $d_2$
and there are no waits, similarly define $(B2_x,B2_y)$ for agent $a_2$.
Let $(A1_x,A1_y)$ be the latest singleton in the path of agent $a_1$ where all moves from $v$ to here are in directions $d_1$ or $d_2$
and there are no waits, similarly define $(A2_x,A2_y)$ for agent $a_2$.

Define $D_x$ to be the closer of $B1_x$ and $B2_x$ to $v_x$,
similarly for $D_y$. Define $E_x$ to be the closer of $A1_x$
and $A2_x$ to $v_x$, similarly for $E_y$. 

Now either the current path of $a_1$ crosses the entry barrier for $d_1$ in $R$ and $a_2$ crosses the entry barrier for $d_2$ in $R$ or there must be a vertex $B'$ before $v$ in both paths where the two paths cross (otherwise they could not enter vertex $v$ in the appropriate direction).  If the second case holds, replace $B$ by $B'$. 
Similarly the current path of $a_1$ must cross the exit barrier for $d_1$ in $R$ and $a_2$ must cross the exit barrier or there is a vertex $E'$ after $v$ in both paths where they cross. Again in the second case replace $E$ by $E'$. Figure~\ref{RecDectFig} shows an example of the detection of a rectangle conflicts when $k$=2.

\begin{figure}
  \centering
  \includegraphics[width=0.4\columnwidth]{RMRecDetect.jpg}
  \caption{Detecting a rectangle conflict when $k=2$; $E$ is replaced by $E'$ as the two paths cross after $V$. }
  \label{RecDectFig}
\end{figure}

By construction the current paths for $a_1$ crosses the entry and exit barriers for $d_1$ at the optimal time wrt $(B,t - |B1_x - v_x| - |B1_y - v_y|)$, similarly $a_2$ crosses the entry and exit barriers for $d_2$ at the optimal time wrt $(B,t+\Delta - |B1_x - v_x| - |B1_y - v_y|)$.
Hence we can apply the rectangle construction of Theorem~\ref{thm:rect:1}
where $rt_1 = t - |B1_x - v_x| - |B1_y - v_y|$ and
$rt_2 = t+\Delta - |B1_x - v_x| - |B1_y - v_y|-1$ unless $\Delta = 0$ and $k = 1$ in which case $rt_2 = rt_1$, since the conditions for the Theorem hold.
The rectangle construction removes the current paths, and other symmetric paths that would lead to the same rectangle conflict.
We call the detection of these more general rectangles and the associated branching K-CBSH-RM (it's a generalization of the RM technique defined by~\citet{li2019}, which has an $O(N^4)$ complexity on rectangle detection while the method here has an complexity of $O(n)$). The correctness holds similarly.

\begin{theorem}
K-CBSH-RM is corect.
\end{theorem}





==> K-Robust Symmetry Breaking (4)/reasoning.tex <==

\section{$k$-Robust Rectangle Reasoning}

Rectangle symmetries arise in $k$-CBS when the paths of two agents cross
topologically. The agents are heading in the same
directions (e.g. down and right in Figure~\ref{fig1:sub1}) and there
exists for each many different but equally shortest paths which arise
from re-ordering their individual moves.
In such cases the standard replanning strategy of $k$-CBS does not help to 
immediately resolve the problem. 
%We formalise this problem as follows:

\begin{definition}[$k$-delay rectangle conflict]
A $k$-delay rectangle conflict between two agents occurs if all paths with cost between optimal and optimal+$k$ (inclusive) for the two agents that enter a given rectangular area have a $k$-delay vertex conflict in the rectangular area. 
\end{definition}

%
%
\noindent
Rectangle conflicts pose substantial challenges for $k$-robust planning
in general and for $k$-CBS in particular because:
\begin{itemize}
\item the agents do not have to reach positions at exactly the
same time to have a conflict; 
\item the delay caused by the conflict can
be up to $k+1$; and 
\item for $k\geq 2$ an agent can leave and enter the
conflicting area without adding more than $k$ steps to its path.
\end{itemize}
%
%Figure~\ref{fig1:sub1} illustrates a rectangle conflict. 
%When $k=0$ any optimal paths for the two agents from their start to target will conflict somewhere in the shaded rectangle. In a $k$-delay rectangle conflict the agents need to arrive at a vertex, instead of at the same time, within $k$ timesteps.
%
\noindent
To address these challenges we follow 
\citet{li2019} where authors develop {\em barrier constraints}:
a pruning strategy that can efficiently resolve rectangle conflicts 
for CBS with $k=0$ in a single 
branching step. With respect to Figure~\ref{fig1:sub1}, one barrier constraint 
prohibits agent $a_1$ from occupying cells (5, 2), (5, 3), and (5,4) at 
timesteps 3, 4, and 5, respectively. Similarly, the other barrier constraint prohibits agent $a_2$ 
from occupying cells (3, 4), (4, 4), and (5, 4) at timesteps 3, 4, and 5, respectively. 
Notice that each barrier blocks all equivalent shortest paths 
and forces one agent or the other to wait, thus resolving 
the conflict.
%If we use the rectangle reasoning method proposed by \citet{li2019} to resolve this conflict, the conflict can be resolved in one split only when $k=0$. 

A straightforward idea for extending this strategy to $k > 0$ would be to increase the ``thickness'' (number of timesteps) of the barrier constraints. We therefore introduce \emph{temporal barrier constraints}, which unify the (temporal) range constraints of~\cite{atzmon} and the (spatial) barrier constraints of~\cite{li2019}.

\begin{definition}[Temporal barrier constraint]
Given a vertex-time pair $p = (u,t)$ we denote with $ot(p, v)$ the \emph{optimal time} 
to reach vertex $v = (v_x,v_y)$ from vertex $u = (u_x,u_y)$ starting at timestep $t$.
We compute the optimal time by adding to $t$ the Manhattan distance from $u$ to $v$:
\mbox{$ot(p,v) = t + |v_x - u_x| + |v_y - u_y|$}.
A \emph{$w$ temporal barrier constraint}, denoted $B(a_x, V, p, w)$, forbids an 
agent $a_x$, currently at vertex-time pair $p$, from visiting any vertex $v \in V$ 
at its optimal time or up to $w$ timesteps later. 
That is, the barrier constraint $B(a_x, V, p, w)$ 
is the set of time-range vertex constraints \mbox{$\langle a_x, v, [ot(p,v), ot(p,v) + w] \rangle, v \in V$}.
\label{defi:barrier}
\end{definition}

To resolve the $k$-robust rectangle conflict in Figure~\ref{fig1:sub1}, one might think that we can replace the two barrier constraints used by \cite{li2019} with two $k$ temporal barrier constraints at the exit of the rectangle. 
However, this approach is not complete! For example, when $k=4$, 
the orange line is a collision-free path for agent $a_2$, no matter what path agent $a_1$ takes. But this solution is eliminated by 
the $w=4$ temporal barrier constraints.
Therefore, we propose a novel approach that enlarges the rectangle area being reasoned about and adding temporal barrier constraints based on it with adjusted thickness so that we can preserve the completeness and optimality by taking into consideration such bypasses.



\subsection{Enlarging Rectangle and Shifting Borders}
\label{section:temporal}

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{temperal_barrier_constraint.png}
\caption{(1) Example of temporal barrier constraints. In this case $k_1=2$, $S1(R)_{l_1}$ and $S4(R)_{l_1}$ are shifted for $l_1 = 1$ grid location away from $S1(R)$ and $S4(R)$,
and $k_2=4$ so $S2(R)_{l_2}$ and $S3(R)_{l_2}$ are shifted for $l_2 = 2$ timesteps from $S2(R)$ and $S3(R)$. (2) The yellow area is the rectangle $R$. Adding the light and dark orange areas
gives rectangle $R'$. (3) The solid red line is a path traversing rectangle $R$ and must have $k$-delay conflicts. The dashed red line is a path bypassing the rectangle $R$, but traversing rectangle $R'$ and must have $k$-delay conflicts as well. 
The green dashed line is a collision-free path bypassing the rectangle $R'$. (4) Extended constraints (Step Temporal Barrier Constraint) defined in Section \ref{section:stepTemporal} fill the gaps in the barriers for the dark orange area.
\label{fig-temporal}}
\end{figure}

Given a 4-neighbor grid map, we define a \emph{rooted rectangle}  $R$ as the set of vertices occurring in the rectangle defined by the 
two corner points $D=(D_x,D_y)$ the root corner, and 
$E=(E_x,E_y)$ the opposite corner. 
As shown in Figure \ref{fig-temporal}, the illustrated rectangle is  defined by $D=(4, 3)$ and $E=(5, 4)$. Given $D$ and $E$, we define four sides: 
$S1(R) = \{ (D_x,D_y) .. (E_x,D_y) \}$,
$S2(R) = \{ (D_x,D_y) .. (D_x,E_y) \}$,
$S3(R) = \{ (E_x,D_y) .. (E_x,E_y) \}$, and
$S4(R) = \{ (D_x,E_y) .. (E_x,E_y) \}$.
We define the \emph{shifted side}
$Sj(R)_l, j \in [1, 4], l \in [0, \lfloor \frac{k}{2}\rfloor]$,
as the side $Sj(R)$ shifted away from the center of $R$
by $l$ grid locations, note the $Sj(R)$ cannot be shifted beyond the start or goal locations of agents involved in the conflict.
Define the  $y$-shifted start location
$D^y_l$ as the root corner $D$ shifted $l$
locations along $y$-axis away from $R$,
and the $x$-shifted start location $D^x_l$ as the start location shifted $l$ locations along $y$-axis away from $R$. Similarly define $E^y_l$ and $E^x_l$.

Given these definitions, the shifted barrier constraints with some particular thickness can define a \emph{$k$-delay rectangle conflict}, that is all paths for two agents $a_1$ and
$a_2$ that cross these barriers must inevitably result in a $k$-delay conflict.

\begin{theorem}\label{thm:rect:1} 
Consider a $k$-robust MAPF problem with an arbitrary rooted rectangle $R$ defined by corners $D$ and $E$
and two arbitrary integers $0 \leq k_1,k_2 \leq k$.
Let root time $rt$ be the minimum of the timestep when agent $a_1$ or $a_2$ reaches the root corner $D$, $l_1 = \lfloor \frac{k_1}{2} \rfloor$,  $l_2 = \lfloor \frac{k_2}{2} \rfloor$, 
$p_1 = (D^y_{l_1},rt-l_1)$, and $p_2 = (D^x_{l_2},rt-l_2)$.
If the paths for agents $a_1$ and $a_2$ violate all of the four constraints:
\begin{itemize}
    \item \emph{$a_1$ Entrance:} $B(a_1, S1(R)_{l_1}, p_1, k_2)$,
    \item \emph{$a_1$ Exit:}     $B(a_1, S4(R)_{l_1}, p_1, k_2)$,
    \item \emph{$a_2$ Entrance:} $B(a_2, S2(R)_{l_2}, p_2, k_1)$,
    \item \emph{$a_2$ Exit:}     $B(a_2, S3(R)_{l_2}, p_2, k_1)$,
\end{itemize}
\noindent 
the paths of the two agents have a $k$-delay vertex conflict. 
\end{theorem}
\begin{proof}
Assume that $S1(R)$ is the top of the rooted rectangle $R$, 
$S4(R)$ the bottom, $S2(R)$ the left, and $S3(R)$ the right. The other cases follow similarly.
$S1(R)_{l_1}$, $S4(R)_{l_1}$, $S2(R)_{l_2}$, $S3(R)_{l_2}$ are corresponding sides shifted away from $R$.
These shifted sides define a new larger rectangle $R'$ with two corner points $D'$ and $E'$, as shown in Figure~\ref{fig-temporal}.

In order to violate the first two constraints, agent $a_1$ has to enter the top of rectangle $R'$ through a vertex $v$ on $S1(R)_{l_1}$ at timestep $ot(p_1,v)$ or up to $k_2$ timesteps later, and leave from the bottom through a vertex $v$ on $S4(R)_{l_1}$ at timestep $ot(p_1,v)$ or up to $k_2$ timesteps later,
so it can wait for at most $k_2$ timesteps in $R'$ but cannot leave $R'$, since this would require at least extra $2l_2 + 2$ timesteps comparing with a shortest path across $R'$ but $2l_2 + 2 > k_2$.
%
Every vertex $v$ it visits in $R'$ is visited 
within the time range [$ot(p_1,v), ot(p_1,v) +k_2]$.

Similarly agent $a_2$ enters the left of rectangle $R'$ through a vertex $v$ on $S2(R)_{l_2}$ at timestep $ot(p_2,v)$ or up to $k_1$ timesteps later, and leaves the right through a vertex $v$ on $S3(R)_{l_2}$ at timestep $ot(p_2,v)$ or up to $k_1$ timesteps later. 
Again it cannot leave $R'$, since this would require at least extra $2l_1 + 2$ timesteps and it can take at most $k_1$ wait in $R'$. Every vertex $v$ it visits in $R'$ is visited
within the time
range $[ot(p_2,v), ot(p_2,v) + k_1]$.

Now since agent $a_1$ crosses from top to bottom and agent $a_2$ from left to right, their paths must cross, say at vertex $v \in R'$. Assume that agent $a_1$ visits vertex $v$ at $t_1 \in [ot(p_1,v), ot(p_1,v) + k_2]$ while agent $a_2$ visits vertex $v$ at $t_2 \in [ot(p_2,v), ot(p_2,v) + k_1]$.
Since $ot(p_1,v)$ and $ot(p_2,v)$ share the same root time $rt$, $ot(p_1,v) = ot(p_2,v)$, and $k_1$ and $k_2$ are both less than or equal to $k$,
which make $|t_1 - t_2| \leq k$,
there is a $k$-delay conflict
$\langle a_1, a_2, v, t_1, t_2-t_1 \rangle$ (if $t_1 \leq t_2$) or $\langle a_2, a_1, v, t_2, t_1-t_2 \rangle$ (if $t_1 > t_2$).
\end{proof}



\subsection{Extending Temporal Barrier Constraints}
\label{section:stepTemporal}

The temporal barrier constraints proposed in Theorem 1 do not cover all situations where two agents must have a $k$-delay vertex conflict in a rectangle area because they do not cover the entire circumference of rectangle $R'$. As the red dashed line path shown in Figure \ref{fig-temporal} illustrates, if agent $a_1$ enters the top of rectangle $R'$ through corner $D'$ at the optimal time, and leaves from left-bottom vertex at the optimal time. This path (red dashed line) traverses through $S2(R)_{l_2}$ and is $2\lfloor \frac{k}{2} \rfloor$ timesteps longer than paths entering through  $S1(R)_{l_1}$ optimally and leaving through $S4(R)_{l_1}$ optimally. Now agent $a_2$ enters $R'$ via $S2(R)_{l_2}$ at the optimal time or up to $k_2$ timesteps later, so they still have a $k$-delay conflict.

We cannot simply extend temporal barrier constraints to the entire circumference of $R'$ to eliminate such conflicts, 
as it would also eliminate the green dashed collision-free path in Figure \ref{fig-temporal}. 
We thus consider a stronger reasoning method.

\begin{definition}[Step temporal barrier constraint]
Denoted by $B_{step}(a_x, S, p, k')$ this constraint reduces the temporal width of 
the barrier $B(a_x, S, p, k')$ by a value of 2 for each step away from the original 
barrier. Let $l' = \lfloor \frac{k'}{2} \rfloor$, we add
range constraints 
$\langle a_x, v, [ot(p,v), ot(p,v)+k' - 2d] \rangle$
for each vertex $v$ in the same line as $S$ 
at distance $d \in [1, l']$ from the original barrier.
\end{definition}

\ignore{
To eliminate these kind of conflicts. We introduce \textbf{Step Temporal Barrier Constraints} denoted by $B_{step}(a_x, V, V_{root}, p, k)$ which is a set of range constraints $\langle a_x, v_i, range(v_i) \rangle, v_i \in V \And v_i\notin V_{root}$.

\pjs{FIX!}
$V$ and $V_{root}$ are two sets of vertexes. Agent $a_x$ is forbid to visit $v_i$, where $v_i \in V$ and $v_i \notin V_{root}$, for a time range. This time range is derived by function $range(v_i)$:
\[
    range(v_i)= 
\begin{cases}
    [ot(p,v_i), upper(v_i)],& \text{if } upper(v_i) \geq ot(p,v_i)\\
    None,              & \text{otherwise}
\end{cases}
\]
\[
upper(v_i) = ot(p,v_i) + k - 2 \cdot d(v_i,V_{root}) 
\]
\[
d(v_i,V_{root}) = \min_{v_j\in V_{root}}Manhattan Distance(v_i, v_j) 
\]
}

For the rectangle $R'$ in Figure~\ref{fig-temporal}, the step temporal barrier constraint
$B_{step}(a_1, S1(R)_{l_1},p_1, k_2)$
consists of $B(a_1, S1(R)_{l_1}, p_1, k_2)$
and the additional range constraints
$\langle a_1, (2,2), [rt+1, rt+1]\rangle$,
$\langle a_1, (3,2), [rt, rt+2]\rangle$,
$\langle a_1, (6,2), [rt+1, rt+3]\rangle$, and
$\langle a_1, (7,2), [rt+2, rt+2]\rangle$.
Notice how the time ranges shrink further from the original barrier.
This prevents the red dashed path in Figure~\ref{fig-temporal}.
We can now extend Theorem~\ref{thm:rect:1}: if the paths of agents $a_1$ and $a_2$ violate all of the four following constraints: 
\begin{itemize}
    \item \emph{$a_1$ Entrance:} $B_{step}(a_1, S1(R)_{l_1},p_1, k_2)$
    \item \emph{$a_1$ Exit:} $B_{step}(a_1, S4(R)_{l_1},p_1, k_2)$
    \item \emph{$a_2$ Entrance:}  $B_{step}(a_2, S2(R)_{l_2},p_2, k_1)$ 
    \item \emph{$a_2$ Exit:} $B_{step}(a_2, S3(R)_{l_2},p_2, k_1)$
\end{itemize}
the paths of the two agents have a
$k$-delay vertex conflict. The proof is similar.



\subsection{Resolution of $k$-Delay Rectangle Conflicts}

We can always 
resolve a rectangle conflict by four-way branching adding to each branch one of the constraints:
$a_1$ Entrance, $a_1$ Exit, 
$a_2$ Entrance, and $a_2$ Exit;
since we know that one of them must be violated in any solution.
\ignore{
$$B_{step}(a_x, S1(R'),S1(R)_{l_1},p_1, k_2) \wedge B(a_1, S1(R)_{l_1},p_1, k_2)$$
$$\vee$$ 
$$ B_{step}(a_x, S4(R'),S4(R)_{l_1},p_1, k_2) \wedge B(a_1, S4(R)_{l_1},p_1 , k_2)$$
$$\vee$$ 
$$ B_{step}(a_x, S2(R'),S2(R)_{l_2},p_2, k_1) \wedge B(a_2, S2(R)_{l_2}, p_2, k_1) $$
$$\vee$$ 
$$B_{step}(a_x, S3(R'),S3(R)_{l_2},p_2, k_1) \wedge B(a_2, S3(R)_{l_2},p_2 , k_1) $$
}
But in many cases, we can correctly resolve the rectangle conflict by two-way branching
on the constraints  $a_1$ Exit and $a_2$ Exit,
if  both agents satisfy the following condition:
\begin{enumerate}[label=\bfseries Condition \arabic*,wide]
\item All possible paths that traverse the exit barrier must also traverse the entrance barrier.\label{condition:1}
\end{enumerate}

We can use a $k$-MDD to check that the condition is satisfied. A $k$-MDD for agent $a_i$ is a modified Multi-Valued Decision Diagram (MDD)~\cite{boyarski2015} that stores all paths of agent $a_i$ from start to goal with path length no more than $k$ above the optimal. 
MDDs are widely used in CBS algorithms to store all optimal paths, the $k$-MDD is a direct extension.


If either agent's $k$-MDD shows that paths that bypass the entrance barrier and traverse the exit barrier exist, the given conflict cannot be resolved by two-way branching on the given barriers, as it may eliminate conflict free paths that bypass the entrance barrier. 
If any combination of $k_1$ and $k_2$ lead to
\ref{condition:1} being satisfied, the given conflict can resolved by two-way branching on the exit barriers.
If none of the combinations satisfy \ref{condition:1}, the given conflict will be resolved as a normal conflict
(i.e. we never do four-way branching).

We can classify $k$-delay rectangle conflicts as cardinal, semi-cardinal and non-cardinal using the $k$-MDD:
\begin{itemize}
    \item A $k$-delay rectangle conflict is \emph{cardinal}, if all paths in the $k$-MDDs of both agents traverse the exit barrier, which means that replanning for any agent involved in the conflict increases the SIC.
    \item A $k$-delay rectangle conflict is \emph{semi-cardinal}, if only one agent has all paths in its $k$-MDD traverse the exit barrier, which again means that replanning this agent involved always increases the SIC while replanning for the other agent does not.
    \item A $k$-delay rectangle conflict is \emph{non-cardinal} if both agents have paths in their $k$-MDD bypass their exit barriers.
\end{itemize}
We can then prioritize selecting conflict based on cardinality.

\subsection{Detecting Rectangle Conflicts}
\label{section:detectRect}

When we detect a vertex conflict during CBS we need to recognise that it's actually a 
rectangle conflict, in order to perform rectangle symmetry breaking.

Assume that agents $a_1$ and $a_2$ have a $k$-delay vertex conflict $\langle a_1, a_2, v, t, \Delta \rangle$. Let $d_1$ and $d_2$ be the moving directions when agents $a_1$ and $a_2$ enter vertex $v$, respectively. If they are the same directions, then there is an earlier vertex conflict (where they both came from). 
If they are opposite directions, then there is no rectangle conflict.

So assume $d_1$ and $d_2$ are orthogonal directions.
Let $(B1_x,B1_y)$ be the earliest vertex in the path of agent $a_1$ where all moves from here to $v$ are in direction $d_1$ or $d_2$, similarly define $(B2_x,B2_y)$ for agent $a_2$. Let $t_{b1}$ be the earliest timestep that $a_1$ visits $(B1_x,B1_y)$ and $t_{b2}$ be the earliest timestep that $a_2$ visits $(B2_x,B2_y)$.
Let $(A1_x,A1_y)$ be the latest vertex in the path of agent $a_1$ where all moves from $v$ to here are in directions $d_1$ or $d_2$, similarly define $(A2_x,A2_y)$ for agent $a_2$.

Define $D_x$ to be the closer of $B1_x$ and $B2_x$ to $v_x$,
similarly for $D_y$. Define $E_x$ to be the closer of $A1_x$
and $A2_x$ to $v_x$, similarly for $E_y$. Figure \ref{RecDectFig} shows an example.

Let $rt_1 = t_{b1} + |B1_x - D_x| + |B1_y - D_y|$ and $rt_2 = t_{b2} + |B2_x - D_x| + |B2_y - D_y|$. 
We define the root time $rt = \min (rt_1,rt_2)$. 

We then for each value $k_1 \in \{0,1,\ldots,k\}$
and $k_2 \in \{0,1,\ldots,k\}$ check if the agents
satisfy \ref{condition:1} using the 
Step Temporal Barriers defined by these values.
We do so by examining the $k$-MDD for each agent,
temporarily blocking its entrance barrier and seeing if its exit barrier is still reachable. 
If not then \ref{condition:1} holds. 
We try the values for $k_1$ and $k_2$ in decreasing order to find the strongest blocking conditions possible.
If $k_1 = a, k_2 = b$ satisfies the conditions we don't
investigate any pairs $(a',b')$ where $a' \leq a$ and 
$b' \leq b$.

\begin{figure}
  \centering
  \includegraphics[width=0.7\columnwidth]{RMRecDetect.png}
  \caption{Detecting a rectangle conflict when $k=2$. }
 
  \label{RecDectFig}
\end{figure}

\ignore{

Then, \textbf{ Algorithm \ref{algoRecDetect}} is used to construct a rectangle that fits Theorem \ref{thm:rect:1}. It tries all possible combinations of $k_1$ and $k_2$ to find rectangles that satisfy \ref{condition:1} and Theorem \ref{thm:rect:1}.
\MikeNote{The pseudo code have the $k'$ part, do I need to further 
explain why I have $k'$ part and why use $k'$ for shift distance $l$? }


\begin{algorithm}
\SetKwFunction{ExtractB}{ExtractB}
\SetKwFunction{ExtractA}{ExtractA}
\SetKwFunction{ExtractDE}{ExtractDE}
\SetKwFunction{GetMDD}{GetKMDD}
\SetKwFunction{BuildBarrier}{BuildBarrier}
\SetKwFunction{SatisCon}{Condition1}
\SetKwFunction{Classify}{Classify}
\SetKwFunction{Blocked}{Blocked}

\SetKwInOut{Input}{input}
\Input{A $k$-delay vertex conflict $\langle a_1, a_2, v,t,\Delta \rangle$, $path_1$, $path_2$,$k$}
$B_1, t_{b1}$ $\leftarrow$ \ExtractB{$path_1,v,t$}\;
$B_2, t_{b2}$ $\leftarrow$ \ExtractB{$path_2,v,t+\Delta$}\;
$A_1$ $\leftarrow$ \ExtractA{$path_1,v,t$}\;
$A_2$ $\leftarrow$ \ExtractA{$path_2,v,t+\Delta$}\;
$D,E,rt_1,rt_2,rt$ $\leftarrow $  \ExtractDE{$B_1,B_2,A_1,A_2,t_{b1},t_{b2}$}\;
$\Delta_{rt} = |rt_1 - rt_2|$\;
$Rectangle \leftarrow null$\;
 \For{$k_{1} \in [0...k]$}{
 \For{$k_{2} \in [0...k]$}{
  $k_1' \leftarrow rt_1 == rt ? k_1 : (k_1 > \Delta_{rt}?k_1 - \Delta_{rt}:0) $\;
  $k_2' \leftarrow rt_2 == rt ? k_2 : (k_2 > \Delta_{rt}?k_2 - \Delta_{rt}:0) $\;
  $l_1 \leftarrow k_2'//2$\;
  $l_2 \leftarrow k_1'//2$\;

 $MDD_1$ $\leftarrow$ \GetMDD{$a_1, k_1'$}\;
 $MDD_2$ $\leftarrow$ \GetMDD{$a_2, k_2'$}\;
 
 $Entrance_1,Exit_1$ $\leftarrow$ \BuildBarrier{$D,E,rt,MDD_1, l_1,k_1$}\;
 $Entrance_2,Exit_2$ $\leftarrow$ \BuildBarrier{$D,E,rt,MDD_2, l_2,k_2$}\;
 
 \If{$Entrance_1$ or $Entrance_2$ or $Exit_1$ or $Exit_2$ is Empty}{
continue\;
 }
 \If{!\SatisCon{$Entrance_1,Exit_1,MDD_1$} or !\SatisCon{$Entrance_2,Exit_2,MDD_2$}}{
 continue\;
 }
 \If{!\Blocked{$path_1,Exit_1$} or !\Blocked{$path_2,Exit_2$}}{
 continue\;
 }
 $Rectangle$ $\leftarrow$ $Entrance_1,Exit_1,Entrance_2,Exit_2$\;
 \Classify{$Rectangle$}
 }
 }
 \If{$Rectangle == null$}{
 return not-rectangle\;
 }
 return $Rectangle$\;
\BlankLine
 * \BuildBarrier{} builds Temporal Barrier Constraints following the definition in Section \ref{section:temporal} and builds Step Temporal Barrier Constraints following the definition in Section \ref{section:stepTemporal}. It also removes vertexes that do not exist in agent's $k$-MDD, and returns empty barriers if Entrance shifted beyond B or Exit shifted beyond E.\;
 \caption{Rectangle Detection}
 \label{algoRecDetect}
\end{algorithm}
}


Figure \ref{RecDectFig} shows an example of the rectangle detection. In this example,  agents $a_1$ and $a_2$ have a 2-delay conflict $\langle a_1,a_2,(3,4),4,2\rangle$ with $d_1$ pointing right and $d_2$ pointing down. Then $B_1$ is located at $(1,4)$ with $t_{b1} = 2$ and $rt_1 = 3$, and $B_2$ located at $(2,1)$ with $t_{b2} = 2$ and $rt_2 = 5$. Root time $rt = min(t_{b1}, t_{b2}) = 3$. 
We detect that for the case $k_1 = k_2 = 2$ the 
Step Temporal Barriers defined by these values satisfy \ref{condition:1}.

%Since the conditions for the Theorem \ref{thm:rect:1} hold.
%The rectangle construction removes the current paths, and other symmetric paths that would lead to the same rectangle conflict.
We call the detection of rectangles and the associated branching K-CBSH-RM (it is a generalization of the RM technique defined by~\citet{li2019}). 

\begin{theorem}
\label{thm:rect:2}
K-CBSH-RM is correct.
\begin{proof}
Since \ref{condition:1} holds for the chosen 
Step Temporal Barriers, and using (extended) Theorem \ref{thm:rect:1}, each pair of paths that violate the exit barriers must conflict. Hence the two-way branching removes no solutions, and advances the search since it is violated by the current paths.
\end{proof}

\end{theorem}




==> K-Robust Symmetry Breaking (4)/symmetries.tex <==
\section{$k$-Symmetries}
\label{section:sym}

\begin{figure}
\centering
\begin{subfigure}{0.6\columnwidth}
  \centering
  \includegraphics[width=\columnwidth]{rectangle.png}
    \caption{}
  \label{fig1:sub1}
\end{subfigure}
\begin{subfigure}{0.8\columnwidth}
  \centering
  \includegraphics[width=\columnwidth]{nodes.png}
    \caption{}
  \label{fig1:sub2}
\end{subfigure}
\caption{ (a)A collision-free solution, orange path, is eliminated, if we simply put "thick" barrier constraints to resolve a $k$-delay rectangle conflict when $k=4$.
(b) How number of high-level nodes expanded by $k$-CBS increases with $k$ and the size of the rectangle area. }
\label{fig1}
\end{figure}

%Although $k$-CBS is currently the most efficient approach we know of to
%generate optimal $k$-robust, it can be highly inefficient when resolving
%symmetric conflicts.  
Symmetries in  MAPF occur when two agents repeatedly run into one another
along equivalent individually optimal paths.  Figure~\ref{fig1:sub1} shows
an example for $k=4$.  Notice that each agent has available a number of optimal-cost
paths. However every optimal path of agent $a_1$ is in collision with
\emph{every} optimal path of agent $a_2$ and vice versa.
Without detecting such situations $k$-CBS will repeatedly split, node after
node, growing the CT tree in order to enumerate all possible
collisions in the highlighted rectangle area. Figure~\ref{fig1:sub2}
shows the result: each time $k$-CBS splits, it potentially doubles the 
amount of search yet remaining to reach the goal node. The size of the
CT tree grows exponentially as the size of the rectangle area increases, causing $k$-CBS 
to return timeout failure. 
Note that as $k$ increases, the size of the CT tree also grows exponentially,
which makes the problem extremely difficulty to solve. 
All this difficulty can be avoided by recognising there exists a simple
optimal strategy: one of the two agents has to wait. 
For $k = 0$ one agent must wait for one timestep. 
For $k > 0$ one agent may need to wait for more than one timestep. 
However, as $k$ grows large the problem can permit optimal-cost
bypass routes that allow one agent to avoid the rectangle area entirely.
For example in Figure~\ref{fig1:sub1}, when $k \geq 4$ the solid-orange-line 
path becomes optimal and agent $a_2$ can reach its target without waiting.

In this work we consider three
distinct symmetric situations which can appear in $k$-robust MAPF:
\begin{itemize}
\item Rectangle Symmetries, as illustrated in Figure~\ref{fig2:sub0}.
\item Corridor Symmetries, as illustrated in Figure~\ref{fig2:sub1}.
\item Target Symmetries, as illustrated in Figure~\ref{fig2:sub2}.
\end{itemize}

Rectangle symmetries have previously been studied in the context of MAPF
($k$ = 0)~\cite{li2019} while
%where they are known to have a dramatic effect
%on CBS performance.  
Corridor and Target Symmetries have only recently been
introduced~\cite{corridor}, again in the context of MAPF ($k$ = 0).
Each time authors show that symmetries are common in a range of standard
benchmarks and they report dramatic gains in performance when these
symmetric situations are resolved via specialised reasoning techniques.
We adapt each of these ideas to $k$-robust planning and we report similarly
strong results. Generalising these constraints is not simply academic. As we
show in the experimental section, $k$-robust plans are needed for important
practical problems. Without the development of suitable algorithmic
techniques such problems will remain out of reach to MAPF planners.

%
%
%
%Each subsequent conflict cause CBS split a node into two child nodes and doubles the work to find a solution. If symmetric conflicts are not handled properly and keep run into conflicts, the CT tress of CBS rapidly grows and finally failed to find a solution. Examples include rectangle conflicts~\cite{li2019}, corridor conflicts and target conflicts~\cite{corridor}. \ref{fig1} shows that if a rectangle conflict is not properly handled, the CT tree of a simple two agent problem can be dramatic huge.
% 
%\subsection{Rectangle Conflicts}



%Figure~\ref{fig1} shows an example of a \emph{rectangle conflict}. 
%\citet{li2019} define the overlapping area of two start and goal rectangles as rectangle area. If every shortest path of agent $a_i$ conflicts with every shortest path of agent $a_j$ in this area, these conflicts are rectangle conflicts. 
%It is very expensive for the CBS-based algorithm to resolve rectangle conflicts~\cite{li2019}, because CBS needs to try every combination of optimal paths from $a_i$ and $a_j$ to realize that any conflict free solution requires one agent to wait for one timestep. 
%In CBS, every split doubles size of CT tree. Figure~\ref{fig1} also shows that the number of nodes expanded by high-level search grows exponentially with  increasing size of the rectangle area. Additionally, the increasing the $k$ 
%for a $k$-robust plan further increase the number of nodes expanded by high-level search.
%
%Just like vertex and edge conflicts, rectangle conflicts can be classified as
%cardinal, semi-cardinal or non-cardinal. High level A* search concentrates on resolving cardinal conflicts first. 
%
%
%\subsection{Corridor Conflicts}
%


%If two agents are moving in opposite directions and the conflicting vertex has a degree of 2, or the conflicting edge is attached to two nodes of degree of two, the conflict is a \emph{corridor conflict}~\cite{corridor}\footnote{Corridor Reasoning and Target Reasoning are introduced in \citet{corridor} which is also submitted to ICAPS 2020. This paper uses Coridor Reasoning and Target Reasoning in different domain compared with \citet{corridor} }. 
%Figure~\ref{fig2}(a) shows an example of a corridor As illustrated
%by the CT tree of Figure~\ref{fig2}(a), CBS need to expand all nodes noted with "..." and their child nodes to prove that +4 node contains optimal solution. This process is expensive, \citet{corridor} found that the cost to resolve a corridor conflict is exponential to the length of the corridor. 
%
%\subsection{Target Conflicts}
%
%\citet{corridor} define that if a conflict happens after one agent reaches its target, the conflict is a target conflict. Figure~\ref{fig2}(b) shows an example of target symmetry conflict. Resolving a target symmetry conflict is also very expensive for CBS, as CBS need to expand all nodes marked "..." and their child nodes to prove that a solution in the +3 node is optimal. ~\citet{corridor} find that the cost to resolve a target symmetry conflict is exponential in the distance between $s_1$ and $g_2$.
%
%\subsection{Symmetric Conflict Reasoning}
%The resolution of symmetric conflict require constraints that let one agent avoid conflict with another one. Normally there are many equivalent paths that allow one agent do not conflict with another one. Therefore we cannot force a agent follow an exact path to avoid conflict. Instead, we need to constraint all conflict solutions and allow CBS to choose any paths that avoid conflict with unconstrained agent.
%
%\citet{li2019} introduced barrier constraint $B<a_x, R_x, R_g> (x = i,j)$ to resolve rectangle conflict. $B<a_x, R_x, R_g> (x = i,j)$ disallow agent $a_x$ visit the vertexes from $R_x$ to $R_g$ on optimal time, which is the border of rectangle area opposite agent $a_x$'s start location. This constraint disallow constrained agent to leave rectangle area on optimal cost and constrained agent can freely choose any path that do not leave rectangle area on optimal cost.
%
%\citet{corridor} introduced corridor reasoning which constraint the time that agent can leave the corridor to eliminate all paths that conflict with unconstrained agent in the corridor. This ensures that constrained agent can choose any path that do not leave corridor within constrained time.
%
%Target reasoning \citet{corridor} also uses constraint to force one agent only can reach its goal after conflict time or force all other agent do not visit the conflict goal location at or after conflict time. They are allowed to choose any path that satisfy these constraint.
%





==> K-Robust Symmetry Breaking (4)/temp.tex <==

% \def\year{2020}\relax
% %File: formatting-instruction.tex
% \documentclass[letterpaper]{article} % DO NOT CHANGE THIS
% \usepackage{aaai20}  % DO NOT CHANGE THIS
% \usepackage{times}  % DO NOT CHANGE THIS
% \usepackage{helvet} % DO NOT CHANGE THIS
% \usepackage{courier}  % DO NOT CHANGE THIS
% \usepackage[hyphens]{url}  % DO NOT CHANGE THIS
% \usepackage{graphicx} % DO NOT CHANGE THIS
% \usepackage{subcaption}
% \usepackage{amsthm}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \urlstyle{rm} % DO NOT CHANGE THIS
% \def\UrlFont{\rm}  % DO NOT CHANGE THIS
% \usepackage{graphicx}  % DO NOT CHANGE THIS
% \frenchspacing  % DO NOT CHANGE THIS
% \setlength{\pdfpagewidth}{8.5in}  % DO NOT CHANGE THIS
% \setlength{\pdfpageheight}{11in}  % DO NOT CHANGE THIS
% %\nocopyright
% %PDF Info Is REQUIRED.
% % For /Author, add all authors within the parentheses, separated by commas. No accents or commands.
% % For /Title, add Title in Mixed Case. No accents or commands. Retain the parentheses.
%  \pdfinfo{
% /Title (Symmetry Breaking $k$-Robust Multi-Agent Path Finding)
% /Author ()
% } %Leave this	
% % /Title ()
% % Put your actual complete title (no codes, scripts, shortcuts, or LaTeX commands) within the parentheses in mixed case
% % Leave the space between \Title and the beginning parenthesis alone
% % /Author ()
% % Put your actual complete list of authors (no codes, scripts, shortcuts, or LaTeX commands) within the parentheses in mixed case. 
% % Each author should be only by a comma. If the name contains accents, remove them. If there are any LaTeX commands, 
% % remove them. 

% % DISALLOWED PACKAGES
% % \usepackage{authblk} --This package is specifically forbidden
% % \usepackage{balance} --This package is specifically forbidden
% % \usepackage{caption} --This package is specifically forbidden
% % \usepackage{color (if used in text)
% % \usepackage{CJK} --This package is specifically forbidden
% % \usepackage{float} --This package is specifically forbidden
% % \usepackage{flushend} --This package is specifically forbidden
% % \usepackage{fontenc} --This package is specifically forbidden
% % \usepackage{fullpage} --This package is specifically forbidden
% % \usepackage{geometry} --This package is specifically forbidden
% % \usepackage{grffile} --This package is specifically forbidden
% % \usepackage{hyperref} --This package is specifically forbidden
% % \usepackage{navigator} --This package is specifically forbidden
% % (or any other package that embeds links such as navigator or hyperref)
% % \indentfirst} --This package is specifically forbidden
% % \layout} --This package is specifically forbidden
% % \multicol} --This package is specifically forbidden
% % \nameref} --This package is specifically forbidden
% % \natbib} --This package is specifically forbidden --use the following workaround:
% % \usepackage{savetrees} --This package is specifically forbidden
% % \usepackage{setspace} --This package is specifically forbidden
% % \usepackage{stfloats} --This package is specifically forbidden
% % \usepackage{tabu} --This package is specifically forbidden
% % \usepackage{titlesec} --This package is specifically forbidden
% % \usepackage{tocbibind} --This package is specifically forbidden
% % \usepackage{ulem} --This package is specifically forbidden
% % \usepackage{wrapfig} --This package is specifically forbidden
% % DISALLOWED COMMANDS
% % \nocopyright --Your paper will not be published if you use this command
% % \addtolength --This command may not be used
% % \balance --This command may not be used
% % \baselinestretch --Your paper will not be published if you use this command
% % \clearpage --No page breaks of any kind may be used for the final version of your paper
% % \columnsep --This command may not be used
% % \newpage --No page breaks of any kind may be used for the final version of your paper
% % \pagebreak --No page breaks of any kind may be used for the final version of your paperr
% % \pagestyle --This command may not be used
% % \tiny --This is not an acceptable font size.
% % \vspace{---No negative value may be used in proximity of a caption, figure, table, section, subsection, subsubsection, or reference
% % \vskip{---No negative value may be used to alter spacing above or below a caption, figure, table, section, subsection, subsubsection, or reference

% \frenchspacing
% \newcommand{\citet}[1]{\citeauthor{#1}~\shortcite{#1}}
% \newcommand{\citep}{\cite}
% \newcommand{\citealp}[1]{\citeauthor{#1}~\citeyear{#1}}
% \usepackage{latexsym}
% %\newcommand{\qed}{\hfill$\Box$}

% \newtheorem{theorem}{Theorem}

% %%%%%%% THIS MUST BE REMOVED BEFORE SUBMISSION!
% \usepackage{color}
% \newcommand{\pjs}[1]{\textcolor{blue}{PJS: #1}}
% \newcommand{\ddh}[1]{\textcolor{red}{DDH: #1}}
% \newcommand{\mike}[1]{\textcolor{green}{Mike: #1}}
% \renewcommand{\pjs}[1]{}
% \renewcommand{\ddh}[1]{}
% \renewcommand{\mike}[1]{}


% \newcommand{\ignore}[1]{}

% \setcounter{secnumdepth}{2} %May be changed to 1 or 2 if section numbers are desired.

% % The file aaai20.sty is the style file for AAAI Press 
% % proceedings, working notes, and technical reports.
% %
% \setlength\titlebox{2.5in} % If your paper contains an overfull \vbox too high warning at the beginning of the document, use this
% % command to correct it. You may not alter the value below 2.5 in


==> K_Corridor_Target.tex <==

\section{$k$-Robust Corridor Reasoning}

A \emph{corridor} from $B$ to $E$ is a chain of nodes $C$ where nodes in $C$ except $B$ and $E$
each have exactly two neighbours, 
and $B$ and $E$ have exactly one neighbour in $C$.
Figure~\ref{fig2:sub1} shows a corridor where $B = (3, 1)$, $C = \{ (1, 3), (2, 3),(3,3), (4, 3), (5, 3) \}$ and $E = (5, 3)$.
A \emph{corridor conflict}~\cite{corridor} 
occurs when two agents have a vertex or edge conflict occurring in a corridor.
In the example agents $a_1$ and $a_2$ conflict at vertex
(3, 3). 
Simply adding a vertex conflict constraint will not resolve the conflict, they will continue to
conflict in the corridor. \citet{corridor} introduce corridor symmetry breaking constraints which we extend here for $k$-delay conflicts.


The difference between corridor conflicts for $k$-robust CBS and normal corridor conflicts is that agents need to occupy vertexes for extra timesteps to avoid $k$-delay conflicts. Assuming there is a corridor with length of $l$ between vertex $B$ and vertex $E$, and a $k$-delay conflict in the corridor with agent $a_1$ ($a_2$) moving from $B$ to $E$ (resp. $E$ to $B$). Let $t_1$ (resp. $t_2$) be the earliest timestep when agent $a_1$ ($a_2$) is able to reach vertex $E$ (resp. $B$). 

Clearly when planning a $k$-robust solution, any path of $a_1$ using the corridor that reaches vertex $E$ at or before timestep $t_2+l+k$ must conflict with any paths of $a_2$ using the corridor that reach vertex $B$ at or before timestep $t_1+l+k$. But there may be alternate paths the agents can take to reach $B$ or $E$.
Assuming agent $a_1$ can reach vertex $E$ at timestep $t'_1$ without using the corridor 
and reach vertex $B$ at timestep $t_b$. Agent $a_2$ can reach vertex $B$ at timestep $t'_2$ without traversing the corridor and reach vertex $E$ at timestep $t_e$. 
Hence in planning a $k$-robust solution, any path of $a_1$ that reaches vertex $E$ at or before timestep $min( max(t_e + k, t'_1 - 1), t_2  + l+k)$ must conflict with any path of $a_2$ that reaches vertex $B$ at or before timestep $min( max(t_b + k, t'_2  - 1),t_1  + l+k)$.

Hence the constraint $\langle a_1,E,[0,min( max(t_e + k, t'_1 - 1), t_2  + l+k)] \rangle \vee \langle a_2,B,[0,min( max(t_b + k, t'_2  - 1),t_1  + l+k)] \rangle$ must hold in all solutions. 
To handle the corridor constraint we branch on this disjunction. Clearly


\begin{theorem}$k$-robust Corridor Reasoning is correct.
\qed
\end{theorem}
\ignore{
\begin{proof}
We have shown that if $a_1$ and $a_2$ both violate constraint $<a_1,E,[0,min(t'_1  - 1+k,t_2  + l+k)]>$ and constraint $<a_2,B,[0,min(t'_2  - 1+k,t_1  + l+k)]>$, they must have a conflict in the corridor. Thus the adding of these constraints will not eliminate any conflict free $k$-robust solution, and will eliminate the current paths.
\end{proof}
}

\section{$k$-Robust Target Reasoning}

A \emph{target conflict}~\cite{corridor} occurs when one agent $a_2$ reaches its goal vertex $g_2$ at timestep $l$, and another agent $a_1$ conflicts with agent $a_2$ at vertex $g_2$ at some later timestep 
$t, t \geq l$.  
Consider Figure~\ref{fig2:sub2} where agent $a_2$ reaches its goal cell (4,2) at timestep 1, and then agent $a_1$ tries to traverse cell (4,2) at timestep 3.  Simply adding the constraint
$\langle a_1,(4,3),[3,3] \rangle$ causes $a_1$ to wait before entering 
cell (4,3) at timestep 4 and then the conflict reoccurs.

To avoid this ~\citet{corridor} resolve the conflict by branching on $et_2 \leq t \vee et_2 > t$
where $et_2$ is the end time for agent $a_2$. In the first case, since agent $a_2$ finishs before or at timestep $t$, agent $a_1$ can never use location $g_2$ at timestep $t$ or after. In the second case agent $a_2$ cannot finish before timestep $t+1$ freeing up the location for agent $a_1$. 

Planning a $k$-robust solution requires the avoiding of $k$-delay conflict. 
Therefore, we branch on $et_2 \leq t+k \vee et_2 > t + k$. The first case forces agent $a_2$ to finish
before timestep $t+k$ preventing agent $a_1$ (or any other agent) from using vertex $g_2$ at timestep $t$, the second case
forces agent $a_2$ not to finish earlier so vertex $g_2$ at timestep $t$ is freed up for agent $a_1$. Again clearly

\begin{theorem}
$k$-Robust Target Reasoning is correct.
\ignore{
\begin{proof}
The disjunction we branch on clearly removes no solutions, and since each disjunct makes one of current paths infeasible, it progresses the search.
\end{proof}}
\qed
\end{theorem}

Note that to handle target symmetries we have to update the low-level path finder for agents to take into account new kinds of constraints where we restrict the end time of an agent, and where we prevent any agent from using a location from some time point onwards. Both are straightforward additions. See~\citet{corridor} for details.



==> Makefile <==
FICHIER = main

TEXFILES = $(wildcard *.tex) $(wildcard images/*.tex) $(wildcard algo/*.tex) $(wildcard tikz/*.tex) 
BIBFILE  = $(wildcard *.bib)
FIGFILES = $(wildcard images/*.fig)
EPSFILES = $(patsubst %.fig,%.eps,$(FIGFILES))

TMPFILES  = $(wildcard *.aux) $(wildcard *.bbl) $(wildcard *.ps) $(wildcard *.dvi) $(wildcard *.blg) $(wildcard *.toc) $(wildcard *.lof) $(wildcard *.log) $(wildcard *.lot) 
BACKFILES = $(wildcard *.bak) $(wildcard */*.bak) $(wildcard *~) $(wildcard */*~) $(wildcard *.tar.gz)
TRUCFILES = $(wildcard _*)

DOTFILES = $(wildcard *.dot)
PSDOTFILES = $(patsubst %.dot,%.tps,$(DOTFILES))

all: $(FICHIER).pdf

%.pdf: $(TEXFILES)
	pdflatex $(FICHIER)
	if grep -q 'citation' $(FICHIER).aux; then if grep -q 'bibdata' $(FICHIER).aux; then bibtex $(FICHIER); fi else rm -f $(FICHIER).bbl; fi
	pdflatex $(FICHIER) 
	pdflatex $(FICHIER)

#%.pdf: %.ps
#	ps2pdf $<

#%.tps: %.dot
#	dot -Tps -o $@ $<

%.ps:  %.dvi
	dvips -o $@ $< > /dev/null
#	dvips -Pcmz -Pamz -o $@ $< > /dev/null

%.eps: %.fig
	fig2dev -L eps $< $@

%.dvi: _tpsfiles _epsfiles $(TEXFILES)
	pdflatex $(FICHIER)
	if grep -q 'citation' $(FICHIER).aux; then if grep -q 'bibdata' $(FICHIER).aux; then bibtex $(FICHIER); fi else rm -f $(FICHIER).bbl; fi
	pdflatex $(FICHIER) > /dev/null
	pdflatex $(FICHIER) > /dev/null

_tpsfiles: $(PSDOTFILES)
	touch _tpsfiles

%.tps: %.dot
	dot -Tps -o $@ $<

_epsfiles: $(EPSFILES)
	@echo $(EPSFILES) > _epsfiles

clean:
	-rm -f $(EPSFILES) $(BACKFILES) $(PSDOTFILES)
	-rm -f $(TMPFILES)
	-rm -f $(TRUCFILES)
	-rm -f $(FICHIER).pdf

tar: clean
	perl -e '$$line=`date +"\%y-\%m-\%d"`;chomp($$line);`tar cvf $(FICHIER)-$$line.tar *`;`gzip $(FICHIER)-$$line.tar`;';

tardir: clean
	perl -e '$$pwd = `pwd`; my($$path,$$dir) = $$pwd =~ m/(.*\/)(.*)$$/; $$line=`date +"\%y-\%m-\%d"`;chomp($$line);`cd .. ; tar cvf $$dir-$$line.tar $$dir ; gzip $$dir-$$line.tar ; mv $$dir-$$line.tar.gz $$dir`;';

pwd:
	perl -e '$$pwd = `pwd`; print $$pwd;'

touch:
	@touch $(FICHIER).tex
	@echo You touch my ``$(FICHIER)''.

open:
#	@kile $(FICHIER).tex &
#	@texmaker $(FICHIER).tex &
	@emacs $(FICHIER).tex &





==> back.tex <==
Proof. Now let’s assume that there is a K-Delay conflict $<a_i, a_j,v, t, \Delta>$ with agent $a_i$ at timestep $t$ and $a_j$ at timestep $t+\Delta, \Delta \in [0, k]$. If $a_i$ and $a_j$ satisfy requirements, which means they all follow their Manhattan optimal paths, then:
\[t_j-t_i=\Delta\]
\[(|v.x-S_j.x|+|v.y-S_j.y|)-(|v.x-S_i.x|+|v.y-S_i.y|)=\Delta\]
\[|v.x-S_j.x|-|v.x-S_i.x|+|v.y-S_j.y|-|v.y-S_i.y|=\Delta\]
If $a_i$ and $a_j$ satisfy requirement b, which means they are moving towards the same direction, then:
\[(v.x-S_i.x)(v.x-S_j.x) \geq 0\]
\[(v.y-S_i.y)(v.y-S_j.y) \geq 0\]
Then, assume $a_i$ and $a_j$ are moving towards the direction that for any vertex $v_a$ in the optimal path of $a_i$ or $a_j$:
\[v_a.x-S_i.x\geq0,v_a.x-S_i.y\geq0\] or \[v_a.x-S_j.x\geq0,v_a.x-S_j.y \geq 0\]
As the problem is invariant with the rotations of direction, this assumption does not lose generality (Li et al., 2019b). 
Then:
\[(v.x-S_j.x)-(v.x-S_i.x)+(v.y-S_j.y)-(v.y-S_i.y) = \Delta\]
\[S_i.x-S_j.x+S_i.y-S_j.y = \Delta\]
for any intersection vertex $v’$ of optimal paths of $a_i$ and $a_j4$:
\[t_j' =|v'.x-S_j.x|+|v'.y-S_j.y|\]
\[t_i' =|v'.x-S_i.x|+|v'.y-S_i.y|\]
\[t_j'-t_i' =|v'.x-S_j.x|+|v'.y-S_j.y|-|v'.x-S_i.x|-|v'.y-S_i.y|\]
\[t_j'-t_i' =|v'.x-S_j.x|-|v'.y-S_i.x|+|v'.y-S_j.y|-|v'.x-S_i.y|\]
As $a_i$ and $a_j$ satisfy requirement $b$, then:
\[(v'.x-S_i.x)(v'.x-S_j.x) \geq 0\]
\[(v'.y-S_i.y)(v'.y-S_j.y) \geq 0\]
As $a_i$ and $a_j$ are moving towards the direction assumed above, Then
\[t_j' -t_i'=(v'.x-S_j.x)-(v'.y-S_i.x)+(v'.y-S_j.y)-(v'.x-S_i.y)\]
\[t_j' -t_i'=S_i.x-S_j.x+S_i.y-S_j.y \]
\[t_j' -t_i'=\Delta\]
As $\Delta \in [0, k]$, then $a_i$ and $a_j$ have a K-Delay conflict at $v’$.
If $a_i$ and $a_j$ also satisfy requirement c, then all optimal path of $a_j$ and $a_j$ always intersect within the rectangle area, and for any intersection vertex $v’$, $a_i$ and $a_j$ have a K-Delay conflict at $v’$. 
Thus, if $a_i$ and $a_j$ have a K-Delay conflict and satisfy all three requirements, $a_i$ and $a_j$ have K-Delay cardinal rectangle conflicts

==> k_symmetries.tex <==
\section{$k$-Robust Rectangle Reasoning}

%$k$-Robust rectangle conflicts occur when 
%two agents arrive in a rectangle area such as Figure~\ref{fig1} (left);
%not just at the same time but also within $k$ timesteps of one another.
The simplest type of rectangle conflict, called CR in~\cite{li2019},
can be understood as follows:
\begin{itemize}
\item[(a)] Both agents follow their Manhattan optimal paths from start to goal. 
\item[(b)] Both agents move in the same direction in all dimensions.
\item[(c)] The start and goal nodes of two agents have relative opposite locations. This requirement ensures that all optimal paths of both agents intersect within the rectangle area.
\end{itemize}

The situation is shown in Figure~\ref{fig1} (left). The only difference between $k$-delay rectangle conflicts and 
$k=0$ is that the agents can arrive at the same vertex in the rectangle area at different timestep. 
To resolve such conflicts we introduce \textbf{Temporal Barrier Constraints}, which unify
the (temporal) range constraints of~\cite{atzmon} and the (spatial) Barrier Constraints of~\cite{li2019}.

%Thus if two agents have a $k$-delay conflict satisfy requirements (a), (b), and (c), they have $k$-delay cardinal rectangle conflicts.

%\subsection{Temporal Barrier Constraints}

%We combine the concept of symmetry range constraint \citet{atzmon} and barrier constraint\citet{li2019} to resolve $k$-delay rectangle conflicts. This new constraint is called the \emph{temporal barrier constraint}.

\begin{defn}
Given a vertex time pair p = (S,t) the \emph{optimal time} 
$ot(p,v)$ to reach 
vertex $v = (v_x,v_y)$ starting from $S = (S_x,S_y)$ at time $t$ is
calculated by adding the Manhattan distance 
$ot(p,v) = t + |v_x - S_x| + |v_y - S_y|$.

A \emph{temporal barrier constraint} is denoted by
$B(a_x, V, p, \Delta)$. 
This constraint forbids the 
agent $a_x$ from visiting any vertex $v \in V$ 
at the optimal time from vertex time pair $p$, or any time step up to $\Delta$ later. 
That is the barrier constraint $B(a_x, V, p, \Delta)$ 
is the set of time-range vertex constraints
$\langle a_x, v, [ot(p,v), ot(p,v) + \Delta] \rangle, v \in V$.
\label{defi:barrier}
\end{defn}

%Figure~\ref{mike-fixme} shows an example. 
Figure~\ref{fig3}(b) shows the example that $a_i$ is blocked by temporal barrier constraint and does not have a $k$-delay conflict anymore.
\ddh{Mike, please fix this example. The diagram should be one picture showing a k-delay conflict and a temporal barrier}\mike{got it}
%Here $a_i$ and $a_j$ have a conflict $(a_i, a_j, v, t, \Delta)$, meaning $a_i$ arrives at $v$ at timestep $t$ and $a_j$ arrives at $v$ at timestep $t+\Delta$. We resolve this conflict with temporal barrier constraints 
%$B(a_i, R_i, R_g, k,0)$ and $B(a_j, R_i, R_g, k,\Delta)$.  

\subsection{Extended Rectangle Area}

\begin{figure}
\centering
\begin{subfigure}{0.48\columnwidth}
  \centering
  \includegraphics[width=0.9\columnwidth]{rectangle.jpg}
  \caption{Rectangle Conflict}
  \label{fig4:sub1}
\end{subfigure}
\begin{subfigure}{0.48\columnwidth}
  \centering
  \includegraphics[width=0.9\columnwidth]{extendedb.jpg}
  \caption{Temporal barrier constraint use start-goal rectangle border eliminate all conflicts and orange area}
  \label{fig4:sub2}
\end{subfigure}
\caption{Extended rectangle area and temporal barrier constraint when k=2. Red numbers are timesteps that $a_j$ reach each vertex. Green numbers for $a_i$. Grey cells are constrained vertexes with constrained timesteps. Orange and yellow area means all paths will conflict in these area. For unconstrained agents these numbers are optimal time they can arrive each location. For constrained agents, numbers are latest time they can reach each vertex.   }
\label{fig4}
\end{figure}

The aim of introducing a temporal barrier constraint is to force the optimal cost of constrained agent to increase by $1+k-delay$. 
However, when $k \geq 2$, the temporal barrier constraint with $B(a_x, R_x, R_g, k, delay)$ failed. As shown in Figure \ref{fig4:sub1}, when $k=2$, temporal barrier constraint $B(a_i,(4,4),(4,5),2,0)$ is used to force $a_i$’s optimal path to increase by 3, to a length of 9, to avoid the conflict with $a_j$. 
However, the cost of optimal paths of agent $a_i$ is still 8, 
because $a_i$ can bypass the temporal barrier constraint. In this case, all paths of $a_i$ with cost 8 conflict with all the optimal paths of $a_j$ in the light yellow area, which is larger than the rectangle. 

The light yellow area is an extended rectangle area. Each time $k$ increased by 2, constrained agent need to find a path with 2 more cost. This makes CBS can choose a wider path with 2 more cost that bypass rectangle area, which means the size of the extended rectangle area increased.

Once $k$ is big enough to force the agent to bypass the unconstrained agent’s start-goal rectangle, the optimal path of constrained agents will no longer intersect with unconstrained agent’s optimal path. Thus the extended rectangle area is at most the unconstrained agent’s start-goal rectangle. 

\subsection{$k$-Robust Cardinal Rectangle Reasoning}

One approach to overcome the above problem is to use the border of the extended rectangle area to define a temporal barrier constraint. 
We use a simpler method which extends the border of unconstrained agent’s start and goal rectangle as the barrier in order to to overcome this problem. Figure \ref{fig4:sub2} shows the latest timestep that $a_i$ can arrive at each vertex in the rectangle area when trying to reach the goal at timestep 9. 
In this case, the low-level search of $a_i$ has many options for reaching 
the goal at timestep 9 without conflicting with the optimal paths of agent $a_j$.  Figure \ref{fig4:sub3} shows the CT tree when solving rectangle conflicts with temporal range constraints. We denote the temporal barrier constraint using the border of unconstrained agent’s start and goal rectangle as $B(a_x, Rs_x, Rg_x, k, delay), x \in [ i, j ]$. 
$Rs_x$ and $Rg_x$ are the two corner nodes of the border of the start-goal rectangle that are opposite to $a_x$’s start location $s_x$. 
We call the algorithm using the extended
temporal border constraint $B(a_x, Rs_x, Rg_x, k, delay), x \in [ i, j ]$ to resolve $k$-delay cardinal rectangle conflict as \textbf{K-CBSH-CR}.

Using the border of unconstrained agent’s start and goal rectangle will introduce some redundant constraints. But they do not over constrain the target agent. Using the example in Figure \ref{fig4:sub2}, if the $k=2$ and 
vertex (4,2) is constrained at timesteps 1, 2, and 3, since the earliest timestep that the constrained agent can arrive at (4,2) is 5 this does remove any possible paths for the agent.
Similarly while vertex (6,7) is constrained at timesteps 6, 7, and 8; paths for $a_i$ to reach the goal through (6,7) have a cost of at least 10, and hence no possible paths are removed. 

\textbf{Property 1.} For any path combination of two agents $a_i$ and $a_j$ that have $k$-delay cardinal rectangle conflict (assuming $a_i$ arrives rectangle area $\Delta$ timestpes early than $a_j$). If one path violates $B(a_i, Rs_i, Rg_i, k,0)$ and the other path violates $B(a_j, Rs_j, Rg_j, k,\Delta)$, then the two agents have $k$-delay conflict within the rectangle area.

\textit{Proof.} 
If the optimal time that agent $a_i$ can arrive vertex $N_i$ on border $Rs_i$ to $Rg_i$ is $c_i$.  Now $a_i$ arrives at $N_i$ at $t_i$, $c_i \leq t_i \leq c_i+k$ and $d_i=t_i-c_i$ ($d_i$ is the timestep difference between the timestep that $a_i$ arrive $N_i$ and the optimal timestep that $a_i$ can arrive $N_i$), hence $a_i$ violates constraint $B(a_i, Rs_i, Rg_i, k,0)$.

If the optimal time that agent $a_j$ can arrive vertex $N_j$ on border $Rs_j$ to $Rg_j$ is $c_j$ and the optimal time that agent $a_i$ can arrive vertex $N_j$ is $c_{i\_nj}$. Hence the timestep difference that two agents optimally arrive a vertex in rectangle area is $\Delta$, $c_{i\_nj} + \Delta = c_j$ and $c_{i\_nj}\leq c_j$. 
Now the $a_j$ arrive $N_j$ at $t_j$, and $c_{i\_nj}\leq c_j\leq t_j\leq c_j-\Delta + k = c_{i\_nj}+k$, hence $a_j$ violate $B(a_j, Rs_j, Rg_j, k,\Delta)$. $d_j=t_j-c_j$, which is the timestep difference between $t_j$ and $c_j$.

The requirement (c) in section 5.1 guarantees that the path of $a_i$ and the path of $a_j$ must have an intersect vertex, which means they both traverse a vertex at same or different timestep. The intersection vertex in denoted as $v$. 

The optimal time that $a_i$ arrive $v$ is $c_{i\_v}$, which is also the earliest time that $a_i$ can arrive $v$. 

The optimal time that $a_j$ can arrive $v$ is $c_{j\_v}$ and the latest time that $a_j$ can arrive $v$ is $c_{j\_v}+d_j$. 

As agent $a_i$ and $a_j$ have $k$-delay rectangle conflicts and the optimal path of $a_i$ arrive rectangle area early than $a_j$, thus $c_{j\_v}-c_{i\_v}=\Delta$ and $\Delta \leq k$. 

Because $t_j\leq c_{i\_nj}+k$:
\[t_j-c_j\leq c_{i\_nj}+k-c_j\]
\[d_j\leq c_{i\_nj}+k-c_j\]
As $a_i$ and $a_j$ have $k$-delay rectangle conflicts, the time difference that two agents' optimal path arrive any vertex in rectangle conflicts is $\Delta$ and also because of $c_{i\_nj}\leq c_j$:
\[d_j\leq -\Delta+k\]
\[d_j+\Delta\leq k\]
Thus 
\[d_j+c_{j\_v}- c_{i\_v} \leq k\]
Hence $d_j+c_{j\_v}$ is the latest time that $a_j$ can arrive vertex $v$ and $c_{i\_v}$ is the earliest time that $a_i$ can arrive $v$, the time difference between the latest time that $a_j$ can arrive $v$ and the earliest time that $a_i$ can arrive $v$ is always smaller than k, which means have a $k$-delay conflict between $a_i$ and $a_j$ at $v$.

Therefore if $a_i$ and $a_j$ have $k$-delay rectangle conflicts, one path violates $B(a_i, Rs_i, Rg_i, k,0)$ and the other path violates $B(a_j, Rs_j, Rg_j, k,\Delta)$, then the two agents have $k$-delay conflict within the rectangle area.
\qed

\mike{Sketch of proof}
\textit{Proof Sketch.} 
The requirement (c) in section 5.1 guarantees that the path of $a_i$ and the path of $a_j$ must have an intersect vertex $v$ if both agents traverse each other's start and goal rectangle. 

Assuming the optimal time that agent $a_i$ can arrive vertex $N_i$ on border $Rs_i$ to $Rg_i$ is $c_i$ and the real time $a_i$ arrives at $N_i$ is $t_i$, $c_i \leq t_i \leq c_i+k$ and $d_i=t_i-c_i$.

Assuming the optimal time that agent $a_j$ can arrive vertex $N_j$ on border $Rs_j$ to $Rg_j$ is $c_j$ and the optimal time that agent $a_i$ can arrive vertex $N_j$ is $c_{i\_nj}$. Hence the timestep difference that two agents optimally arrive a vertex in rectangle area is $\Delta$, $c_{i\_nj} + \Delta = c_j$ and $c_{i\_nj}\leq c_j$. Assuming the real time the $a_j$ arrive $N_j$ is $t_j$, $c_{i\_nj}\leq c_j\leq t_j\leq c_j-\Delta + k = c_{i\_nj}+k$, and $d_j=t_j-c_j$.

Assuming the optimal time (earliest time) that $a_i$ can arrive $v$ is $c_{i\_v}$. 

Assuming optimal time that $a_j$ can arrive $v$ is $c_{j\_v}$, the latest time that $a_j$ can arrive $v$ is $c_{j\_v}+d_j$. 

As $a_i$'s optimal path have $k$-delay conflict with $a_j$'s optimal path, we know $c_{j\_v}-c_{i\_v}=\Delta$.

With these information, we can prove that $c_{j\_v}+d_j - c_{i\_v}$ always smaller than k, which means we have a $k$-delay conflict at $v$.
\qed


\subsubsection{Theorem 1.} K-CBSH-CR is complete and optimal.

\textit{Proof.}  The proof is similar to the proofs in \citet{atzmon} and \citet{li2019}.  
If $a_i$ and $a_j$ have a conflict $(a_i, a_j, v, t, \Delta$. For a CT node $N$, $N1$ and $N2$ are the child nodes for $N$. $N1$ hold the constraint $B(a_i, Rs_i, Rs_i, k,0)$ and $N2$ hold the constraint $B(a_j, Rs_j, 
Rs_j, k,\Delta)$. $\pi(N1)$ denotes all the $k$-Robust plans that satisfy $N1.constraints$ and $\pi(N2)$ denotes all the $k$-Robust plans that satisfy $N2.constraints$. Based on property 1, the temporal barrier constraint does not eliminate any conflict-free solutions. Thus $\pi (N) =  \pi (N1) \cup \pi (N2)$. Thus K-CBSH-CR does not eliminate any possible solution and is complete. Furthermore, the low-level search of any kind of CBS always returns an optimal path, the high-level search always chooses a CT node with minimum $f$-value to expand and K-CBSH-CR does not eliminate any possible solution when splitting. Therefore, the first chosen CT node whose paths are conflict-free has a set of conflict-free paths with minimum cost. Thus K-CBSH-CR is optimal.
\qed

\subsection{Extending $k$-Robust Rectangle Reasoning}

\citet{li2019} shows that rectangle reasoning can also be used to resolve semi-cardinal rectangle conflict and non-cardinal rectangle conflicts, not only cardinal rectangle conflicts. This algorithm is called CBSH-R. As the 
barrier constraints only block paths that traverse the rectangle area and do not block all optimal paths for semi-cardinal or non-cardinal rectangle conflicts, it may fail to resolve some conflicts. CBSH-R needs to esnure 
the barrier constraint resolves the current conflict so that it cannot
arise in the current node’s ancestors.  By replacing the barrier constraint with a temporal barrier constraint using the border of the unconstrained agent’s start-goal rectangle, CBSH-R is modified to plan $k$-Robust solutions and we denote this algorithm \textbf{K-CBSH-R}. 

\textbf{Theorem 2.} K-CBSH-R is complete and optimal.

\textbf{Proof.} As temporal barrier constraint for $a_i$ will not block any path that does not traverse $a_j$’s start goal rectangle, thus temporal barrier constraint for $a_i$ will not block any path that does not intersect with $a_j$’s path. Therefore Property 1 still holds for K-CBSH-R. Thus the proof in Theorem 1 still works for K-CBSH-R, which means K-CBSH-R also is complete and optimal. \qed

\subsubsection{Rectangle Conflict in Path Segments}
\citet{li2019} further extends the usage of barrier constraints and use it to solve rectangle conflicts caused by obstacles and other constraints. It uses a Multi-Valued Decision Diagram (MDD) (Sharon et al. 2013), which is a directed acyclic graph, to find singletons in the paths of each agent. An MDD stores all possible locations at each timestep for an agent to reach its goal optimally, which is the same as storing all optimal paths of an agent. If a timestep only has one possible location, which means all optimal paths must traverse this location at this timestep, this location at this time step is called a singleton. This algorithm uses all the singletons from conflict agents’ paths as candidate start and goal locations and then CBSH-RM try to find and classify rectangle conflicts in all possible start and goal combinations. When multiple conflicts exist, CBSH-RM first prefers rectangle conflicts with higher priority type, then it prefers a larger rectangle area. 

For $k$-delay rectangle conflicts, current conflict detection tie braking policy cannot efficiently resolve all problems, as the rectangle conflicts does not consider extended rectangle area. Thus, for $k$-Robust plan, the rectangle conflicts with larger extended rectangle area are preferred when two rectangle conflicts have the same priority type and rectangle area.\

\subsubsection{Adding Temporal Barrier Constraint}
\citet{li2019} also find that if blocking all vertexes on the border of the rectangle opposite the constrained agent, CBSH-RM may lose optimality. Because when barrier constraint force the agent to reach the goal with a higher cost, it is possible that alternative paths, which do not traverse selected start singleton but traverse constrained barrier vertexes. Blocking all vertexes on the border of the rectangle area loses these path choices. By using MDD for each agent in conflict, CBSH-RM avoid losing optimality by checking does any optimal path of constrained agent traverse the vertexes included in barrier constraint and if no any optimal path traverse a vertex, this vertex will not be constrained.

$k$-Robust rectangle reasoning requires to block the extended rectangle area as well. Although the MDD provides the information of all optimal paths of an agent, these optimal paths do not traverse extended rectangle area. Therefore, if the optimal cost from selected start singleton to selected goal singleton is $c$, an MDD of constrained agent stores all paths from selected start singleton to selected goal singleton with a cost of $c+k$ is used to support the adding of temporal barrier constraint. An MDD with the cost of $c+k$ contains all paths with cost $i,  c\leq i \leq c+k$, as a path with cost i can become a path with cost c+k by waiting at goal location.

For any vertex $v$ in the border of extended rectangle area opposite to constrained agent, if the optimal time that the agent arrives at the vertex is $t$ , the time that the agent arrive selected start singleton is $t_s$, and the level $(t-t_s) +i,i\in (0,k)$, of the MDD include vertex $v$, $v$ is constrained from time $t+i$ to $t +k$. By constraint the vertexes only exist in MDD Property 1 still holds here. This algorithm is denoted as K-CBSH-RM.

\mike{A shorten version:} \citet{li2019} shows that rectangle reasoning can also be used to resolve semi-cardinal rectangle conflict and non-cardinal rectangle conflicts, not only cardinal rectangle conflicts. By replacing the barrier constraint with a temporal barrier constraint, it is modified to plan $k$-Robust solutions and we denote this as \textbf{K-CBSH-R}. \citet{li2019} further extends the usage of barrier constraints and use it to solve rectangle conflicts caused by obstacles and other constraints. It uses a Multi-Valued Decision Diagram (MDD) (Sharon et al. 2013), which is a directed acyclic graph, to find singletons in the paths of each agent. An MDD stores all possible paths of an agent at a certain cost. If a timestep only has one location, which means all paths traverse this location at this timestep, it is called a singleton. This algorithm uses all the singletons from conflict agents’ paths as candidate start and goal locations and then CBSH-RM try to find rectangle conflicts in all possible start and goal combinations. By replacing barrier constraint with temporal constraint, it works for planning $k$-robust solution and is denoted as \textbf{K-CBSH-RM}.



\section{$k$-Robust Corridor Reasoning}
The difference between corridor conflict with $k$-Robust CBS and normal corridor conflict is that agents need to occupy vertexes for extra timesteps to avoid $k$-delay conflicts. Assume there is a corridor conflict with a length of $l$ between vertex $b$ and vertex $e$. Agent $a_1$ moving from $b$ to $e$ and agent $a_2$ moving from $e$ to $b$. If the agent $a_1$ reach vertex $e$ at timestep $t_1$ and agent $a_2$ reach vertex $b$ at timestep $t_2$.For planning $k$-Robust solution, any path of $a_1$ that reach vertex $e$ at or before timestep $t_2+l+k$ must conflict with any paths of $a_2$ that reach vertex $b$ at or before timestep $t_1+l+k$.

When considering bypasses, assuming agent $a_1$ can reach vertex $e$ at timestep $t'_1$ and agent $a_2$ reach vertex $b$ at timestep $t'_2$ without traverse the corridor. Therefore for planning $k$-Robust solution, any path of $a_1$ that reach vertex $e$ at or before timestep $min(t'_1  - 1+k,t_2  + l+k)$ must conflict with any paths of $a_2$ that reach vertex $b$ at or before timestep $min(t'_2  - 1+k,t_1  + l+k)$.

Therefore, a pair of range constraint is used to perform $k$-Robust corridor reasoning. When splitting CT node, child node 1 hold the constraint $<a_1,e,[0,min(t'_1  - 1+k,t_2  + l+k)]>$ and child node 2 hold the constraint $<a_2,b,[0,min(t'_2  - 1+k,t_1  + l+k)]>$.

\textbf{Theorem 2.} $k$-Robust Corridor Reasoning is complete and optimal.

\textit{Proof} We have shown that if $a_1$ and $a_2$ both violate constraint $<a_1,e,[0,min(t'_1  - 1+k,t_2  + l+k)]>$ and constraint $<a_2,b,[0,min(t'_2  - 1+k,t_1  + l+k)]>$, they must have a conflict in the corridor. Thus the adding of these constraints will not eliminate any conflict free $k$-Robust solution. Thus $k$-Robust Corridor Reasoning is complete. $k$-Robust Corridor Reasoning is based on CBS, as proved in Theorem 1, CBS guarantees that the solution is optimal as long as no conflict free solution is eliminated.

\section{$k$-Robust Target Reasoning}
Assuming that agent $a_i$ reaches its goal $g_i$ on timestep $l$, and agent $a_j$ has a target conflict with the agent $a_i$ at $g_i$ on timestep $t,t \geq l$. All solutions that both $a_i$ and $a_j$ visit $g_i$ at $t$ must have conflict. ~\citet{corridor} resolve target conflict by force $a_i$ to reach its goal after $t$ or force any other agent visit $g_i$ at or after $t$. Planning $k$-Robust solution requires the avoiding of $k$-delay conflict. Therefore, when splitting, one child node forces $a_i$ to reach its goal after $t+k$ to give $a_2$ priority and do not cause $k$-delay conflict. Another child node forbids any other agent visit $g_i$ at or after $t$ to force all other agents find bypasses to their goal locations. If any agent failed to find a bypass route, we do not generate this child node. 

\textbf{Theorem 3.} $k$-Robust Target Reasoning is complete and optimal.

\textit{Proof} We have shown that target reasoning only eliminate the solutions that have target conflict and do not eliminate any conflict free solution. Thus $K$-robust Target Reasoning is complete. $k$-Robust Target Reasoning is based on CBS. As proved in Theorem 1, CBS guarantees that the solution is optimal as long as no conflict free solution is eliminated.

%%%%%%%%% OLD OLD OLD OLD  %%%%%%%%%%%%%%%%%%%%%
%\subsection{Identifying $k$-delay Cardinal Rectangle Conflicts}
%
%\citet{li2019} introduced an algorithm to identify cardinal rectangle conflicts for CBSH-CR. If agent $a_i$ and $a_j$ have a conflict $<a_i, a_j, v, t>$, $S_i$, $G_i$ are start and goal nodes for $a_i$ and $S_j$, $G_j$ are start and goal nodes for $a_j$, 
%if they satisfy following requirements, they have cardinal rectangle conflict. Requirements are:
%\begin{itemize}
%\item[(a)] Both agents follow their Manhattan optimal paths from start to goal. 
%\item[(b)] Both agents move in the same direction in all dimensions.
%\item[(c)] Start and goal nodes of two agents have relative opposite locations. This requirement ensures that all optimal paths of both agents intersect within the rectangle area.
%\end{itemize}
%The only difference for $k$-delay rectangle conflicts is that the 
%agents can arrive at the same vertex in the rectangle area at different timestep. Thus if two agents have a $k$-delay conflict satisfy requirements (a), (b), and (c), they have $k$-delay cardinal rectangle conflicts.
%
%\subsection{Temporal Barrier Constraints}
%\begin{figure}
%\centering
%\begin{subfigure}{0.48\columnwidth}
%  \centering
%  \includegraphics[width=1\columnwidth]{rectangle.jpg}
%  \caption{Rectangle Conflict. }
%  \label{fig3:sub1}
%\end{subfigure}
%\begin{subfigure}{0.48\columnwidth}
%  \centering
%  \includegraphics[width=0.98\columnwidth]{temporalBarrier.jpg}
%  \caption{Temporal barrier constraints for $a_i$. }
%  \label{fig3:sub2}
%\end{subfigure}
%\caption{Examples of rectangle conflicts and barrier constraints when k=1. The green numbers are timesteps that agent $a_i$ reach each vertex. The red numbers are timesteps that $a_j$ reach each vertex. Grey cells are constrained vertexes and black numbers are constrained timesteps for constrained vertexes. Orange area means all paths will conflict in this area. For unconstrained agents these numbers are optimal time they can arrive each location. For constrained agents, numbers are latest time they can reach each vertex.}
%\label{fig3}
%\end{figure}
%
%We combine the concept of symmetry range constraint \citet{atzmon} and barrier constraint\citet{li2019} to resolve $k$-delay rectangle conflicts. This new constraint is called the \emph{temporal barrier constraint}.
%
%\textbf{Definition 1}  A  \emph{temporal barrier constraint} is denoted by $B(a_x, R_x, R_g, k, delay), x \in [ i, j ]$. It forbids the agent $a_x$ from visiting any vertex $v_n$ within $R_x$ to $R_g$ area (the rectangle area border that is opposite to $a_x$) from timestep $t - delay$, where $t$ is the earliest time that agent $a_x$ can arrive vertex $v_n$, to timestep $t-delay + k$. The variable $delay$ is used to note the timestep difference between agents in the $k$-delay conflict. For the agent (say $a_i$) that arrives rectangle first, $delay = 0$. For the agent (say $a_j$) arrives rectangle second, $delay$ is the timestep difference that agents arrive at conflict vertex $v$.
%
%Assume $a_i$ and $a_j$ have a conflict $(a_i, a_j, v, t, \Delta)$, meaning $a_i$ arrives at $v$ at timestep $t$ and $a_j$ arrives at $v$ at timestep $t+\Delta$. We resolve this conflict with temporal barrier constraints 
%$B(a_i, R_i, R_g, k,0)$ and $B(a_j, R_i, R_g, k,\Delta)$.  
%Figure~\ref{fig3}(b) shows the example that $a_i$ is blocked by temporal barrier constraint and does not have a $k$-delay conflict anymore.
%
%\subsection{Extended Rectangle Area}
%
%\begin{figure}
%\centering
%\begin{subfigure}{0.48\columnwidth}
%  \centering
%  \includegraphics[width=0.9\columnwidth]{extendeda.jpg}
%  \caption{Normal barrier constraint failed, the orange area still exists.}
%  \label{fig4:sub1}
%\end{subfigure}
%\begin{subfigure}{0.48\columnwidth}
%  \centering
%  \includegraphics[width=0.9\columnwidth]{extendedb.jpg}
%  \caption{Temporal barrier constraint use start-goal rectangle border eliminate all conflicts and orange area}
%  \label{fig4:sub2}
%\end{subfigure}
%\begin{subfigure}{0.8\columnwidth}
%  \centering
%  \includegraphics[width=1\columnwidth]{extendedc.jpg}
%  \caption{The CT tree for resolving $k$-delay rectangle conflicts with temporal barrier constraints using start-goal rectangle border.}
%  \label{fig4:sub3}
%\end{subfigure}
%\caption{Extended rectangle area and using the start-goal border for temporal barrier constraint when k=2.   }
%\label{fig4}
%\end{figure}
%
%The aim of introducing a temporal barrier constraint is to force the optimal cost of constrained agent to increase by $1+k-delay$. 
%However, when $k \geq 2$, the temporal barrier constraint with $B(a_x, R_x, R_g, k, delay)$ failed. As shown in Figure \ref{fig4:sub1}, when $k=2$, temporal barrier constraint $B(a_i,(4,4),(4,5),2,0)$ is used to force $a_i$’s optimal path to increase by 3, to a length of 9, to avoid the conflict with $a_j$. 
%However, the cost of optimal paths of agent $a_i$ is still 8, 
%because $a_i$ can bypass the temporal barrier constraint. In this case, all paths of $a_i$ with cost 8 conflict with all the optimal paths of $a_j$ in the light yellow area, which is larger than the rectangle. 
%
%The light yellow area is an extended rectangle area. Each time $k$ increased by 2, constrained agent need to find a path with 2 more cost. This makes CBS can choose a wider path with 2 more cost that bypass rectangle area, which means the size of the extended rectangle area increased.
%
%Once $k$ is big enough to force the agent to bypass the unconstrained agent’s start-goal rectangle, the optimal path of constrained agents will no longer intersect with unconstrained agent’s optimal path. Thus the extended rectangle area is at most the unconstrained agent’s start-goal rectangle. 
%
%\subsection{$k$-Robust Cardinal Rectangle Reasoning}
%
%On approach to overcome the above problem is to use the border of the extended rectangle area to define a temporal barrier constraint. 
%We use a simpler method which extends the border of unconstrained agent’s start and goal rectangle as the barrier in order to to overcome this problem. Figure \ref{fig4:sub2} shows the latest timestep that $a_i$ can arrive at each vertex in the rectangle area when trying to reach the goal at timestep 9. 
%In this case, the low-level search of $a_i$ has many options for reaching 
%the goal at timestep 9 without conflict with optimal paths of agent $a_i$.  Figure \ref{fig4:sub3} shows the CT tree when solving rectangle conflicts with temporal range constraints. We denote the temporal barrier constraint using the border of unconstrained agent’s start and goal rectangle as $B(a_x, Rs_x, Rg_x, k, delay), x \in [ i, j ]$. 
%$Rs_x$ and $Rg_x$ are the two corner nodes of the border of the start-goal rectangle that are opposite to $a_x$’s start location $s_x$. 
%We call the algorithm using the extended
%temporal border constraint $B(a_x, Rs_x, Rg_x, k, delay), x \in [ i, j ]$ to resolve $k$-delay cardinal rectangle conflict as \textbf{K-CBSH-CR}.
%
%Using the border of unconstrained agent’s start and goal rectangle will introduce some redundant constraints. But they do not over constrain the target agent. Using the example in Figure \ref{fig4:sub2}, if the $k=2$ and 
%vertex (4,2) is constrained at timesteps 1, 2, and 3, since the earliest timestep that the constrained agent can arrive at (4,2) is 5 this does remove any possible paths for the agent.
%Similarly while vertex (6,7) is constrained at timesteps 6, 7, and 8; paths for $a_i$ to reach the goal through (6,7) have a cost of at least 10, and hence no possible paths are removed. 
%
%\textbf{Property 1.} For any path combination of two agents $a_i$ and $a_j$ that have $k$-delay cardinal rectangle conflict (assuming $a_i$ arrives rectangle area $\Delta$ timestpes early than $a_j$). If one path violates $B(a_i, Rs_i, Rg_i, k,0)$ and the other path violates $B(a_j, Rs_j, Rg_j, k,\Delta)$, then the two agents have $k$-delay conflict within the rectangle area.
%
%\textit{Proof.} 
%If the optimal time that agent $a_i$ can arrive vertex $N_i$ on border $Rs_i$ to $Rg_i$ is $c_i$.  Now $a_i$ arrives at $N_i$ at $t_i$, $c_i \leq t_i \leq c_i+k$ and $d_i=t_i-c_i$ ($d_i$ is the timestep difference between the timestep that $a_i$ arrive $N_i$ and the optimal timestep that $a_i$ can arrive $N_i$), hence $a_i$ violates constraint $B(a_i, Rs_i, Rg_i, k,0)$.
%
%If the optimal time that agent $a_j$ can arrive vertex $N_j$ on border $Rs_j$ to $Rg_j$ is $c_j$ and the optimal time that agent $a_i$ can arrive vertex $N_j$ is $c_{i\_nj}$. Hence the timestep difference that two agents optimally arrive a vertex in rectangle area is $\Delta$, $c_{i\_nj} + \Delta = c_j$ and $c_{i\_nj}\leq c_j$. 
%Now the $a_j$ arrive $N_j$ at $t_j$, and $c_{i\_nj}\leq c_j\leq t_j\leq c_j-\Delta + k = c_{i\_nj}+k$, hence $a_j$ violate $B(a_j, Rs_j, Rg_j, k,\Delta)$. $d_j=t_j-c_j$, which is the timestep difference between $t_j$ and $c_j$.
%
%The requirement (c) in section 5.1 guarantees that the path of $a_i$ and the path of $a_j$ must have an intersect vertex, which means they both traverse a vertex at same or different timestep. The intersection vertex in denoted as $v$. 
%
%The optimal time that $a_i$ arrive $v$ is $c_{i\_v}$, which is also the earliest time that $a_i$ can arrive $v$. 
%
%The optimal time that $a_j$ can arrive $v$ is $c_{j\_v}$ and the latest time that $a_j$ can arrive $v$ is $c_{j\_v}+d_j$. 
%
%As agent $a_i$ and $a_j$ have $k$-delay rectangle conflicts and the optimal path of $a_i$ arrive rectangle area early than $a_j$, thus $c_{j\_v}-c_{i\_v}=\Delta$ and $\Delta \leq k$. 
%
%Because $t_j\leq c_{i\_nj}+k$:
%\[t_j-c_j\leq c_{i\_nj}+k-c_j\]
%\[d_j\leq c_{i\_nj}+k-c_j\]
%As $a_i$ and $a_j$ have $k$-delay rectangle conflicts, the time difference that two agents' optimal path arrive any vertex in rectangle conflicts is $\Delta$ and also because of $c_{i\_nj}\leq c_j$:
%\[d_j\leq -\Delta+k\]
%\[d_j+\Delta\leq k\]
%Thus 
%\[d_j+c_{j\_v}- c_{i\_v} \leq k\]
%Hence $d_j+c_{j\_v}$ is the latest time that $a_j$ can arrive vertex $v$ and $c_{i\_v}$ is the earliest time that $a_i$ can arrive $v$, the time difference between the latest time that $a_j$ can arrive $v$ and the earliest time that $a_i$ can arrive $v$ is always smaller than k, which means have a $k$-delay conflict between $a_i$ and $a_j$ at $v$.
%
%Therefore if $a_i$ and $a_j$ have $k$-delay rectangle conflicts, one path violates $B(a_i, Rs_i, Rg_i, k,0)$ and the other path violates $B(a_j, Rs_j, Rg_j, k,\Delta)$, then the two agents have $k$-delay conflict within the rectangle area.
%\qed
%
%\mike{Sketch of proof}
%\textit{Proof Sketch.} 
%The requirement (c) in section 5.1 guarantees that the path of $a_i$ and the path of $a_j$ must have an intersect vertex $v$ if both agents traverse each other's start and goal rectangle. 
%
%Assuming the optimal time that agent $a_i$ can arrive vertex $N_i$ on border $Rs_i$ to $Rg_i$ is $c_i$ and the real time $a_i$ arrives at $N_i$ is $t_i$, $c_i \leq t_i \leq c_i+k$ and $d_i=t_i-c_i$.
%
%Assuming the optimal time that agent $a_j$ can arrive vertex $N_j$ on border $Rs_j$ to $Rg_j$ is $c_j$ and the optimal time that agent $a_i$ can arrive vertex $N_j$ is $c_{i\_nj}$. Hence the timestep difference that two agents optimally arrive a vertex in rectangle area is $\Delta$, $c_{i\_nj} + \Delta = c_j$ and $c_{i\_nj}\leq c_j$. Assuming the real time the $a_j$ arrive $N_j$ is $t_j$, $c_{i\_nj}\leq c_j\leq t_j\leq c_j-\Delta + k = c_{i\_nj}+k$, and $d_j=t_j-c_j$.
%
%Assuming the optimal time (earliest time) that $a_i$ can arrive $v$ is $c_{i\_v}$. 
%
%Assuming optimal time that $a_j$ can arrive $v$ is $c_{j\_v}$, the latest time that $a_j$ can arrive $v$ is $c_{j\_v}+d_j$. 
%
%As $a_i$'s optimal path have $k$-delay conflict with $a_j$'s optimal path, we know $c_{j\_v}-c_{i\_v}=\Delta$.
%
%With these information, we can prove that $c_{j\_v}+d_j - c_{i\_v}$ always smaller than k, which means we have a $k$-delay conflict at $v$.
%\qed
%
%
%\subsubsection{Theorem 1.} K-CBSH-CR is complete and optimal.
%
%\textit{Proof.}  The proof is similar to the proofs in \citet{atzmon} and \citet{li2019}.  
%If $a_i$ and $a_j$ have a conflict $(a_i, a_j, v, t, \Delta$. For a CT node $N$, $N1$ and $N2$ are the child nodes for $N$. $N1$ hold the constraint $B(a_i, Rs_i, Rs_i, k,0)$ and $N2$ hold the constraint $B(a_j, Rs_j, 
%Rs_j, k,\Delta)$. $\pi(N1)$ denotes all the $k$-Robust plans that satisfy $N1.constraints$ and $\pi(N2)$ denotes all the $k$-Robust plans that satisfy $N2.constraints$. Based on property 1, the temporal barrier constraint does not eliminate any conflict-free solutions. Thus $\pi (N) =  \pi (N1) \cup \pi (N2)$. Thus K-CBSH-CR does not eliminate any possible solution and is complete. Furthermore, the low-level search of any kind of CBS always returns an optimal path, the high-level search always chooses a CT node with minimum $f$-value to expand and K-CBSH-CR does not eliminate any possible solution when splitting. Therefore, the first chosen CT node whose paths are conflict-free has a set of conflict-free paths with minimum cost. Thus K-CBSH-CR is optimal.
%\qed
%
%\subsection{Extending $k$-Robust Rectangle Reasoning}
%
%\citet{li2019} shows that rectangle reasoning can also be used to resolve semi-cardinal rectangle conflict and non-cardinal rectangle conflicts, not only cardinal rectangle conflicts. This algorithm is called CBSH-R. As the 
%barrier constraints only block paths that traverse the rectangle area and do not block all optimal paths for semi-cardinal or non-cardinal rectangle conflicts, it may fail to resolve some conflicts. CBSH-R needs to esnure 
%the barrier constraint resolves the current conflict so that it cannot
%arise in the current node’s ancestors.  By replacing the barrier constraint with a temporal barrier constraint using the border of the unconstrained agent’s start-goal rectangle, CBSH-R is modified to plan $k$-Robust solutions and we denote this algorithm \textbf{K-CBSH-R}. 
%
%\textbf{Theorem 2.} K-CBSH-R is complete and optimal.
%
%\textbf{Proof.} As temporal barrier constraint for $a_i$ will not block any path that does not traverse $a_j$’s start goal rectangle, thus temporal barrier constraint for $a_i$ will not block any path that does not intersect with $a_j$’s path. Therefore Property 1 still holds for K-CBSH-R. Thus the proof in Theorem 1 still works for K-CBSH-R, which means K-CBSH-R also is complete and optimal. \qed
%
%\subsubsection{Rectangle Conflict in Path Segments}
%\citet{li2019} further extends the usage of barrier constraints and use it to solve rectangle conflicts caused by obstacles and other constraints. It uses a Multi-Valued Decision Diagram (MDD) (Sharon et al. 2013), which is a directed acyclic graph, to find singletons in the paths of each agent. An MDD stores all possible locations at each timestep for an agent to reach its goal optimally, which is the same as storing all optimal paths of an agent. If a timestep only has one possible location, which means all optimal paths must traverse this location at this timestep, this location at this time step is called a singleton. This algorithm uses all the singletons from conflict agents’ paths as candidate start and goal locations and then CBSH-RM try to find and classify rectangle conflicts in all possible start and goal combinations. When multiple conflicts exist, CBSH-RM first prefers rectangle conflicts with higher priority type, then it prefers a larger rectangle area. 
%
%For $k$-delay rectangle conflicts, current conflict detection tie braking policy cannot efficiently resolve all problems, as the rectangle conflicts does not consider extended rectangle area. Thus, for $k$-Robust plan, the rectangle conflicts with larger extended rectangle area are preferred when two rectangle conflicts have the same priority type and rectangle area.\
%
%\subsubsection{Adding Temporal Barrier Constraint}
%\citet{li2019} also find that if blocking all vertexes on the border of the rectangle opposite the constrained agent, CBSH-RM may lose optimality. Because when barrier constraint force the agent to reach the goal with a higher cost, it is possible that alternative paths, which do not traverse selected start singleton but traverse constrained barrier vertexes. Blocking all vertexes on the border of the rectangle area loses these path choices. By using MDD for each agent in conflict, CBSH-RM avoid losing optimality by checking does any optimal path of constrained agent traverse the vertexes included in barrier constraint and if no any optimal path traverse a vertex, this vertex will not be constrained.
%
%$k$-Robust rectangle reasoning requires to block the extended rectangle area as well. Although the MDD provides the information of all optimal paths of an agent, these optimal paths do not traverse extended rectangle area. Therefore, if the optimal cost from selected start singleton to selected goal singleton is $c$, an MDD of constrained agent stores all paths from selected start singleton to selected goal singleton with a cost of $c+k$ is used to support the adding of temporal barrier constraint. An MDD with the cost of $c+k$ contains all paths with cost $i,  c\leq i \leq c+k$, as a path with cost i can become a path with cost c+k by waiting at goal location.
%
%For any vertex $v$ in the border of extended rectangle area opposite to constrained agent, if the optimal time that the agent arrives at the vertex is $t$ , the time that the agent arrive selected start singleton is $t_s$, and the level $(t-t_s) +i,i\in (0,k)$, of the MDD include vertex $v$, $v$ is constrained from time $t+i$ to $t +k$. By constraint the vertexes only exist in MDD Property 1 still holds here. This algorithm is denoted as K-CBSH-RM.
%
%\mike{A shorten version:} \citet{li2019} shows that rectangle reasoning can also be used to resolve semi-cardinal rectangle conflict and non-cardinal rectangle conflicts, not only cardinal rectangle conflicts. By replacing the barrier constraint with a temporal barrier constraint, it is modified to plan $k$-Robust solutions and we denote this as \textbf{K-CBSH-R}. \citet{li2019} further extends the usage of barrier constraints and use it to solve rectangle conflicts caused by obstacles and other constraints. It uses a Multi-Valued Decision Diagram (MDD) (Sharon et al. 2013), which is a directed acyclic graph, to find singletons in the paths of each agent. An MDD stores all possible paths of an agent at a certain cost. If a timestep only has one location, which means all paths traverse this location at this timestep, it is called a singleton. This algorithm uses all the singletons from conflict agents’ paths as candidate start and goal locations and then CBSH-RM try to find rectangle conflicts in all possible start and goal combinations. By replacing barrier constraint with temporal constraint, it works for planning $k$-robust solution and is denoted as \textbf{K-CBSH-RM}.
%
%
%
%\section{$k$-Robust Corridor Reasoning}
%The difference between corridor conflict with $k$-Robust CBS and normal corridor conflict is that agents need to occupy vertexes for extra timesteps to avoid $k$-delay conflicts. Assume there is a corridor conflict with a length of $l$ between vertex $b$ and vertex $e$. Agent $a_1$ moving from $b$ to $e$ and agent $a_2$ moving from $e$ to $b$. If the agent $a_1$ reach vertex $e$ at timestep $t_1$ and agent $a_2$ reach vertex $b$ at timestep $t_2$.For planning $k$-Robust solution, any path of $a_1$ that reach vertex $e$ at or before timestep $t_2+l+k$ must conflict with any paths of $a_2$ that reach vertex $b$ at or before timestep $t_1+l+k$.
%
%When considering bypasses, assuming agent $a_1$ can reach vertex $e$ at timestep $t'_1$ and agent $a_2$ reach vertex $b$ at timestep $t'_2$ without traverse the corridor. Therefore for planning $k$-Robust solution, any path of $a_1$ that reach vertex $e$ at or before timestep $min(t'_1  - 1+k,t_2  + l+k)$ must conflict with any paths of $a_2$ that reach vertex $b$ at or before timestep $min(t'_2  - 1+k,t_1  + l+k)$.
%
%Therefore, a pair of range constraint is used to perform $k$-Robust corridor reasoning. When splitting CT node, child node 1 hold the constraint $<a_1,e,[0,min(t'_1  - 1+k,t_2  + l+k)]>$ and child node 2 hold the constraint $<a_2,b,[0,min(t'_2  - 1+k,t_1  + l+k)]>$.
%
%\textbf{Theorem 2.} $k$-Robust Corridor Reasoning is complete and optimal.
%
%\textit{Proof} We have shown that if $a_1$ and $a_2$ both violate constraint $<a_1,e,[0,min(t'_1  - 1+k,t_2  + l+k)]>$ and constraint $<a_2,b,[0,min(t'_2  - 1+k,t_1  + l+k)]>$, they must have a conflict in the corridor. Thus the adding of these constraints will not eliminate any conflict free $k$-Robust solution. Thus $k$-Robust Corridor Reasoning is complete. $k$-Robust Corridor Reasoning is based on CBS, as proved in Theorem 1, CBS guarantees that the solution is optimal as long as no conflict free solution is eliminated.
%
%\section{$k$-Robust Target Reasoning}
%Assuming that agent $a_i$ reaches its goal $g_i$ on timestep $l$, and agent $a_j$ has a target conflict with the agent $a_i$ at $g_i$ on timestep $t,t \geq l$. All solutions that both $a_i$ and $a_j$ visit $g_i$ at $t$ must have conflict. ~\citet{corridor} resolve target conflict by force $a_i$ to reach its goal after $t$ or force any other agent visit $g_i$ at or after $t$. Planning $k$-Robust solution requires the avoiding of $k$-delay conflict. Therefore, when splitting, one child node forces $a_i$ to reach its goal after $t+k$ to give $a_2$ priority and do not cause $k$-delay conflict. Another child node forbids any other agent visit $g_i$ at or after $t$ to force all other agents find bypasses to their goal locations. If any agent failed to find a bypass route, we do not generate this child node. 
%
%\textbf{Theorem 3.} $k$-Robust Target Reasoning is complete and optimal.
%
%\textit{Proof} We have shown that target reasoning only eliminate the solutions that have target conflict and do not eliminate any conflict free solution. Thus $K$-robust Target Reasoning is complete. $k$-Robust Target Reasoning is based on CBS. As proved in Theorem 1, CBS guarantees that the solution is optimal as long as no conflict free solution is eliminated.


==> reasoning-old.tex <==
\section{$k$-Robust Rectangle Reasoning}

%$k$-Robust rectangle conflicts occur when 
%two agents arrive in a rectangle area such as Figure~\ref{fig1} (left);
%not just at the same time but also within $k$ timesteps of one another.


A rectangle conflict arises when two agents paths need to cross
but there are many ways that they can cross. This causes difficulty 


Figure~\ref{fig1} (a) illustrates a ($k = 0$) rectangle conflict,
any optimal paths for the two agents from their start to target will conflict somewhere in the rectangle. In a $k$-delay rectangle conflict the agents may not arrive at a vertex at the same time, but within $k$ timesteps. For example is we move $S_2$ to (2,2) the same illustrated rectangle is a $1$-delay rectangle conflict. 

To resolve such conflicts we introduce \textbf{Temporal Barrier Constraints}, which unify
the (temporal) range constraints of~\cite{atzmon} and the (spatial) Barrier Constraints of~\cite{li2019}.

\begin{defn}
Given a vertex time pair $p = (u,t)$ the \emph{optimal time} 
$ot(p,v)$ to reach 
vertex $v = (v_x,v_y)$ starting from $u = (u_x,u_y)$ at time $t$ is
calculated by adding the Manhattan distance 
$ot(p,v) = t + |v_x - u_x| + |v_y - u_y|$.

A \emph{$w$ temporal barrier constraint} is denoted by
$B(a_x, V, p, w)$. 
This constraint forbids the 
agent $a_x$ from visiting any vertex $v \in V$ 
at the optimal time from vertex time pair $p$, or any time step up to $w$ later. 
That is the barrier constraint $B(a_x, V, p, w)$ 
is the set of time-range vertex constraints$\langle a_x, v, [ot(p,v), ot(p,v) + w] \rangle, v \in V$.
\label{defi:barrier}
\end{defn}


Given a rectangular grid map we can define a \emph{rooted rectangle} $R$ as the set of vertices
occurring in the rectangle defined by the 
two corner points $(D_x,D_y)$ the root corner, and 
$(E_x,E_y)$ the opposite corner. 
In Figure~\ref{fig1} the illustrated rectangle is  defined by (2,2) and (3,3).

A rectangle $R$ defined by $((D_x,D_y),(E_x,E_y))$ defines 4 sides: 
$S1(R) = \{ (D_x,D_y) .. (D_x,E_y) \}$,
$S2(R) = \{ (D_x,D_y) .. (E_x,D_y) \}$,
$S3(R) = \{ (D_x,E_y) .. (E_x,E_y) \}$, and
$S4(R) = \{ (E_x,D_y) .. (E_x,E_y) \}$.
For the illustrated rectangle of Figure~\ref{fig1}, 
$S1(R)$ is the left side \{ (2,2),(2,3)\},
$S2(R)$ is the top, $S3(R)$ is the bottom, and $S4(R)$ the right side.

We can now explain a rectangle conflict for the case $k = 0$
differently from the explanation in ~\cite{li2019}.

\begin{theorem}\label{thm:rect:0}
Given an arbitrary rectangle $R$ defined by $((D_x,D_y),(E_x,E_y))$
and root time $rt$
and two paths for agents $a_1$ and $a_2$ such that
constraints $B(a_1,S1(R),(D,rt),0)$,
$B(a_1,S4(R),(D,rt),0)$,
$B(a_2,S2(R),(D,rt),0)$, and
$B(a_2,S3(R),(D,rt),0)$ are all violated, then
the paths of the two agents have a $0$-delay vertex conflict.
\end{theorem}
\begin{proof}
Assume that $S1(R)$ is the left of the rectangle, 
$S4(R)$ the right, $S2(R)$ the top, and $S3(R)$ the bottom, 
the other cases follow similarly. 

Since agent $a_1$ enters the rectangle at the left at the optimal time, and leaves from the right at the optimal time it cannot wait, and must remain within the rectangle, and every vertex it visits within the rectangle it visits at the optimal time.
Similarly for agent $a_2$. 
Now since agent $a_1$ crosses from left to right, and agent $a_2$ from top to bottom, there paths must cross.  Since they share a vertex $v \in R$ and they only visit vertices at the optimal time, their paths have the vertex conflict $\langle a_1,a_2,v,ot((D,rt),v),0 \rangle$.
\end{proof}

This leads to a generic way of handling a rectangle conflict. 
Since no two compatible agents paths can violate all four barriers we can impose the constraint 
$B(a_1,S1(R),(D,rt),0)$ $\vee$
$B(a_1,S4(R),(D,rt),0)$ $\vee$
$B(a_2,S2(R),(D,rt),0)$ $\vee$
$B(a_2,S3(R),(D,rt),0)$ 
without removing solutions.  This is imposed by a four way branch where we impose of the constraints in each branch. 

We can usually do better than this. If all possible paths for $a_1$ 
(given the current set of constraints upon it) that violate
$B(a_1,S4(R),(D,rt),0)$ must also violate $B(a_1,S1(R),(D,rt),0)$ 
we can remove the second disjunct. 
This is common, note for the example that any path for agent $a_1$ in Figure~\ref{fig1}
which reaches the right side at the optimal time, also crossed the left side at the optimal time.
The same reasoning applies for $B(a_2,S2(R),(D,rt),0)$ $\vee$
$B(a_2,S3(R),(D,rt),0)$. Hence usually we end up with a two way branch
$B(a_1,S4(R),(D,rt),0)$ $\vee$
$B(a_2,S3(R),(D,rt),0)$.

We can extend the above 
reasoning for $k > 0$ conflicts.

\begin{theorem}\label{thm:rect:1}
Given an arbitrary rectangle $R$ defined by $((D_x,D_y),(E_x,E_y))$
and two root times $rt_1$ and $rt_2$
and two paths for agents $a_1$ and $a_2$ such that
constraints 
$B(a_1,S1(R),(D,rt_1),1)$,
$B(a_1,S4(R),(D,rt_1),1)$,
$B(a_2,S2(R),(D,rt_2)),1)$, and
$B(a_2,S3(R),(D,rt_2)),1)$ are all violated, then
the paths of the two agents have a $k$-delay vertex conflict,
assuming $max(rt_1,rt_2)+1 - min(rt_1,rt_2) \leq k$
\end{theorem}
\begin{proof}
Assume that $S1(R)$ is the left of the rectangle, 
$S4(R)$ the right, $S2(R)$ the top and $S3(R)$ the bottom, 
the other cases follow similarly. 

Since agent $a_1$ enters the rectangle at the left at the optimal time wrt $rt_1$ or one later, and leaves from the right at the optimal time or one later
its path can wait at most one step in the rectangle, and cannot leave the rectangle, since this would require at least 2 time steps.
Every vertex it visits in the rectangle is visited at the optimal time wrt $rt_1$, or the optimal time + 1 (or both).
Similarly agent $a_2$ enters the top of rectangle at optimal time wrt $rt_2$ or one later, and leaves the bottom of the rectangle at the optimal time wrt $rt_2$ or one later. Again it cannot leave the rectangle, and can take at most one wait in the rectangle. Every vertex it visits at the optimal time wrt $r_t$ or one later (or both).

Now since agent $a_1$ crosses from left to right, and agent $a_2$ from top to bottom, there paths must cross.  Since they share a vertex $v \in R$ since they agent $a_1$ this vertex at $t_1 \in ot((D,rt_1),v) .. ot((D,rt_1),v)+1$, agent $a_2$ visits this vertex at $t_2 \in ot((D,rt_1),v).. ot((D,rt_2),v) + 1$
there is a $k$-delay conflict
$\langle a_1, a_2, v, t, k \rangle$, 
since by the conditions on
$rt_1$ and $rt_2$, $| t_1 - t_2| \leq k$.
\end{proof}

We can resolve the rectangle conflict by branching on 
$B(a_1,S1(R),(D,rt_1),1)$ $\vee$
$B(a_1,S4(R),(D,rt_1),1)$ $\vee$
$B(a_2,S2(R),(D,rt_2),1)$ $\vee$
$B(a_2,S3(R),(D,rt_2),1)$,
and often, if we can prove the required implications, the simpler 
$B(a_1,S4(R),(D,rt_1),1)$ $\vee$
$B(a_2,S3(R),(D,rt_2),1)$.
Currently none of our methods detect the simpler 2 way splitting case.
\pjs{Is this true mike! mike: for the plots currently showing in this paper, no 2-way split CR/RM.}
Note that the barriers we create are $1$-barriers (for two consecutive time steps). 
Unfortunately we cannot easily extend to $w$-barriers where $w \geq 2$.
As shown in Figure~\ref{fig3}, consider the 3x3 rectangle $R = ((2,2),(4,4))$ 
with root times $rt_1 = rt_2 = 1$, 
and the paths for agent $a_1$ 
[((1,2),0), ((1,3),1), ((1,4),2), ((2,4),3), 
 ((2,5),4), ((3,5),5), ((4,5),6), ((4,4),7), ((5,4),8))]
 and for agent $a_2$
[((2,1),0), ((3,1),1), ((3,2),2), ((3,3),3), ((3,4),4), 
 ((3,4),5), ((3,4),6), ((3,4),7), ((3,5),8), ((4,5),9)].
Note that agent $a_1$ violates $2$-barrier $B(a_1,S1(R),((2,2),1),2)$ 
at $((2,4),3)$
and $2$-barrier $B(a_1,S4(R),((2,2),1),2)$ at $((4,4),7)$; while
agent $a_2$ violates $2$-barrier $B(a_2,S2(R),((2,2),1),2)$ 
at $((3,2),2)$
and $2$-barrier $B(a_2,S3(R),((2,2),1),2)$ at $((3,4),4)$ but 
the paths of the agents do not intersect within the rectangle $R$,
indeed there are no conflicts, since agent $a_2$ waits before leaving the rectangle. 



\begin{figure}
  \centering
  \includegraphics[width=0.50\columnwidth]{2barrierExample.jpg}
  \caption{Example of how $w$-barriers where $w \geq 2$ can eliminate a conflict free solution.}
  \label{fig3}
\end{figure}

\subsection{Detecting Rectangle Conflicts}

When we detect a vertex conflict during CBS we need to recognise that it's actually a 
rectangle conflict, in order to perform the rectangle symmetry breaking.
The simplest way of recognizing a rectangle conflict, called CR in~\cite{li2019}, can be understood as follows:
\begin{itemize}
\item[(a)] Both agents follow their Manhattan optimal paths from start to goal. 
\item[(b)] Both agents move in only the same horizontal and vertical directions along their paths.
\item[(c)] The start and goal nodes of two agents have relative opposite locations. This requirement ensures that all optimal paths of both agents intersect within the rectangle area.
\end{itemize}
Figure~\ref{fig1} gives an example. 

In this case \citet{li2019} defines the rectangle from the start and goal locations.
Suppose the agents currents paths have $k$-delay conflict 
at vertex $v$ with agent $a_1$ arriving at time $t$ and agent $a_2$ arriving at time $t + \Delta, 
\Delta \leq k$. 
$D = (D_x,D_y)$ is given by $D_x$ is the closest of the start locations in the $x$ dimension to $v$, and similarly $D_y$ in the $y$ dimension.
$E = (E_x,E_y)$ is defined similarly from the goal locations. 

Using Theorem~\ref{thm:rect:1} we can extend this to handle $k$-delay conflicts.
Clearly the current paths must conflict with barriers of the rectangle $R$ defined by $D$ and $E$.
Hence we can apply the rectangle conflict splitting to remove the current paths.
We call the detection of CR rectangle and the associated branching K-CBSH-CR

\begin{theorem}
K-CBSH-CR is correct.
\end{theorem}
\begin{proof}
By definition all barrier constraints of the rectangle $R$ are violated by the current paths of the agents. 
From Theorem~\ref{thm:rect:1} applying the barrier disjunction cannot remove solutions, and certainly removes the current paths.
\end{proof}


We can extend the detection of rectangle conflicts to more complicated cases as follows.

Assume agent $a_1$ and $a_2$ have a $k$-delay vertex conflict $\langle a_1, a_2, v, t, \Delta \rangle$.
Assume that $a_1$ enters $v$ moving in direction $d_1$ and $a_2$ enters moving in direction $d_2$.  They must be different or there is an earlier vertex conflict (where they both came from). 
If they are opposite directions then there is no rectangle conflict.

So assume $d_1$ and $d_2$ are orthogonal directions.
Let $(B1_x,B1_y)$ be the earliest singleton in the path of agent $a_1$ where all moves from here to $v$ are in direction $d_1$ or $d_2$
and there are no waits, similarly define $(B2_x,B2_y)$ for agent $a_2$.
Let $(A1_x,A1_y)$ be the latest singleton in the path of agent $a_1$ where all moves from $v$ to here are in directions $d_1$ or $d_2$
and there are no waits, similarly define $(A2_x,A2_y)$ for agent $a_2$.

Define $D_x$ to be the closer of $B1_x$ and $B2_x$ to $v_x$,
similarly for $D_y$. Define $E_x$ to be the closer of $A1_x$
and $A2_x$ to $v_x$, similarly for $E_y$. 

Now either the current path of $a_1$ crosses the entry barrier for $d_1$ in $R$ and $a_2$ crosses the entry barrier for $d_2$ in $R$ or there must be a vertex $B'$ before $v$ in both paths where the two paths cross (otherwise they could not enter vertex $v$ in the appropriate direction).  If the second case holds, replace $B$ by $B'$. 
Similarly the current path of $a_1$ must cross the exit barrier for $d_1$ in $R$ and $a_2$ must cross the exit barrier or there is a vertex $E'$ after $v$ in both paths where they cross. Again in the second case replace $E$ by $E'$. Figure~\ref{RecDectFig} shows an example of the detection of a rectangle conflicts when $k$=2.

\begin{figure}
  \centering
  \includegraphics[width=0.4\columnwidth]{RMRecDetect.jpg}
  \caption{Detecting a rectangle conflict when $k=2$; $E$ is replaced by $E'$ as the two paths cross after $V$. }
  \label{RecDectFig}
\end{figure}

By construction the current paths for $a_1$ crosses the entry and exit barriers for $d_1$ at the optimal time wrt $(B,t - |B1_x - v_x| - |B1_y - v_y|)$, similarly $a_2$ crosses the entry and exit barriers for $d_2$ at the optimal time wrt $(B,t+\Delta - |B1_x - v_x| - |B1_y - v_y|)$.
Hence we can apply the rectangle construction of Theorem~\ref{thm:rect:1}
where $rt_1 = t - |B1_x - v_x| - |B1_y - v_y|$ and
$rt_2 = t+\Delta - |B1_x - v_x| - |B1_y - v_y|-1$ unless $\Delta = 0$ and $k = 1$ in which case $rt_2 = rt_1$, since the conditions for the Theorem hold.
The rectangle construction removes the current paths, and other symmetric paths that would lead to the same rectangle conflict.
We call the detection of these more general rectangles and the associated branching K-CBSH-RM (it's a generalization of the RM technique defined by~\citet{li2019}, which has an $O(N^4)$ complexity on rectangle detection while the method here has an complexity of $O(n)$). The correctness holds similarly.

\begin{theorem}
K-CBSH-RM is corect.
\end{theorem}





==> temp.tex <==

% \def\year{2020}\relax
% %File: formatting-instruction.tex
% \documentclass[letterpaper]{article} % DO NOT CHANGE THIS
% \usepackage{aaai20}  % DO NOT CHANGE THIS
% \usepackage{times}  % DO NOT CHANGE THIS
% \usepackage{helvet} % DO NOT CHANGE THIS
% \usepackage{courier}  % DO NOT CHANGE THIS
% \usepackage[hyphens]{url}  % DO NOT CHANGE THIS
% \usepackage{graphicx} % DO NOT CHANGE THIS
% \usepackage{subcaption}
% \usepackage{amsthm}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \urlstyle{rm} % DO NOT CHANGE THIS
% \def\UrlFont{\rm}  % DO NOT CHANGE THIS
% \usepackage{graphicx}  % DO NOT CHANGE THIS
% \frenchspacing  % DO NOT CHANGE THIS
% \setlength{\pdfpagewidth}{8.5in}  % DO NOT CHANGE THIS
% \setlength{\pdfpageheight}{11in}  % DO NOT CHANGE THIS
% %\nocopyright
% %PDF Info Is REQUIRED.
% % For /Author, add all authors within the parentheses, separated by commas. No accents or commands.
% % For /Title, add Title in Mixed Case. No accents or commands. Retain the parentheses.
%  \pdfinfo{
% /Title (Symmetry Breaking $k$-Robust Multi-Agent Path Finding)
% /Author ()
% } %Leave this	
% % /Title ()
% % Put your actual complete title (no codes, scripts, shortcuts, or LaTeX commands) within the parentheses in mixed case
% % Leave the space between \Title and the beginning parenthesis alone
% % /Author ()
% % Put your actual complete list of authors (no codes, scripts, shortcuts, or LaTeX commands) within the parentheses in mixed case. 
% % Each author should be only by a comma. If the name contains accents, remove them. If there are any LaTeX commands, 
% % remove them. 

% % DISALLOWED PACKAGES
% % \usepackage{authblk} --This package is specifically forbidden
% % \usepackage{balance} --This package is specifically forbidden
% % \usepackage{caption} --This package is specifically forbidden
% % \usepackage{color (if used in text)
% % \usepackage{CJK} --This package is specifically forbidden
% % \usepackage{float} --This package is specifically forbidden
% % \usepackage{flushend} --This package is specifically forbidden
% % \usepackage{fontenc} --This package is specifically forbidden
% % \usepackage{fullpage} --This package is specifically forbidden
% % \usepackage{geometry} --This package is specifically forbidden
% % \usepackage{grffile} --This package is specifically forbidden
% % \usepackage{hyperref} --This package is specifically forbidden
% % \usepackage{navigator} --This package is specifically forbidden
% % (or any other package that embeds links such as navigator or hyperref)
% % \indentfirst} --This package is specifically forbidden
% % \layout} --This package is specifically forbidden
% % \multicol} --This package is specifically forbidden
% % \nameref} --This package is specifically forbidden
% % \natbib} --This package is specifically forbidden --use the following workaround:
% % \usepackage{savetrees} --This package is specifically forbidden
% % \usepackage{setspace} --This package is specifically forbidden
% % \usepackage{stfloats} --This package is specifically forbidden
% % \usepackage{tabu} --This package is specifically forbidden
% % \usepackage{titlesec} --This package is specifically forbidden
% % \usepackage{tocbibind} --This package is specifically forbidden
% % \usepackage{ulem} --This package is specifically forbidden
% % \usepackage{wrapfig} --This package is specifically forbidden
% % DISALLOWED COMMANDS
% % \nocopyright --Your paper will not be published if you use this command
% % \addtolength --This command may not be used
% % \balance --This command may not be used
% % \baselinestretch --Your paper will not be published if you use this command
% % \clearpage --No page breaks of any kind may be used for the final version of your paper
% % \columnsep --This command may not be used
% % \newpage --No page breaks of any kind may be used for the final version of your paper
% % \pagebreak --No page breaks of any kind may be used for the final version of your paperr
% % \pagestyle --This command may not be used
% % \tiny --This is not an acceptable font size.
% % \vspace{---No negative value may be used in proximity of a caption, figure, table, section, subsection, subsubsection, or reference
% % \vskip{---No negative value may be used to alter spacing above or below a caption, figure, table, section, subsection, subsubsection, or reference

% \frenchspacing
% \newcommand{\citet}[1]{\citeauthor{#1}~\shortcite{#1}}
% \newcommand{\citep}{\cite}
% \newcommand{\citealp}[1]{\citeauthor{#1}~\citeyear{#1}}
% \usepackage{latexsym}
% %\newcommand{\qed}{\hfill$\Box$}

% \newtheorem{theorem}{Theorem}

% %%%%%%% THIS MUST BE REMOVED BEFORE SUBMISSION!
% \usepackage{color}
% \newcommand{\pjs}[1]{\textcolor{blue}{PJS: #1}}
% \newcommand{\ddh}[1]{\textcolor{red}{DDH: #1}}
% \newcommand{\mike}[1]{\textcolor{green}{Mike: #1}}
% \renewcommand{\pjs}[1]{}
% \renewcommand{\ddh}[1]{}
% \renewcommand{\mike}[1]{}


% \newcommand{\ignore}[1]{}

% \setcounter{secnumdepth}{2} %May be changed to 1 or 2 if section numbers are desired.

% % The file aaai20.sty is the style file for AAAI Press 
% % proceedings, working notes, and technical reports.
% %
% \setlength\titlebox{2.5in} % If your paper contains an overfull \vbox too high warning at the beginning of the document, use this
% % command to correct it. You may not alter the value below 2.5 in

